DiPETrans: A Framework for Distributed Parallel Execution of Transactions of Blocks in Blockchain

Contemporary blockchain such as Bitcoin and Ethereum execute transactions serially by miners and validators and determine the Proof-of-Work (PoW). Such serial execution is unable to exploit modern multi-core resources efficiently, hence limiting the system throughput and increasing the transaction acceptance latency. The objective of this work is to increase the transaction throughput by introducing parallel transaction execution using a static analysis technique. We propose a framework DiPETrans for the distributed execution of the transactions in a block. Here, peers in the blockchain network form a community to execute the transactions and find the PoW parallelly, using a leader-follower approach. During mining, the leader statically analyzes the transactions, creates different groups (shards) of independent transactions, and distributes them to followers to execute them in parallel. After the transaction executes, the community's compute power is utilized to solve the PoW concurrently. When a block is successfully created, the leader broadcasts the proposed block to other peers in the network for validation. On receiving a block, validators re-execute the block transactions and accept the block if they reach the same state as shared by the miner. Validation can also be done as a community, in parallel, following the same leader-follower approach as mining. We report experiments using over 5 Million real transactions from the Ethereum blockchain and execute them using our DiPETrans framework to empirically validate the benefits of our techniques over traditional sequential execution. We achieve a maximum speedup of 2.2x for the miner and 2.0x for the validator, with 100 to 500 transactions per block. Further, we achieve a peak of 5x end-to-end block creation speedup using a parallel miner over a serial miner when using 6 machines in the community.

==> Arxiv on-13-3-2021/Backup-intro.tex <==
\section{Introduction}
\label{introduction}
According to a report published by World  Economic  Forum  (WEF)  based on a survey on the future of the blockchain technology predicted that $\approx10\%$ of the Global Gross Domestic Product (GDP) would be stored on the blockchain by $2025$ \cite{WEFBlockchains2017}. Furthermore, with an annual growth rate of $26.2\%$, the capital market of $\$2.5$ billion in 2016 may touch the $\$19.9$ billion by 2025 \cite{Zhang:2019arXiv190307602Z, CoinDesk}. Many well-known information technology vendors, governments across the world, Internet giants, and banks are investing in blockchain to accelerate research to make distributed ledger technology versatile \cite{Zhang:2019arXiv190307602Z}. \todo{This text looks like has been lifted from elsewhere.}
% (such as Microsoft, IBM, HSBC, Cisco, JPMorgan, Goldman Sachs, etc.)

%A blockchain can be defined as a distributed decentralized database which is tamper-proof, publicly accessible, highly secure, append-only, the permanent collection of the records organized in the chain of the blocks \cite{nakamoto2009bitcoin, Dickerson+:ACSC:PODC:2017,Vikram:DBLP:journals/corr/abs, Ethereum, Hyperledger}. It maintains a distributed global state of the transactions in the absence of a trusted central authority. An anonymous group or individual known as Satoshi Nakamoto was the first who introduced blockchain in a paper titled Bitcoin: a peer-to-peer electronic cash system in 2008 \cite{nakamoto2009bitcoin}. Since then, it is commonly believed that there is a possibility of becoming rich by mining coins \cite{bitcoin:faq:2019}. Both industries and academia are trying to generalize this technology to support different type of applications. However, it is still not matured enough and experiencing a lot of development.

A blockchain is a distributed decentralized database which is a secure, tamper-proof, publicly accessible collection of the records organized as a chain of the blocks \cite{nakamoto2009bitcoin, Dickerson+:ACSC:PODC:2017,Vikram:DBLP:journals/corr/abs, Ethereum, Hyperledger}. It maintains a distributed global state of the transactions in the absence of a trusted central authority. Due to its usefulness, it has gained wide interest both in industry and academia. 

A blockchain is a distributed system consisting of \emph{nodes} or \emph{peers} maintained in a peer-to-peer manner. Normally, the entire copy of the blockchain is stored on all the nodes of the system. \emph{Clients} external to the system use the services of the blockahins by sending requests to the nodes of the blockchain systems. 

%Bitcoin is an application specific distributed ledger technology.
Bitcoin \cite{nakamoto2009bitcoin}, the first blockchain system proposed (by Satoshi Nakamoto), is the most popular blockchain system till date. It is a cryptocurrency system which is highly secure where the users need not trust anyone. Further there is no central controlling agency like current day banking system. Ethereum \cite{Ethereum} is another popular blockchain currently in use and provides various other services apart from cryptocurrencies. As compared to Bitcoin \cite{nakamoto2009bitcoin}, Ethereum  provides support for user-defined programs (scripts), called \emph{smart contracts} \cite{Solidity} to offer complex services. 

%Bitcoin \cite{nakamoto2009bitcoin} is a highly secure, cryptocurrency system is the first public blockchain which is still highly popular. It processes the transactions in a distributed decentralized manner where a user need not to trust anyone, further there is no central controlling agency like current day banking system. Ethereum \cite{Ethereum} is another popular blockchain. As compared to Bitcoin \cite{nakamoto2009bitcoin}, Ethereum  provides support for user-defined programs (scripts), called \emph{smart contracts} \cite{Solidity} to offer complex services. 

Smart contracts in the Ethereum are written in Turing complete language Solidity \cite{Solidity}. These contracts automatically provide several complex services using pre-recorded terms and conditions in the contract without the intervention of a trusted third party. In general, a smart contract is like an object in object-oriented programming languages, which consists of methods and data (state) \cite{Dickerson+:ACSC:PODC:2017, Solidity}. A client request, aka transaction, consists of these methods and corresponding input parameters. A transaction can be initiated by a client (user) or a peer and executed by all the peers. 

A client wishing to the use the services of the blockchain, contacts a node of the system and send the request which is a transaction. A node $N_i$ on receiving several such transactions from different clients or other peers, forms a \emph{block} to be added to the blockchain. The node $N_i$ is said to be a \emph{\bp} and cryptocurrencies based blockchains such as Bitcoin, Ethereum, \bp{s} are called as \emph{miners} as they can `mine' new coins. In this document, we use these terms interchangeably. 

%Whenever a user sends a request, the corresponding method of the contract is called by the miner, and the contract state may change to the new state. In Ethereum, every account has its separate space to maintain state updates. Contracts are also yet another address on Ethereum and maintain separate space for modifications done via contract transactions \cite{Ethereum}.

%It executes the respective methods of the contract and changes the current state of the contract to the new state.
%It uses the cryptographic algorithm to encrypt everything and record them in the form of a chain of the blocks hence known as a blockchain.

%In the current implementation of most popular blockchain designs such as Bitcoin \cite{nakamoto2009bitcoin} and Ethereum \cite{Ethereum}, these transactions are executed in an ordered manner first by the miner later by the validators \cite{Dickerson+:ACSC:PODC:2017}. Basically, when a miner creates a block, miner is given a choice to pick the transactions based on its preference, for e.g., giving high priority to higher transactions fees, sequentially execute associated transactions, find the proof-of-work (PoW), and finally broadcast the block to other peers for validation to earn reward and append it to its local blockchain. The validation by other peers is also done sequentially in the same order as proposed by the miner to attain the consensus. Finally, after successful validation of a block by the majority (accepted by more than 50\%) of the peers/validators, the consensus is reached, and the miner gets the incentive for that block.

In most of the popular blockchain systems such as Bitcoin and Ethereum, transactions in a block are executed in an ordered manner first by the miners later by the validators \cite{Dickerson+:ACSC:PODC:2017}. When a miner creates a block, the miners typically chooses transactions to form a block from a pool based on their preference, e.g., giving higher priority to transaction with higher fees. After selecting the transactions the miner (1) serially executes the transactions, (2) adds the final state of the system to the block after execution, (3) next find the proof-of-work (PoW) \cite{PoW} and (4) broadcast the block in the network to other peers for validation to earn the reward. PoW is an answer to a mathematical puzzle in which a miner tries to find the hash of the block smaller than the given difficulty. This technique is used in the Bitcoin and Ethereum. 

Later after receiving a block, a node validates the contents of the block. Such a node is called the \emph{validator}. Thus when a node $N_i$ is \bp then every other node in the system acts as a validator. Similarly when another node $N_j$ is the miner then $N_i$ acts as a validator. The validators (1) re-execute the transactions in the block received serially, (2) verify to see if the final state computed by them is same as the final state provided by the miner in the block, and (3) also validates if the miner solved the puzzle (PoW) correctly. The transaction re-execution by the validators is done serially in the same order as proposed by the miner to attain the consensus \cite{Dickerson+:ACSC:PODC:2017}. After validation, if the block is accepted by the majority (accepted by more than 50\%) of the validators, then the block is added to the blockchain, and the miner gets the incentive (in case Bitcoin and Ethereum).% However, it is also possible that multiple blocks are proposed and added to the chain at the same time, which creates the fork in the chain; but, the longest chain is considered as the consistent one.

%Further, blockchain is designed such a way that every block which is added to the chain depends on the previous block's hash to force a chronological order. This ordering based on cryptographic hash makes it exponentially challenging to make any change to earlier transactions because this will requires recalculation of PoW of all the subsequent blocks and accepted by the majority of them. Also if two blocks are proposed at the same time and added to the blockchain, they form the fork, miners work on the first block they receive and switch to the longest chain of blocks as soon as the next block is formed. This allows mining to secure and maintain a global consensus based on processing power. If a miner can possess the majority of compute power, then theoretically can manipulate the transactions for its own gain \cite{BC-Mining}.

Further, blockchain is designed such a way that it forces a chronological order between the blocks. Every block which is added to the chain depends on the cryptographic hash of the previous block. This ordering based on cryptographic hash makes it exponentially challenging to make any change to the previous blocks. In order to make any small change to already accepted transactions or a block stored in the blockchain requires recalculation of PoW of all the subsequent blocks and acceptance by the majority of the peers in the network. Also, if two blocks are proposed at the same time and added to the chain, they form a \emph{fork}. To resolve the forks, the branch with the longest chain is considered as the final. This allows mining to be secure and maintain a global consensus based on processing power.

% Miners work on the first block they receive and switch to the longest chain. 

% If a miner can possess the majority of computing power, then theoretically can manipulate the transactions for its gain \cite{BC-Mining}.
% Forks are formed in the absence of a robust consensus protocol. 
%miners work on the first block they receive and switch to the longest chain. These allow mining to be secure and maintain a global consensus based on processing power.% If a


%The problem in the above approach is that both miners and validators sequentially execute the transactions and finds the PoW. Further finding the PoW is highly computation intensive. In the current era of distributed and multi-core system, the sequential execution of the transactions results in poor throughput.

%The problem in the above approach is that both miners and validators sequentially execute the transactions and finds the PoW. Further finding the PoW is highly computational intensive and require a lot of calculation to form a block. The PoW is required to delay wait for the network to reach consensus and avoid miners to waste energy on execution of transactions in their favour. The high computation requirements make it very difficult for a resource constraint miner to compete for the block creation process to get intensive. In the literature, there are several solutions proposed to mitigate this issue. One such solution is that several resource constraint miners form a pool (community) and determines the PoW and at the end after successful block creation shares the incentive among them. For sharing the incentive several solutions have been proposed in the literature and used in the Bitcoin mining pools \cite{qin18mining, lewenberg2015bitcoin, MiningPools:NBERw25592}. In the rest of the paper we will use mining pool and mining community interchangeably.

%In most of the blockchains, PoW \cite{PoW} is used to achieve the consensus by all the peers in the system to add new blocks to the blockchain. So it is a consensus protocol which is nothing but a mathematical computation introduced in Bitcoin and later adopted by various other cryptocurrency based blockchain platforms. Adding a new block to the blockchain by solving a mathematical puzzle is known as mining, and the peers of the network who do this task are known as miners. The PoW requires a considerable amount of work and computations to solve the puzzle. The puzzle is to get an answer to the problem in which miners have to run a very long random trial and error procedure. The miners continuously test different numbers (nonce) until they find a lower number smaller than the block hash (i.e., the header of the hashed block). This answer is also known as the target hash. Finding the target hash is a random process, which means that it can be solved in a single attempt or may not be after so many trials.


%In the current implementation of Bitcoin and Ethereum, throughput is very low, which leads to poor transaction acceptance rate. Further, poor transaction acceptance rate leads to poor user experience. A user does not wish to wait for a longer time for his transaction to be accepted, and they prefer the current centralized system over the blockchain based solution. In Bitcoin, less than seven transactions are accepted per second over 6K full nodes; on the other hand in Ethereum, only four transactions are processed per second instead of a theoretical maximum of 25 \cite{Mustafa:DBLP:journals/corr/abs-1708-03778}. 

\vspace{1mm}
\noindent
\textbf{Drawback with Existing System:} The drawback with the existing blockchain system is that miners and validators execute the transactions serially and so is computing the PoW. Further, finding the PoW \cite{PoW} is highly computationally intensive random process which requires a lot of computation to create a new block. PoW is required to delay-wait the network to reach consensus and allow miners to create a new block in their favor. But the problem is that the high computation requirements make it very difficult for a resource constraint miner to compete for the block creation to get intensive \cite{Eyal:BitcoinMiningVulnerable}.

Also, in the current era of distributed and multi-core system, sequential transaction execution results in poor throughput. Dickerson et al., \cite{Dickerson+:ACSC:PODC:2017} observed that the transactions are executed serially in two different contexts. First, they are executed serially by the miner while creating a block. Later, validator re-executes the transactions serially to validate the block. Serial execution of the transaction leads to poor throughput. Also, block transactions are executed several times by the miners and many many times by the validators.

In addition to these problems, due to the substantial high transaction fee, poor throughput (transactions/second), significant transaction acceptance latency, and limited computation capacities prevent widespread adoption \cite{eos:url, BC-Scalability}. Hence adding parallelism to the blockchain can achieve better efficiency and higher throughput.

\vspace{1mm}
\noindent
\textbf{Solution Approach - Mining Pools:} There are few solutions proposed and used in Bitcoin and Ethereum blockchain to mitigate these issues. One such solution is that several resource constraint miners form a pool (community) known as \emph{mining pool} and determines the PoW, and after block acceptance, they share the incentive among them \cite{Eyal:BitcoinMiningVulnerable, Eyal:MiningPool, qin18mining, lewenberg2015bitcoin, MiningPools:NBERw25592, Wiki:MiningPool, MiningPoolCentralized}. %For sharing the incentive, several solutions (proportional, pay-per-share, pay-per-last-N-shares) have been proposed in the literature and implemented by the mining pools.
In the rest of the paper, we use pool and community interchangeably.

Other solutions as proposed by \cite{Dickerson+:ACSC:PODC:2017, Vikram:DBLP:journals/corr/abs, Anjana:OptSC:PDP:2019, ZangandZang:ECSC:WBD:2018, Anjana:DBLP:journals/corr/abs} suggested concurrent execution of the transactions at runtime. In proposed techniques, the concurrent execution is done in two stages first while forming the block and second while validating the block. It helps in achieving better speed up also increase chances of a miner to receive rewards. However, it is not straight forward and requires a proper strategy so that a valid block should not be rejected due to false block rejection or FBR error \cite{Anjana:DBLP:journals/corr/abs}.

In this work, our objective is to execute the transactions parallelly based on statical analysis based technique using community (pool) of the trusted nodes along with finding the PoW parallelly to improve the performance. We proposed a framework for distributed parallel execution in a formal setting based on Ethereum \cite{Ethereum}. The core idea is to form a community of multiple trusted nodes and make use of the distributed compute power using a master-slave approach. In proposed approach different tasks (transactions) are assigned to different nodes of the community (as depicted in \emph{Fig. \ref{fig:arch}}), the nodes execute the independent transactions (different shards) in parallel. As far as our knowledge, this is the first work which focuses on statical analysis based parallel execution of the block transactions and combines the benefit associated with sharding and mining pools.

\vspace{-.48cm}
\begin{figure}[hb!]
\centering
	{\includegraphics[width=0.38\textwidth]{figs/Distributed_execution_V2.pdf}}
	\caption{Sharding of the Block Transactions}
	\label{fig:ds}
\end{figure}
\vspace{-.35cm}

As shown in \emph{Fig. \ref{fig:ds}}, all the dependent transactions are grouped into one shard and executed serially; however, the non-conflicting transactions belong to different shards executed parallelly by different workers. In \emph{Fig. \ref{fig:ds}}, transaction \emph{T$_1$} access the account (data item) \emph{A$_1$}, \emph{A$_3$}, transaction \emph{T$_5$} access account \emph{A$_1$}, \emph{A$_8$}, and transaction \emph{T$_7$} access \emph{A$_2$}, \emph{A$_3$}. Here it can be seen that \emph{T$_1$, T$_5$}, and \emph{T$_7$} are accessing common data items (accounts) hence grouped into the same shard (\emph{Shard$_{1}$}). Similarly transaction \emph{T$_2$, T$_3$}, and \emph{T$_9$} are grouped into \emph{Shard$_{2}$}, while \emph{T$_4$, T$_6$,} and \emph{T$_8$} are grouped in \emph{Shard$_{3}$}. Further, there is no dependency between the shards. Hence these shards can be executed parallelly by different nodes of the community. The proposed technique is based on the assumption that there is no nested call between the transactions (one contract internally call to another contract). In the presence of nested transaction calls, the technique will not work.

%\noindent
%\textit{Why distributed mining?}
%\par Managing the cluster (compute nodes connected via high-speed LAN) by the solo miner will require skill to manage and cost associated with deployment and maintenance. With the above approach, unskilled peers can form a community and can share resources to gain the reward proportional to their participation. This approach will give equal opportunity to every peer to participate in the mining to earn the reward.


%\vspace{-.45cm}
\noindent
%\textbf{Contributions:}
\emph{The \textbf{major contributions} of this work is as follows:}
\begin{itemize}
    \item We propose a framework \emph{DiPETrans} for parallel execution of the transactions at miner and validator based on transaction sharding using static analysis and mining pools. The novelty of this work is that it is the first contribution which combines the advantages associated with both sharding and mining pools.% based parallel execution.% The proposed technique allows computation constraint miner to participate in the mining to earn the rewards (intensive) and improve the overall throughput of the system.
    \item Once the miner proposes a block; the validator executes the transactions parallelly using the same approach followed by the miner.% However, the only difference is that validators do not determine PoW.% The validator executes the transactions parallelly and checks the final state computed by them matches with the final state of the block as computed by the miner, subsequently also confirms that the PoW is valid or not.
    \item We implemented two different approaches for the validator; in the first approach, the miner incorporates some information about the conflicting transactions (shards) in the block to help the validators to execute the block transactions deterministically parallelly. While in the second approach, the miner does not include dependency information in the block, and validator have to determine the dependencies.
    \item We experimented with actual transactions from the Ethereum blockchain and simulated the behavior of the proposed technique to prove the potential benefits over traditional sequential execution.% We also show the tradeoff between sharing information about dependencies in the block to the validators concerning not sharing the information.
    \item The proposed approach achieved maximum speedup of $2.18\times$ for miner, $2.02\times$ for \emph{no info sharing validator} and $2.04\times$ for \emph{info sharing validator} for 100 to 500 transactions per block with max 5 workers in the community. %this should not come as a contribution but is more of a result.
    %\item The proposed approach achieves linear speedup for overall block execution at miner using distributed execution of transaction and mining. We achieved \textit{xxxx}, \textit{yyyy}, and \textit{zzzz} speedup for \emph{miner, info sharing validator}, and \emph{no info sharing validator} respectively.
\end{itemize}

The rest of the paper is organized as follows: We present the related work and literature in \textit{Section \ref{relatedWork}}. While in \textit{Section \ref{methodology}}, we describe the proposed methodology, \emph{DiPETrans} architecture, and algorithms. \textit{Section \ref{experiment}} consist of the experimental evaluation and results. Finally, we conclude with some future research directions in \textit{Section \ref{conclusion}}.

%The rest of the paper is organised as follows: in \textit{Section \ref{relatedWork}} we present the related work. The proposed methodology, architecture, and algorithms are given in the \textit{Section \ref{methodology}}. While \textit{Section \ref{expriment}} consist of the experimental evaluation and results. Finally in the \textit{Section \ref{conclusion}} we will conclude with some future research directions.

%The rest of the paper is organised as follows: In \textit{Section \ref{relatedWork}}, we summarize the related literature. The proposed methodology, architecture, and algorithms are presented in the \textit{Section \ref{methodology}}. \textit{Section \ref{experiment}} consist of the experimental evaluation and results. Finally, at the end, we conclude with some future research directions in \textit{Section \ref{conclusion}}.

==> Arxiv on-13-3-2021/ap-algo.tex <==
\subsection{Proposed Algorithms}
\label{ap:rpa}
%This section describes the remaining proposed algorithm.

This section describes the proposed algorithms and a short description of them.

%\vspace{-.25cm}
\begin{algorithm}%[htb!]
%\footnotesize
  {
	\SetAlgoLined
	\KwData{ethereumData, followerList, dataItemMap}
	\KwResult{blockchain (blockList)}
	
	\SetKwFunction{FLeaderMinerTask}{LeaderMinerTask}
	\SetKwFunction{FLeaderValidator}{LeaderValidator}
	\SetKwFunction{FConnectFollower}{ConnectFollower}
	\SetKwFunction{FFollowerMineBlock}{FollowerMineBlock}
	\SetKwFunction{FProcessBlock}{ProcessBlock}
	\SetKwFunction{FCreateBlock}{CreateBlock}
	\SetKwFunction{FSendTxns}{SendTxns}
	\SetKwFunction{FFollowerRecvTxns}{FollowerRecvTxns}
	\SetKwFunction{FMineBlock}{MineBlock}
	\SetKwFunction{FMiningStatus}{MiningStatus}
	\SetKwFunction{FAnalyze}{Analyze}
	\SetKwFunction{FCallContract}{CallContract}
	
	\SetKwProg{Pn}{Procedure}{:}{\KwRet $blocklist$}
	\Pn{\FLeaderMinerTask {$ethereumData$}}{
		Block $block$\;
		\For{$data \in ethereumData$}{
		    \tcp{Creates candidate block}
		    
		    $block$ = \FCreateBlock{$data$}\;
		    
		    \If{$block.txnsList.size() > 0$}{
		        \tcp{Identify disjoint sets of txns (Weakly Connected Components)}
		        
		        $sendTxnsMap$ = \FAnalyze{$block.txnsList$}\;
		        
		        
		        \tcp{Parallel call to each follower to assign transactions}
		        
		        \For{$follower \in followerList$}{
		        	
		            \FConnectFollower{$follower$, $sendTxnsMap$}\;
		        }
		        \tcp{Wait till all follower execution completes}
		    }
		    \tcp{Start Block Mining}
		    
		    $miningStatus$ = $false$\;
		    
		    \For{$follower \in followerList$}{
		    	
		    \tcp{Parallel call to each Follower to mine block}
		    
	            \FFollowerMineBlock{$follower$, $block$}\;
	        }
		    \While{$!miningStatus$}{$wait()$\;}
		    
		    \tcp{Broadcast the block for validation to all other peers}% and after more than 51\% acceptance}
		    
		    $blockchain$.append($block$)\;
		    
		}
	}
	\caption{{LeaderMinerTask(ethereumData)}}
	\label{alg:mmt}
  }
\end{algorithm}
%\vspace{-.6cm}



%\vspace{-.51cm}



\noindent
\textbf{\emph{Algorithm}~\ref{alg:mmt}: \emph{LeaderMinerTask()} -- }
The \mMiner starts block creation by calling \emph{CreateBlock()} ({Algorithm~\ref{alg:cb}}). The candidate block consists of block number, nonce, previous hash, miner detail (coin base address), transaction list, etc. The \emph{Analyze()} (Algorithm~\ref{alg:analyze}) is used to analyzes the candidate block transactions for sharding. The leader receives a response \emph{sendTxnsMap} from \emph{Analyze()}, which consist a map of \emph{followerID} and transactions list. Each follower is allocated a unique id during the initialization of the leader server. Leader connects to the follower by creating parallel threads with a call to \emph{ConnectFollower()} ({Algorithm~\ref{alg:cw}}). The leader waits for the follower's to complete the transaction execution. So as soon as the leader receives the \emph{follower response (SResponse)}, it makes changes to its state in \emph{dataItemMap}.

After transaction execution, the leader starts mining (determine PoW) by setting \emph{miningStatus} to \emph{false}. For this leader distributes task among the followers to mine the block using asynchronous call to \emph{FollowerMineBlock()} ({Algorithm~\ref{alg:wmb}}). Leader calls each follower to mine from different starting nonce in sequence. In this way, search space is distributed among the followers for PoW calculation. The leader waits until the \emph{miningStatus} turned to be true by a follower. The follower who finds the correct PoW sends the information to the leader. Finally, the leader saves the nonce and broadcast the block in the network for validation. %Later leader restarts the whole process with a fresh set of pending transactions for next block creation.

%\ysnote{Note to self: Algorithm Analyze was present here.}







%\vspace{.08cm}
%\noindent
\textbf{\emph{Algorithm}~\ref{alg:mvnsi}: \emph{DefaultValidator()} -- }
When a validator receives a block for the validation, it re-executes the transactions. It then matches the final state of the \emph{dataItemMap} state. Since in this approach dependency (shard) information is not added to the block by the miner, the leader validator needs to call the \emph{Analyze()} to determine the disjoint sets of transactions. Then leader validator follows the same approach as the miner to distribute transactions to the follower and waits for all followers to complete. The leader validator does not have to mine the block. The leader validator updates its \emph{dataItemMap} state based on the responses from the followers. Finally, it verifies its \emph{dataItemMap} state with the block's \emph{dataItemMap} state. If \emph{dataItemMap} state matches after successful execution of block's transaction, then it checks for PoW by verifying $hash(block) < difficulty$. If both the checks come out to be successful, an acceptance message propagated in the network. Otherwise, the block is rejected by the validator, and no propagation can and cannot be entertained. After majority acceptance or consensus, the block is added to the \emph{blockchain}.
 
 


\begin{algorithm}%[htb!]
%\footnotesize
  {
	\SetAlgoLined
    \KwData{block}
	\KwResult{blocklist}
    \SetKwProg{Pn}{Procedure}{:}{\KwRet}
	\Pn{\FLeaderValidator{$block$}}{
	    \If{$block.txnsList.size() > 0$}{
	    	
	        \tcp{Identify disjoint sets of txns (Weakly Connected Components)}
	        
	        $sendTxnsMap$ = \FAnalyze{$block.txnsList$}\;
	        
	        \tcp{Parallel call to each follower to assign transactions}
	        
	        \For{$follower \in followerList$}{
	        	
	            \FConnectFollower{$follower$, $sendTxnsMap$}\;
	        }
	        \tcp{Wait till all follower execution completes}
	        
	        $reject$ = $false$\;
	        
	        \tcp{Verify PoW}
	        
	        \uIf{$hash(block) > difficulty$}{
	        	
	            \tcp{PoW is incorrect}
	            
	            $reject$ = $true$\;
	        }
	        \Else{
	        	
    	        \tcp{Verify dataItemMap with block's dataItemMap state.}
    	        
    	        \For{$adr, value \in block.dataItemMap$}{
    	        	
    	            \If{dataItemMap[adr] != value}{
    	            	
    	                $reject$ = $true$\;
    	                
    	                break\;
    	            }
    	        }
    	   }
	    }
	    \tcp{If Accepted than add to local blockchain}%51\% peers}
	    
	    \If{$!reject$}{
	    	
	        $blockchain$.append($block$)\;
	    } 
	}
	\caption{{LeaderValidator(block)}}
	\label{alg:mvnsi}
  }
\end{algorithm}




%\vspace{-0.8cm}
%\noindent
\textbf{\sval() -- }
In this function, sharding information is added to block by the miner, so the leader validators do not call the \emph{Analyze}() at \emph{line 3} in {Algorithm~\ref{alg:mvnsi}}. Therefore, the Analyze function's overhead can be avoided, and the validator utilizes the analysis work done by the miner for parallel execution. So, in the \sVal, the \mVal deterministically assigns the different shards based on the dependency information in the block to the different \wVal along with the current state of the data items from its local chain for transaction execution. The rest of the functionality of this algorithm is the same as \dVal.



%\noindent
\textbf{\emph{Algorithm} \ref{alg:cb}: \emph{CreateBlock()} -- }
In this function, the leader creates the candidate block by picking pending transactions from the pending transactions pool. Leader also assigns block number, previous hash, and miner (coin base address) to the block. There can be some uncles blocks, which are valid blocks and the miner who proposed that blocks deserve incentive for their work. If these blocks are added by the upcoming blocks ($<$ 8), also called nephew blocks, they are given partial incentives based on the Eqn \eqref{eq:neprew}. Some incentive based on the Eqn \eqref{eq:unrew} is also given to the miner who adds the uncle blocks. The maximum limit on the inclusion of uncle blocks is 2. %Eqn \eqref{eq:unrew} and \eqref{eq:neprew} are used to compute the rewards for the miner who added uncle and nephew node, respectively.

\begin{equation}   
    \label{eq:neprew}
    nephew Miner Reward = \frac{baseReward}{32}
\end{equation}

\begin{equation}
\label{eq:unrew}
    uncle Miner Reward = \frac{(uncleBlockNumber + 8 - nephewBlockNumber)*baseReward}{8}
\end{equation}




\begin{algorithm}%[!htb]
%\footnotesize
  {
	\SetAlgoLined
    \KwData{data, prevHash}
	\KwResult{block}
	\SetKwFunction{FLeaderMinerTask}{LeaderMinerTask}
	\SetKwFunction{FLeaderValidator}{LeaderValidator}
	\SetKwFunction{FConnectFollower}{ConnectFollower}
	\SetKwFunction{FFollowerMineBlock}{FollowerMineBlock}
	\SetKwFunction{FProcessBlock}{ProcessBlock}
	\SetKwFunction{FCreateBlock}{CreateBlock}
	\SetKwFunction{FSendTxns}{SendTxns}
	\SetKwFunction{FFollowerRecvTxns}{FollowerRecvTxns}
	\SetKwFunction{FMineBlock}{MineBlock}
	\SetKwFunction{FMiningStatus}{MiningStatus}
	\SetKwFunction{FAnalyze}{Analyze}
	\SetKwFunction{FCallContract}{CallContract}
    \SetKwProg{Pn}{Procedure}{:}{\KwRet $block$}
	\Pn{\FCreateBlock {$data$, $prevHash$}}{
	    Block $block$\;
	    block.number = data.number\;
	    
	    block.prevHash = prevHash\;
	    
	    block.miner = data.miner\;
	    
	    \tcp{creates candidate block}
	    
	    \For{$tx \in data.txns$}{
	    	
	        Transaction $txn$($tx.txID$, $tx.to$, $tx.from$, $tx.value$, $tx.input$, $tx.creates$)\;
	        
	        $block.txnsList$.append($txn$)\;
	    }
	    \For{$u \in data.uncles$}{
	    	
	        Uncle $unc$($u.number$,$u.miner$)\;
	        
	        $block.unclesList$.append($unc$)\;
	    }
	}
    \caption{{CreateBlock(data, prevHash)}}%:\emph{ this algorithm is used to creates the new block and populate required information. It is called by the \mMiner.}}}
    \label{alg:cb}
  }

\end{algorithm}



%\noindent
\textbf{\emph{Algorithm} \ref{alg:ms}: \emph{MiningStatus()} -- }
This function is called by a follower to send the block's nonce value to leader and signaling leader that mining has complete. In this function, follower checks for block number on which leader is working on with its block number and the \emph{miningStatus} not true. Then, the follower updates the nonce value of the block and set \emph{miningStatus} to true. As soon as leader notices change in \emph{miningStatus} variable and come out of the wait loop. Then starts working on the next block after sending the current block for its inclusion in blockchain and verification by validators.

\begin{algorithm}%[!htb]
%\footnotesize
  {
	\SetAlgoLined
    \KwData{block, nonce, number}
	\KwResult{miningStatus}
    \SetKwProg{Pn}{Procedure}{:}{\KwRet $miningStatus$}
    
	\Pn{\FMiningStatus{$block$, $nonce$, $number$}}{
		
        \If{$block.number == number$ \&\& $!miningStatus$}{
        	
            $block.nonce$ = $nonce$\;
            
            $miningStatus$ = $true$\;
        }
	}
	\caption{{MiningStatus(block, nonce, number)}}%: \emph{This function is called by one of the \wMiner to send the nonce value for the block to \mMiner and signaling \mMiner that mining has complete.}}}
	\label{alg:ms}
 }
\end{algorithm}


%\noindent
\textbf{\emph{Algorithm} \ref{alg:wmb}: \emph{FollowerMineBlock()} -- }
In this function, followers receive the starting nonce and interval along with the block to find the PoW. The PoW is found when $hash(block) < difficulty$ is found for a particular value of nonce. Otherwise, a nonce is incremented by interval to try again in an infinite loop. The difficulty we have set for now takes approximately 15 seconds to mine a block, close to the current average time of Ethereum block execution. The actual difficulty is much larger than what we are using, considering the resources deployed by miners to find PoW. 
\begin{algorithm}%[!htb]
%\footnotesize
  {
	\SetAlgoLined
    \KwData{block, nonce, interval, difficulty}
	\KwResult{nonce}
    \SetKwProg{Pn}{Procedure}{:}{\KwRet $nonce$}
    
	\Pn{\FFollowerMineBlock{$block$, $nonce$, $interval$, $difficulty$}}{
        \While{$true$}{
        	
            \If{$hash256(block) < difficulty$}{               
            	
            	\FMiningStatus{$nonce$,$block.number$}\;
            	
                break\;
            }
            $nonce$ += $interval$\;
        }
	}
	\caption{{FollowerMineBlock(block, nonce, interval, difficulty)}}%: \emph{this algorithm is called by \mMiner to assign starting  nonce  and  interval along with the block to the \wMiner to find the PoW for the block.}}}
	\label{alg:wmb}
  }
\end{algorithm}




%\vspace{.08cm}
%\noindent
\textbf{\emph{Algorithm} \ref{alg:cw}: \emph{ConnectFollower()} -- }
Leader calls \emph{ConnectFollower()} ({Algorithm~\ref{alg:cw}}) using parallel threads to assign different task to the followers. Here leader identifies each follower \emph{localDataItemMap} state from it's (leader's) \emph{dataItemMap} state based on the transactions a follower is going to execute. leader sends transaction list (shards) and associated \emph{dataItemMap} to each follower by calling \emph{FollowerRecvTxns()} ({Algorithm~\ref{alg:wrt}}). On this call follower executes the transactions while leader waits for the followers responses (\emph{SResponse}). The \emph{SResponse} is used to update the leader's \emph{dataItemMap}.% state.

\begin{algorithm}%[htb!]
%\footnotesize
  {
	\SetAlgoLined
    \KwData{follower, sendTxnsMap}
	\KwResult{dataItemMap}
    \SetKwProg{Pn}{Procedure}{:}{\KwRet $dataItemMap$}
    
	\Pn{\FConnectFollower{$follower$, $sendTxnsMap$}}{
		
        \tcp{Identify Associated dataItemMap for each follower}
        
        \For{$tx \in sendTxnsMap[SID]$}{
        	
            $localDataItemMap[tx]$ = $dataItemMap[tx]$ \;
        }
        \tcp{Send txns to follower to execute, receive updated state}
        
        $SResponse$ =  \FFollowerRecvTxns{$sendTxnsMap[Follower]$, $localDataItemMap$}\;
        
        \tcp{Update leader's dataItemMap state}
        
        \For{$ adr, dataItem \in SResponse.dataItemMap$}{
        	
            $dataItemMap[adr]$ = $dataItem$\;
        }
	}
	\caption{{ConnectFollower(follower, sendTxnsMap)}}
	\label{alg:cw}
  }
\end{algorithm}





\textbf{\emph{Algorithm} \ref{alg:wrt}: \emph{FollowerRecvTxns()} -- }
%While executing \emph{FollowerRecvTxns()}, the follower receives the transaction list and associated \emph{dataItemMap} state from the leader.This function internally called by Connectfollower(), which is called by the \mMiner to send the respective transaction list and current data item state to the individual \wMiner. This algorithm also distinguish between contract, and the non-smart contract calls considered as monetary exchanges.
%\vspace{.08cm}
%\noindent
%\textbf{\emph{FollowerRecvTxns()} -- }
While executing \emph{FollowerRecvTxns()} (i.e., {Algorithm~\ref{alg:wrt}}), the follower receives the transaction list and associated \emph{dataItemMap} state from the leader. The follower first identifies smart contract and non-smart contract calls (transactions). If the transaction is a smart contract call, then the transaction is executed by invoking \emph{CallContract()} to execute the respective smart contract method. Otherwise, non-smart contract calls are considered as monetary exchanges and executed within the scope of this function. For \emph{CallContract()} transaction execution, we have implemented the top 11 functions calls in Ethereum, which cover 80\% of real transactions of block numbers between 4370000 and 4450000.

%\vspace{-.5cm}
\begin{algorithm}%[htb!]
%\footnotesize
  {
	\SetAlgoLined
    \KwData{txnsList, dataItemMap}
	\KwResult{SResponse}
    \SetKwProg{Pn}{Procedure}{:}{\KwRet $SResponse$}
	\Pn{\FFollowerRecvTxns{$txnsList$, $dataItemMap$}}{
		
        \tcp{Execute txns serially}
        
        \For{$tx \in txnsList$}{
        	
            \tcp{Smart Contract txn}
            
            \uIf{$tx$ is $contractCall$}{
            	
                \FCallContract(tx)\;
                
            }
            \tcp{Non-Smart Contract txn}
            
            \uElseIf{$tx.value \leq dataItemMap$[$tx.from$].$value$}{
            
            $dataItemMap$[$tx.fromAddress$].$value$ -=  $tx.value$\;
            
            $dataItemMap$[$tx.toAddress$].$value$ += $tx.value$\;
            }
            \Else {
            	
                \tcp{Invalid txn: txn execution failed!}
            }
        }
	}
	\caption{{FollowerRecvTxns(txnsList, dataItemMap)}}
    \label{alg:wrt}
 }
\end{algorithm}




\begin{comment}

\textbf{\emph{Algorithm} \ref{alg:lb}: \emph{LoadBalance()} -- }
The number of shards created may exceed the number of followers. 
While executing the \emph{LoadBalance()} (i.e., {Algorithm~\ref{alg:lb}}), the leader receives the \emph{shardsMap}, \emph{followerList} and \emph{txnsList}. Here leader sorts the shards map in decreasing order of transaction count and assigns eachshard to the follower with the least number of transaction count. The information is saved in \emph{sendTxnsMap} which will be used to update the followers about the transactions to execute. In this way, we we attempt to load balance the number of transactions per follower.



\begin{algorithm}%[!htb]
%\footnotesize
  {
	%\SetAlgoLined
    \KwData{shardsMap, followerList, txnsList}
	\KwResult{sendTxnsMap}
	\SetKwFunction{FLeaderMinerTask}{LeaderMinerTask}
	\SetKwFunction{FLeaderValidator}{LeaderValidator}
	\SetKwFunction{FConnectFollower}{ConnectFollower}
	\SetKwFunction{FFollowerMineBlock}{FollowerMineBlock}
	\SetKwFunction{FProcessBlock}{ProcessBlock}
	\SetKwFunction{FCreateBlock}{CreateBlock}
	\SetKwFunction{FSendTxns}{SendTxns}
	\SetKwFunction{FFollowerRecvTxns}{FollowerRecvTxns}
	\SetKwFunction{FMineBlock}{MineBlock}
	\SetKwFunction{FMiningStatus}{MiningStatus}
	\SetKwFunction{FAnalyze}{Analyze}
	\SetKwFunction{FCallContract}{CallContract}
	\SetKwFunction{FLoadBalance}{LoadBalance}
    \SetKwProg{Pn}{Procedure}{:}{\KwRet $sendTxnsMap$}
    
	\Pn{\FLoadBalance({$shardsMap$, $followerList$, $txnsList$})}{
		
	    Map<int,List<Transaction>> $sendTxnsMap$ \;
	    
        \tcp{Sort the shards in decreasing order of transaction count}
        
        $shardMap$ = sorted($shardMap$, reverse=True)
        
        \For{$ccID \in shardMap$}{
            \tcp{Find the followerID which has least number of transactions and assign them the shard transactions}
            
            Map<int,List<Transaction>>::iterator $it1$, $it2$\;
            
            \For{$it1=sendTxnsMap.begin()\; it1!=sendTxnsMap.end()\; it1++$}{
            	
                \For{$it2=sendTxnsMap.begin()\; it2!=sendTxnsMap.end()\; it2++$}{
                	
                    \If{$it1->second.size() > it2->second.size()$}{
                    	
                        \tcp{Follower id with least number of transactions}
                        
                        $id$ = $it2->first$ - $1$;
                        
                        \tcp{Assignment of shard transactions}
                        
                        \For{$txid \in shardMap[ccID]$}{
                        	
                            sendTxnsMap[followerList[id].followerID].push\_back(txnsList[txid]\;
        	            }
                    }
                }
            }
        }
	}
    \caption{{LoadBalance(shardsMap, followerList, txnsList)}}%:\emph{ this algorithm is used to creates the new block and populate required information. It is called by the \mMiner.}}}
    \label{alg:lb}
  }

\end{algorithm}
\end{comment}

==> Arxiv on-13-3-2021/ap-background.tex <==
\subsection{Background}
\label{ap:back}

In most popular blockchain systems such as Bitcoin~\cite{nakamoto2009bitcoin} and Ethereum~\cite{Ethereum}, transactions in a block are executed in an ordered manner, first by the miners later by the validators~\cite{Dickerson+:ACSC:PODC:2017}. When a miner creates a block, it typically chooses transactions from a pending transaction queue based on their preference, e.g., giving higher priority to the transactions with higher fees. After selecting the transactions, the miner (1) serially executes the transactions, (2) adds the final state of the system to the block after execution, (3) next find the PoW, and (4) broadcast the block in the network to other peers for validation to earn the reward. PoW is an answer to a mathematical puzzle in which miners try to find the hash of the block smaller than the given difficulty.


Later after receiving a block, a node validates the contents of the block. Such a node is called the validator. Thus when a node $N_i$ is \bp, every other node in the system acts as a validator. Similarly, when another node $N_j$ is the miner, then $N_i$ acts as a validator. The validators (1) re-execute the transactions in the block received serially, (2) verify to see if the final state computed by them is the same as the final state provided by the miner in the block, and (3) also validates if the miner solved the puzzle (PoW) correctly. The transaction re-execution by the validators is done serially in the same order as proposed by the miner to attain the consensus~\cite{Dickerson+:ACSC:PODC:2017}. After validation, if the block is accepted by the majority (accepted by more than 50\%) of the validators, the block is added to the blockchain, and the miner gets the incentive (in the case of Bitcoin and Ethereum).



Further, blockchain is designed in such a way that it forces a chronological order between the blocks. Every block which is added to the chain depends on the cryptographic hash of the previous block. This ordering based on cryptographic hash makes it exponentially challenging to make any change to the previous blocks. To make any small change to already accepted transactions or a block stored in the blockchain requires recalculation of PoW of all subsequent blocks and acceptance by the majority of the peers. Also, if two blocks are proposed simultaneously and added to the chain, they form a \emph{fork}, the branch with the longest chain is considered the final. This allows mining to be secure and maintain a global consensus based on processing power.

\begin{comment}
As well, existing blockchain platforms calibrate the difficulty to keep the mean end-to-end block creation time within limits like in Bitcoin; the block is created every 10 minutes and every two weeks 2016 blocks. After every 2016 blocks, the difficulty is calibrated based on how much time is taken if it has taken more than two weeks, the difficulty is reduced otherwise increased also several other factors are also considered to change the difficulty. While in Ethereum blockchain, roughly every 10 to 19 seconds, a block is produced, so the difficulty is fixed accordingly. After every block creation, if mining time goes below 9 seconds, then \emph{Geth}, a multipurpose command line tool that runs Ethereum full node, tries to increase the difficulty. In case when the block creation difference is more than 20, Geth tries to reduce the mining difficulty of the system. In the proposed \emph{DiPETrans} framework throughout the experiments, we fixed the difficulty, and due to that reason with an increase in transaction per block increase in mining time can be observed.
\end{comment}

==> Arxiv on-13-3-2021/ap-rA2500.tex <==
\subsection{Results and Analysis when Number of Transaction Varies from 500 to 2500 per Block}
\label{ap:txv2500}
This section includes the experiment done on a varying number of transactions from 500 to 2500 per block. Similar to the earlier experiments, where transactions per block vary from 100 to 500, this experiment for {Workload-1} transactions varies from 500 to 2500. The speedup is averaged over varying the contract to monetary transaction ratio $\rho$ (i.e., from $\frac{1}{1}$ to $\frac{1}{16}$). In {Workload-2} $\rho$ varies from $\frac{1}{1}$ to $\frac{1}{16}$ while the number of transactions per block remains fixed to 2500. While in {Workload-3}, community size varies from 1 follower up to 5 followers, and the number of transactions per block remains fixed to 2500. In all the figures, serial execution served as a baseline.




%%%%%%%%%%%%%%%%%%%%%    Execution Time       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\vspace{-.8cm}
\begin{figure*}%[hbt!]
    \centering
     {\includegraphics[width=1\textwidth]{figs/FinalResults/W1/W1-ExeTime2500-v1.pdf}}\vspace{-.2cm}
    \caption{Workload 1: average transaction execution time by miner (omitting time to find PoW) and validator when transactions varies from 500 to 2500 per block.}
    \label{fig:W1:avg-txn2500}
\vspace{.35cm}
    \centering
     {\includegraphics[width=1\textwidth]{figs/FinalResults/W2/W2-ExeTime2500-v1.pdf}}\vspace{-.2cm}
    \caption{Workload 2: average transaction execution time by miner (omitting time to find PoW) and validator for 2500 transactions per block.}
    \label{fig:W2:avg-txn2500}
\vspace{.35cm}
    \centering
    {\includegraphics[width=1\textwidth]{figs/FinalResults/W3/W3-ExeTime2500-v1.pdf}}\vspace{-.2cm}
    \caption{Workload 3: average transaction execution time by miner (omitting time to find PoW) and validator for 2500 transactions per block.}
    \label{fig:W3:avg-txn2500}
\end{figure*}






\subsubsection{Transaction Execution Time Analysis}
\textbf{Workload-1: }{\figref{W1:avg-txn2500}} shows the average transaction execution time taken by the miner and validator. As shown in the {\figref{W1:avg-txn2500}(a), \ref{fig:W1:avg-txn2500}(b), and \ref{fig:W1:avg-txn2500}(c)} the time required to execute transactions per block increases as the number of transactions increases in a block. Also, the 1 follower performs worst due to the overhead of static analysis and communication with the leader. Other follower configurations from 2 to 5 are all the better than serial. The difference between \dVal and \sVal validators is that \dVal needs to run static analysis on block transactions before execution. The \dVal is supposed to take more time compared to \sVal. The experiment shows slight performance improvement for \sVal over \dVal as the execution time and is significant enough to see the difference.



\textbf{Workload-2: }In this workload, the number of transactions per block is fixed to 2500, while the the contract to monetary transaction ratio $\rho$ varies from $\frac{1}{1}$ to $\frac{1}{16}$. In {\figref{W2:avg-txn2500}(a), \ref{fig:W2:avg-txn2500}(b)}, and {\ref{fig:W2:avg-txn2500}(c)}, it can be seen that decreasing the number of contract transactions than monetary transaction per block the overall time required to execute transactions also decreases because contractual transaction includes the external calls. Further, it can be noticed that serial execution outperforms 1 follower configuration due to the static analysis and communication overhead associated with one follower configuration. Although, other configurations (2 to 5 followers in the community) outperform serial execution with the increases in the number of followers in the community. However, with the increase of monetary transactions in the block, serial execution started giving better performance because it may be because of communication dominates the transaction execution. In these figures, we can see that the time required to execute more transactions per block decreases as the number of contract transactions decreases. The parallel validator is always taking less time than serial, and we can also observe a significant gap as we increase the number of monetary transactions per block. The \sVal  achieved a slight improvement over \dVal infects very close to each other.




\textbf{Workload-3: }{\figref{W3:avg-txn2500}} shows the analysis for a fixed number of transactions (2500) per block with varying community size. Here we see how the transaction ratio in each block will have an impact on the performance. We can observe in {\figref{W3:avg-txn2500}(a), \ref{fig:W3:avg-txn2500}(b), and \ref{fig:W3:avg-txn2500}(c)} that 1 follower is performing worst due to the overhead of static analysis and communication with leader. Other follower configurations from 2 to 5 are all working better than serial, and execution time decreases as the number of followers increases. Also, the smaller the number of contractual transactions per block, the performance will be better, i.e., $\frac{1}{1}$ is taking higher time then $\frac{1}{2}$ and $\frac{1}{16}$ is taking least time among them since it consists of 16$\times$ more monetary transactions than contractual transactions in a block. We can see the slight performance difference in \sVal and \dVal.



%%%%%%%%%%%%%%%%%%%%%   Speedup       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[hbt!]
    \centering
     {\includegraphics[width=1\textwidth]{figs/FinalResults/W1/W1-Speedup2500-v1.pdf}}\vspace{-.2cm}
    \caption{Workload 1: average speedup by community miner (omitting time to find PoW) and validator for transaction execution when transactions varies from 500 to 2500 per block.}
    \label{fig:W1:avg-speed-up2500}
\vspace{.35cm}
     {\includegraphics[width=1\textwidth]{figs/FinalResults/W2/W2-Speedup2500-v1.pdf}}\vspace{-.2cm}
    \caption{Workload 2: average speedup by community miner (omitting time to find PoW) and validator for transaction execution for 2500 transactions per block.}
    \label{fig:W2:avg-speed-up2500}
\vspace{.35cm}
    \centering
     {\includegraphics[width=1\textwidth]{figs/FinalResults/W3/W3-Speedup2500-v1.pdf}}\vspace{-.2cm}
    \caption{Workload 3: average speedup by community miner (omitting time to find PoW) and validator for transaction execution for 2500 transactions per block.}
    \label{fig:W3:avg-speed-up2500}
\end{figure*}







\subsubsection{Speedup Analysis}
\textbf{Workload-1: }{\figref{W1:avg-speed-up2500}} shows the mean speedup obtained by the parallel miner (omitting time to find PoW) and validator over serial miner and validator. As shown in \figref{W1:avg-speed-up2500}, the mean speedup increases as the number of transactions per block increases but, the serial is outperforming 1 follower configuration of community-based parallel execution. This happens due to the static analysis and communication overhead associated with leader and one follower communicate with the leader. Other settings, i.e., 2 to 5 followers in the community, all achieving better speedup over serial. Also, there is a drop in speedup going from 500 to 1000, but then onwards, there is a steady increase in speedup. The \dVal and \sVal is outperforming over serial.

\textbf{Workload-2: }In this workload, we fixed the number of transactions per block to 2500. However, the the contract to monetary transaction ratio $\rho$ varies from $\frac{1}{1}$ to $\frac{1}{16}$, i.e., contractual to monetary transaction ratio varies. In {\figref{W2:avg-speed-up2500}(a), \ref{fig:W2:avg-speed-up2500}(b)}, and {\ref{fig:W2:avg-speed-up2500}(c)}, it can be observed that by varying the ratio of contractual to monetary transaction the overall speedup increase because contractual transaction drops with number of increase in monetary transaction per block. Further, we can observe that speedup increases till $\frac{1}{8}$ and then decreases if the further decrease in the number of contract transactions per block. There is a slight performance improvement in \sVal over \dVal. 



\textbf{Workload-3: }{\figref{W3:avg-speed-up2500}} shows that 1 follower is performing worst due to the overhead of static analysis and communication. Other follower configurations from 2 to 5 are all doing better than serial, and speedup increases as the number of followers increases. Also, the smaller the number of contractual transactions per block, the performance will be the better. As explained in the {Workload-2}, this is because of the external method call by the contractual transaction.

==> Arxiv on-13-3-2021/ap-rETE.tex <==
\subsection{End-to-end Block Creation Time}
\label{apn:betete}
This section presents the analysis for the end-to-end block creation time, including time to find PoW  at the miner for transaction varies from 100 to 500 in {Workload-1} while it is fixed to 500 in {Workload-2} and {Workload-3} however other parameters as data set and community size varies respectively.

\begin{figure}[htb!]
	\begin{minipage}{.44\textwidth}
		\centering
		\includegraphics[width=.93\textwidth]{figs/FinalResults/WithMining/EtETimeW3.pdf}
		%\vspace{-.27cm}
		\caption{Workload3: average end-to-end block creation time by miner including time to find PoW.}
		\label{fig:EtETimeW3}
	\end{minipage}
\qquad
	\begin{minipage}{.45\textwidth}
		\centering\vspace{.22cm}
		\includegraphics[width=.85\textwidth]{figs/FinalResults/WithMining/EtESpeedupW3.pdf}
		\caption{Workload3: average end-to-end block creation speedup by community miner over serial miner including time to find PoW.}
		\label{fig:EtESpeedupW3}
	\end{minipage}
\end{figure}


\subsubsection{Transaction Execution Time Analysis}
{\figref{EtETime}(a)} shows the line plots for mean end-to-end block creation time taken by the miner (including time to find PoW) for {Workload-1}. The overhead of static analysis and communication is negligible including time to find PoW. Here, all followers configuration are performing better than serial. Since the PoW is random nonce for which the hash of a block is less than the given difficulty, it can take a variable amount of time to find nonce. Also, the serial and follower configurations have a different order of transactions in the final block. Both blocks are correct as proposed by the miner and considered as the final order of transaction execution. It is possible that due to some outliers in serial execution resulted higher mean for the end-to-end time required to create a block as compared to 1 follower.  Another observation is that the time required to create block increases linearly as the number of transactions per block increases. Across the different number of transactions, the trend remains consistent with followers, the higher number of followers takes less time than the less number of followers.

For {Workload-2} results are shown in {\figref{EtETime}(b)}. The reason for serial and one follower for these plots remains the same as explained above. The time required to create block across different data sets varies and does not show any pattern based on a contract to monetary transactions ratio. Since it largely depends on the PoW search. With PoW, we are always guaranteeing that when the number of followers increases, it will take less time to create a block (including time to find PoW) than the serial.


Similarly, in {Workload-3} when the number of transactions per block is fixed to 500 and community size increases (i.e., followers in the community increases) the time taken to mine a block always takes lesser time than the serial and smaller size community. \figref{EtETimeW3} confirms this observation; however, it is challenging to claim about which data set is doing better over others, and the reason is that mining time dominates the transaction execution time.



\subsubsection{Speedup Analysis}
For {Workload-1} {\figref{EtESpeedup}(a)} shows the mean speedup achieved by parallel community-based miner over serial by the miner (including time to find PoW). Here, all followers configuration are achieving better speedup over serial. The observation here is that the speedup varies as the number of transactions per block increases. Across the different number of transactions, the trend remains consistent with followers, the higher number of followers gives higher speed up than the less number of followers. 

{\figref{EtESpeedup}(b)} shows the line plots for mean speedup achieved over serial by the parallel miner including time to find PoW for {Workload-2}. The time required to create block across different data sets varies and does not show any pattern based on transactions ratio (i.e., contractual : momentary transactions). Since it largely depends on the PoW search. With PoW, we are always guaranteeing that more number of followers gives higher speedup over serial including time to find PoW. In {Workload-3} the speedup increases with increase in the size of the community, but there are no fixed trained with varying transaction ratio.






==> Arxiv on-13-3-2021/ap-rResults500.tex <==
\subsection{Additional Results and Observation for Transaction Execution Time and Speedup}
\label{ap:bes}

This section presents the experimental analysis for transaction execution time for {Workload-3} and speedup achieved in transactions execution by parallel miner and validator over serial. First, we present the analysis for transaction execution time for {Workload-3}. Then we present the additional analysis for speedup on {Workload-1}, {Workload-2}, and {Workload-3}.



\subsubsection{Transaction Execution Time Analysis}
\textbf{Workload-3: }{\figref{W3:avg-txn}} shows the analysis for a fixed number of transactions (500) per block with varying community size. This workload is designed to see how the transaction ratio (contract call: monetary transaction) in each block will impact the performance. We can observe in {\figref{W3:avg-txn}(a), \ref{fig:W3:avg-txn}(b), and \ref{fig:W3:avg-txn}(c)} that 1 follower is performing worst due to the overhead of static analysis and communication with leader. Other follower configurations from 2 to 5 are all outperforming over serial, and execution time decreases as the number of followers increases. Also, the smaller the number of contractual transactions per block, the performance will be the better. This is because of the external method call by the contractual transaction. Similar to {Workload-1} and {Workload-2}, also there is no much performance difference in \sVal and \dVal.

\begin{figure*}
    \centering
     {\includegraphics[width=.95\textwidth]{figs/FinalResults/W3/W3-ExeTime-v1.pdf}}\vspace{-.2cm}
    \caption{Workload-3: average transaction execution time by miner (omitting time to find PoW) and validator.}
    \label{fig:W3:avg-txn}
\end{figure*}



\subsubsection{Speedup Analysis}
\label{subsec:sa}
Here we will present the result analysis for all three workloads based on speedup achieved by parallel miner and validator over serial miner and validator.

\textbf{Workload-1: }{\figref{W1:avg-speed-up}} shows the average transaction speedup achieved by the miner (omitting time to find PoW) and validator. As shown in the {\figref{W1:avg-speed-up}(a), \ref{fig:W1:avg-speed-up}(b), and \ref{fig:W1:avg-speed-up}(c)} the mean speedup increases as the number of transactions per block increases. Also, one follower is performing worst due to the small overhead of static analysis and communication with the leader. Other follower configurations from 2 to 5 are all working better than serial. %The reason for speedup can be the communication cost becomes smaller than the transaction execution time.
The difference between \dVal and \sVal is that \dVal needs to run static analysis on transactions present in a block before execution. The \dVal is supposed to take more time compared to \sVal. However, the experiment shows no significant benefits of information sharing. The time taken by the static analysis is comparatively very less than expected. However, when the number of transactions per block increases to a very large number in a block, it is expected that information sharing by the miner benefits the validators.


%\vspace{.08cm}
%\noindent
\textbf{Workload-2: }In {\figref{W2:avg-speed-up}(a), \ref{fig:W2:avg-speed-up}(b)}, and {\ref{fig:W2:avg-speed-up}(c)}, we can observe that when the number of contract transactions decreases per block, the overall speedup increases because contractual transaction includes the external contract method calls. Also, we can see that the speedup increases until $\frac{1}{4}$ (contract : monetary transactions) and decreases with a further decrease in the number of contract transactions per block. The experiment shows there is no significant time taken by analyzing function to gain some performance improvement over \sVal. Hence both \dVal and \sVal are performing almost same.



%\vspace{.08cm}
%\noindent
\textbf{Workload-3: }As we can see in all this {\figref{W3:avg-speed-up}(a), \ref{fig:W3:avg-speed-up}(b), and \ref{fig:W3:avg-speed-up}(c)} that 1 follower is performing worst due to the obvious reason of overhead of static analysis and communication with follower. Other follower configurations all outperforming over serial. Also, the smaller the number of contractual transactions per block, the performance will be the better. However, there is no much performance benefit due to information sharing with the validator. 

\begin{figure}
    \centering
     {\includegraphics[width=.95\textwidth]{figs/FinalResults/W3/W3-Speedup-v1.pdf}}\vspace{-.2cm}
    \caption{Workload-3: average speedup by miner (omitting time to find PoW) and validator for transaction execution.}
    \label{fig:W3:avg-speed-up}
\end{figure}

\begin{comment}
Below tables shows the respective numbers for the workloads. The summary of transactions in experiment workload are given in Table~\ref{tab:txn-sim} while Table \ref{tab:sc-calls} reports most frequent functions called by contract transactions. Table \ref{tab:W1:TxExe} and Table \ref{tab:W2-W3:TxExe} shows the transaction execution time while Table \ref{tab:W1:Speedup} and Table \ref{tab:W2-W3:Speedup} the respective speedup. Here, the block \emph{data-1-2-300} means $\rho = \frac{1}{2}$ is the ratio of contractual to monetary transactions per block while 300 is the total number of transactions in this block.

\iffalse
%\vspace{-.4cm}
\begin{table}[t!]
	\centering
	\caption{Summary of transactions in experiment workload}
	\vspace{-.2cm}
	\label{tab:txn-sim}
	\resizebox{.6\columnwidth}{!}{%
		\begin{tabular}{c|c|c|r|r|r}
			\hline % (\#Txns/Block)
			{\textbf{Block type}} & $\rho$ & \multicolumn{1}{p{1.1cm}|}{\textbf{\# Txns/ block}} & {\textbf{\# Blocks}} & \multicolumn{1}{p{1.7cm}|}{\textbf{$\sum$\# Contract txns}} & \multicolumn{1}{p{1.7cm}}{\textbf{$\sum$\# Non-con\-tract txns}}\\
			\hline
			\hline
			data-1-1-100 & \multirow{5}{*}{$\frac{1}{1}$} & $100$ & 3,880 & 193,959 & 194,000 \\
			data-1-1-200 &  & $200$ & 1,940 & 193,959 & 194,000 \\
			data-1-1-300 &  & $300$ & 1,294 & 193,959 & 194,100 \\
			data-1-1-400 &  & $400$ & 970 & 193,959 & 194,000 \\
			data-1-1-500 &  & $500$ & 776 & 193,959 & 194,000 \\
			\hline
			data-1-2-100 & \multirow{5}{*}{$\frac{1}{2}$} &  $100$  &5,705 & 193,959 & 376,530 \\
			data-1-2-200 &  & $200$ &2,895 & 193,959 & 385,035 \\
			data-1-2-300 &  & $300$ &1,940 & 193,959 & 388,000 \\
			data-1-2-400 &  & $400$ &1,448 & 193,959 & 385,168 \\
			data-1-2-500 &  & $500$ &1,162 & 193,959 & 386,946 \\
			\hline
			data-1-4-100 & \multirow{5}{*}{$\frac{1}{4}$} &  $100$  &9,698 & 193,959 & 775,840 \\
			data-1-4-200 &  & $200$ &4,849 & 193,959 & 775,840 \\
			data-1-4-300 &  & $300$ &3,233 & 193,959 & 775,840 \\
			data-1-4-400 &  & $400$ &2,425 & 193,959 & 776,000 \\
			data-1-4-500 &  & $500$ &1,940 & 193,959 & 776,000 \\
			\hline
			data-1-8-100 & \multirow{5}{*}{$\frac{1}{8}$} &  $100$  &16,164 & 193,959 & 1,422,432 \\
			data-1-8-200 &  & $200$ &8,434 & 193,959 & 1,492,818 \\
			data-1-8-300 &  & $300$ &5,705 & 193,959 & 1,517,530 \\
			data-1-8-400 &  & $400$ &4,311 & 193,959 & 1,530,405 \\
			data-1-8-500 &  & $500$ &3,464 & 193,959 & 1,538,016 \\
			\hline
			data-1-16-100 & \multirow{5}{*}{$\frac{1}{16}$} &  $100$  &32,327 & 193,959 & 3,038,738 \\
			data-1-16-200 &  & $200$ &16,164 & 193,959 & 3,038,832 \\
			data-1-16-300 &  & $300$ &10,776 & 193,959 & 3,038,832 \\
			data-1-16-400 &  & $400$ &8,082 & 193,959 & 3,038,832 \\
			data-1-16-500 &  & $500$ &6,466 & 193,959 & 3,039,020 \\
			\hline
		\end{tabular}
	}
%\end{table}

\vspace{.3cm}
%\begin{table}[t]
	\centering
	\caption{Most frequent functions called by contract transactions}
	\vspace{-.2cm}
	\label{tab:sc-calls}
	\resizebox{.6\columnwidth}{!}{%
		\begin{tabular}{r|l|c|p{2.2cm}|r|r}
			\hline
			{\textbf{\#}} &{\textbf{Function}} & {\textbf{Fn. Hash}} & {\textbf{Param. Types}} & {\textbf{\# Txns}} &  {\textbf{\%'ile}}\\
			\hline\hline
			1 & transfer & 0xa9059cbb & address, uint256 & 56,654 & 37.72 \\
			2 & approve & 0x095ea7b3 & address, uint256 & 11,799 & 45.58 \\
			3 & vote & 0x0121b93f & uint256 & 11,509 & 53.24 \\
			4 & submitTransaction & 0xc6427474 & address, uint256, bytes & 8,163 & 58.67 \\
			5 & issue & 0x867904b4 & address, uint256 & 5,723 & 62.49 \\
			6 & \_\_callback & 0x38bbfa50 & bytes32, string, bytes & 5,006 & 65.82 \\
			7 & playerRollDice & 0xdc6dd152 & uint256 & 4,997 & 69.15 \\
			8 & multisend & 0xad8733ca & address, address[], uint256[] & 4,822 & 72.36 \\
			9 & SmartAirdrop & 0xa8faf6f0 & - & 4,467 & 75.33 \\
			10 & PublicMine & 0x87ccccb3 & - & 4,157 & 78.10 \\
			11 & setGenesisAddress & 0x0d571742 & address, uint256, bytes & 3,119 & 80.17 \\
			\hline
		\end{tabular}
	}
\end{table}

\end{comment}

\begin{table}%[!htb]
	\centering
	\caption{Workload-1: average transaction execution time (ms) taken by miner (omitting time to find PoW) and validator.}\vspace{-.2cm}
	\label{tab:W1:TxExe}
    \resizebox{.8\columnwidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \hline
        \multicolumn{8}{c}{\textbf{Workload 1: Execution Time-Averaged Across Data Set}} \\ \hline
        \multicolumn{3}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Average Transaction\\Execution Time (ms)\end{tabular}}}} & \multicolumn{5}{c}{\textbf{\# Transactions/Block}} \\ \cline{4-8} 
        \multicolumn{3}{c|}{} & \textbf{100} & \textbf{200} & \textbf{300} & \textbf{400} & \textbf{500} \\ \hline\hline
            \multirow{17}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\\ \\\# Followers\end{tabular}}} & \multirow{2}{*}{\textbf{Serial}} & \textbf{Miner} & 209.178 & 259.680 & 333.517 & 485.548 & 652.948 \\ \cline{3-8} 
             &  & \textbf{Validator} & 209.178 & 259.680 & 333.517 & 485.548 & 652.948 \\ \cline{2-8} 
             & \multirow{3}{*}{\textbf{1 Follower}} & \textbf{Miner} & 214.934 & 338.606 & 449.450 & 560.487 & 670.041 \\ \cline{3-8} 
             &  & \textbf{Default Validator} & 222.632 & 345.584 & 455.267 & 564.490 & 673.896 \\ \cline{3-8} 
             &  & \textbf{Sharing Validator} & 222.769 & 345.301 & 454.884 & 564.661 & 673.295 \\ \cline{2-8} 
             & \multirow{3}{*}{\textbf{2 Follower}} & \textbf{Miner} & 163.906 & 239.518 & 304.819 & 372.045 & 435.397 \\ \cline{3-8} 
             &  & \textbf{Default Validator} & 175.435 & 250.367 & 315.849 & 384.773 & 449.132 \\ \cline{3-8} 
             &  & \textbf{Sharing Validator} & 175.397 & 250.078 & 315.076 & 383.825 & 447.844 \\ \cline{2-8} 
             & \multirow{3}{*}{\textbf{3 Follower}} & \textbf{Miner} & 145.597 & 202.979 & 255.478 & 305.016 & 352.256 \\ \cline{3-8} 
             &  & \textbf{Default Validator} & 159.253 & 218.479 & 270.447 & 320.623 & 365.106 \\ \cline{3-8} 
             &  & \textbf{Sharing Validator} & 159.765 & 218.633 & 269.393 & 319.897 & 363.379 \\ \cline{2-8} 
             & \multirow{3}{*}{\textbf{4 Follower}} & \textbf{Miner} & 138.346 & 188.285 & 231.101 & 272.976 & 314.880 \\ \cline{3-8} 
             &  & \textbf{Default Validator} & 154.815 & 204.332 & 248.875 & 289.148 & 332.949 \\ \cline{3-8} 
             &  & \textbf{Sharing Validator} & 154.416 & 203.515 & 247.842 & 287.508 & 331.248 \\ \cline{2-8} 
             & \multirow{3}{*}{\textbf{5 Follower}} & \textbf{Miner} & 137.786 & 181.983 & 219.573 & 255.971 & 292.882 \\ \cline{3-8} 
             &  & \textbf{Default Validator} & 153.819 & 198.089 & 236.746 & 273.503 & 316.972 \\ \cline{3-8} 
             &  & \textbf{Sharing Validator} & 155.583 & 196.923 & 235.712 & 270.301 & 314.148 \\ \hline
    \end{tabular}%
    }

\end{table}

%\vspace{.3cm}
\begin{table}%[t]
	\centering
	\caption{Workload-2: average transaction execution time (ms) taken by miner (omitting time to find PoW) and validator for fixed 500 transactions per block.}\vspace{-.2cm}
	\label{tab:W2-W3:TxExe}
    \resizebox{.9\columnwidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \hline
    \multicolumn{8}{c}{\textbf{Workload 2: for Fixed 500 Transactions/Block}} \\ \hline
    \multicolumn{3}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Average Transaction\\ Execution Time (ms)\end{tabular}}}} &
      \multicolumn{5}{c}{\textbf{Data Set (Contractual:non-Contractual Transactions)}} \\ \cline{4-8} 
      \multicolumn{3}{c|}{} &
      \multicolumn{1}{c|}{\textbf{$\frac{1}{1}$}} &
      \multicolumn{1}{c|}{\textbf{$\frac{1}{2}$}} &
      \multicolumn{1}{c|}{\textbf{$\frac{1}{4}$}} &
      \multicolumn{1}{c|}{\textbf{$\frac{1}{8}$}} &
      \multicolumn{1}{c}{\textbf{$\frac{1}{16}$}} \\ 
      \hline\hline
    \multirow{17}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\\\# Followers\end{tabular}}} &
      \multirow{2}{*}{\textbf{Serial}} &
      \textbf{Miner} & 899.501289 & 803.576592 & 745.571134 & 467.861432 & 348.230281 \\ \cline{3-8} 
     &                                    & \textbf{Validator}         & 899.501289 & 803.576592 & 745.571134 & 467.861432 & 348.230281 \\ \cline{2-8} 
     & \multirow{3}{*}{\textbf{1 Worker}} & \textbf{Miner}             & 903.435111 & 752.360205 & 643.277768 & 561.327611 & 489.805732 \\ \cline{3-8} 
     &                                    & \textbf{Default Validator} & 904.014969 & 752.002998 & 648.402244 & 568.376649 & 496.685453 \\ \cline{3-8} 
     &                                    & \textbf{Sharing Validator} & 903.007643 & 752.793573 & 647.327419 & 567.519549 & 495.828668 \\ \cline{2-8} 
     & \multirow{3}{*}{\textbf{2 Worker}} & \textbf{Miner}             & 588.783061 & 500.214417 & 416.558371 & 288.769832 & 314.299498 \\ \cline{3-8} 
     &                                    & \textbf{Default Validator} & 602.824561 & 509.827405 & 428.57958  & 375.175437 & 329.251927 \\ \cline{3-8} 
     &                                    & \textbf{Sharing Validator} & 602.51179  & 508.784815 & 428.126662 & 375.175437 & 327.188706 \\ \cline{2-8} 
     & \multirow{3}{*}{\textbf{3 Worker}} & \textbf{Miner}             & 476.161763 & 403.197954 & 339.777975 & 288.769832 & 253.374965 \\ \cline{3-8} 
     &                                    & \textbf{Default Validator} & 488.706527 & 417.246162 & 354.410015 & 300.69738  & 264.469156 \\ \cline{3-8} 
     &                                    & \textbf{Sharing Validator} & 487.988044 & 413.735028 & 353.356387 & 299.256845 & 262.558388 \\ \cline{2-8} 
     & \multirow{3}{*}{\textbf{4 Worker}} & \textbf{Miner}             & 431.591137 & 361.181846 & 299.185373 & 255.518217 & 226.925341 \\ \cline{3-8} 
     &                                    & \textbf{Default Validator} & 456.400858 & 377.23306  & 316.040787 & 268.870945 & 246.200944 \\ \cline{3-8} 
     &                                    & \textbf{Sharing Validator} & 459.72049  & 372.980863 & 314.459004 & 265.77754  & 243.299923 \\ \cline{2-8} 
     & \multirow{3}{*}{\textbf{5 Worker}} & \textbf{Miner}             & 403.518486 & 334.074014 & 278.474287 & 236.432035 & 211.909309 \\ \cline{3-8} 
     &                                    & \textbf{Default Validator} & 441.50758  & 350.673057 & 295.937754 & 263.881831 & 232.858487 \\ \cline{3-8} 
     &                                    & \textbf{Sharing Validator} & 437.904549 & 347.662261 & 293.810249 & 261.895526 & 229.464985 \\ \hline
    \end{tabular}%
    }
\end{table}

%\vspace{.3cm}
\begin{table}%[t]
	\centering
	\caption{Workload-1: average speedup by community miner (omitting time to find PoW) and validator.}\vspace{-.2cm}
	\label{tab:W1:Speedup}
    \resizebox{.7\columnwidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \hline
        \multicolumn{8}{c}{\textbf{Workload-1: Execution Time-Averaged Across Data Set}} \\ \hline
        \multicolumn{3}{c|}{\multirow{2}{*}{\textbf{Average Speedup}}} & \multicolumn{5}{c}{\textbf{\# Transactions/Block}} \\ \cline{4-8} 
        \multicolumn{3}{c|}{} & \textbf{100} & \textbf{200} & \textbf{300} & \textbf{400} & \textbf{500} \\ \hline \hline
            \multirow{17}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\\ \\ \# Followers\end{tabular}}} & \multirow{2}{*}{\textbf{Serial}} & \textbf{Miner} & 1 & 1 & 1 & 1 & 1 \\ \cline{3-8} 
             &  & \textbf{Validator} & 1 & 1 & 1 & 1 & 1 \\ \cline{2-8} 
             & \multirow{3}{*}{\textbf{1 Follower}} & \textbf{Miner} & 0.869 & 0.723 & 0.723 & 0.843 & 0.953 \\ \cline{3-8} 
             &  & \textbf{Default Validator} & 0.838 & 0.708 & 0.713 & 0.837 & 0.947 \\ \cline{3-8} 
             &  & \textbf{Sharing Validator} & 0.837 & 0.709 & 0.714 & 0.837 & 0.948 \\ \cline{2-8} 
             & \multirow{3}{*}{\textbf{2 Follower}} & \textbf{Miner} & 1.148 & 1.024 & 1.068 & 1.271 & 1.467 \\ \cline{3-8} 
             &  & \textbf{Default Validator} & 1.069 & 0.979 & 1.029 & 1.230 & 1.421 \\ \cline{3-8} 
             &  & \textbf{Sharing Validator} & 1.067 & 0.980 & 1.031 & 1.233 & 1.425 \\ \cline{2-8} 
             & \multirow{3}{*}{\textbf{3 Follower}} & \textbf{Miner} & 1.295 & 1.209 & 1.273 & 1.550 & 1.813 \\ \cline{3-8} 
             &  & \textbf{Default Validator} & 1.179 & 1.121 & 1.200 & 1.475 & 1.747 \\ \cline{3-8} 
             &  & \textbf{Sharing Validator} & 1.174 & 1.119 & 1.205 & 1.479 & 1.755 \\ \cline{2-8} 
             & \multirow{3}{*}{\textbf{4 Follower}} & \textbf{Miner} & 1.371 & 1.303 & 1.406 & 1.734 & 2.032 \\ \cline{3-8} 
             &  & \textbf{Default Validator} & 1.217 & 1.198 & 1.305 & 1.636 & 1.921 \\ \cline{3-8} 
             &  & \textbf{Sharing Validator} & 1.220 & 1.202 & 1.311 & 1.648 & 1.933 \\ \cline{2-8} 
             & \multirow{3}{*}{\textbf{5 Follower}} & \textbf{Miner} & 1.388 & 1.350 & 1.478 & 1.848 & 2.185 \\ \cline{3-8} 
             &  & \textbf{Default Validator} & 1.249 & 1.237 & 1.370 & 1.728 & 2.022 \\ \cline{3-8} 
             &  & \textbf{Sharing Validator} & 1.244 & 1.243 & 1.376 & 1.747 & 2.040 \\ \hline
    \end{tabular}%
    }
\end{table}

%\vspace{.2cm}
\begin{table}%[t]
	\centering
	\caption{Workload-2: average speedup by community miner (omitting time to find PoW) and validator.}\vspace{-.2cm}
	\label{tab:W2-W3:Speedup}
    \resizebox{.7\textwidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \hline
        \multicolumn{8}{c}{\textbf{Workload-2: for Fixed 500 Transactions/Block}} \\ \hline
        \multicolumn{3}{c|}{\multirow{2}{*}{\textbf{Average Speedup}}} & \multicolumn{5}{c}{\textbf{Data Set (Contractual:Monetary Trans.)}} \\ \cline{4-8} 
        \multicolumn{3}{c|}{} & \textbf{$\frac{1}{1}$} & \textbf{$\frac{1}{2}$} & \textbf{$\frac{1}{4}$} & \textbf{$\frac{1}{8}$} & \textbf{$\frac{1}{16}$} \\ \hline\hline
            \multirow{17}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\\ \\ \# Followers\end{tabular}}} & \multirow{2}{*}{\textbf{Serial}} & \textbf{Miner} & 1 & 1 & 1 & 1 & 1 \\ \cline{3-8} 
             &  & \textbf{Validator} & 1 & 1 & 1 & 1 & 1 \\ \cline{2-8} 
             & \multirow{3}{*}{\textbf{1 Follower}} & \textbf{Miner} & 0.995 & 1.067 & 1.158 & 0.832 & 0.710 \\ \cline{3-8} 
             &  & \textbf{Default Validator} & 0.994 & 1.068 & 1.149 & 0.822 & 0.701 \\ \cline{3-8} 
             &  & \textbf{Sharing Validator} & 0.996 & 1.067 & 1.151 & 0.823 & 0.702 \\ \cline{2-8} 
             & \multirow{3}{*}{\textbf{2 Follower}} & \textbf{Miner} & 1.527 & 1.605 & 1.788 & 1.308 & 1.107 \\ \cline{3-8} 
             &  & \textbf{Default Validator} & 1.491 & 1.575 & 1.738 & 1.245 & 1.057 \\ \cline{3-8} 
             &  & \textbf{Sharing Validator} & 1.492 & 1.578 & 1.740 & 1.253 & 1.064 \\ \cline{2-8} 
             & \multirow{3}{*}{\textbf{3 Follower}} & \textbf{Miner} & 1.888 & 1.992 & 2.193 & 1.617 & 1.373 \\ \cline{3-8} 
             &  & \textbf{Default Validator} & 1.840 & 1.925 & 2.102 & 1.553 & 1.316 \\ \cline{3-8} 
             &  & \textbf{Sharing Validator} & 1.842 & 1.941 & 2.108 & 1.561 & 1.325 \\ \cline{2-8} 
             & \multirow{3}{*}{\textbf{4 Follower}} & \textbf{Miner} & 2.083 & 2.223 & 2.490 & 1.828 & 1.534 \\ \cline{3-8} 
             &  & \textbf{Default Validator} & 1.970 & 2.129 & 2.357 & 1.737 & 1.413 \\ \cline{3-8} 
             &  & \textbf{Sharing Validator} & 1.956 & 2.153 & 2.369 & 1.757 & 1.430 \\ \cline{2-8} 
             & \multirow{3}{*}{\textbf{5 Follower}} & \textbf{Miner} & 2.228 & 2.404 & 2.675 & 1.975 & 1.642 \\ \cline{3-8} 
             &  & \textbf{Default Validator} & 2.036 & 2.290 & 2.517 & 1.770 & 1.494 \\ \cline{3-8} 
             &  & \textbf{Sharing Validator} & 2.053 & 2.310 & 2.536 & 1.783 & 1.517 \\ \hline
    \end{tabular}%
    }
\end{table}


\begin{comment}

\vspace{.2cm}
\begin{minipage}[b]{.49\textwidth}
\centering
\captionof{table}{Workload-1: average transaction execution time (ms) taken by miner (omitting time to find PoW) and validator.}\vspace{-.2cm}
\label{tab:W1:TxExe}
\resizebox{.93\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
\multicolumn{8}{c}{\textbf{Workload 1: Execution Time-Averaged Across Data Set}} \\ \hline
\multicolumn{3}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Average Transaction\\Execution Time (ms)\end{tabular}}}} & \multicolumn{5}{c}{\textbf{\# Transactions/Block}} \\ \cline{4-8} 
\multicolumn{3}{c|}{} & \textbf{100} & \textbf{200} & \textbf{300} & \textbf{400} & \textbf{500} \\ \hline\hline
\multirow{17}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\\ \\\# Followers\end{tabular}}} & \multirow{2}{*}{\textbf{Serial}} & \textbf{Miner} & 209.178 & 259.680 & 333.517 & 485.548 & 652.948 \\ \cline{3-8} 
&  & \textbf{Validator} & 209.178 & 259.680 & 333.517 & 485.548 & 652.948 \\ \cline{2-8} 
& \multirow{3}{*}{\textbf{1 Follower}} & \textbf{Miner} & 214.934 & 338.606 & 449.450 & 560.487 & 670.041 \\ \cline{3-8} 
&  & \textbf{Default Validator} & 222.632 & 345.584 & 455.267 & 564.490 & 673.896 \\ \cline{3-8} 
&  & \textbf{Sharing Validator} & 222.769 & 345.301 & 454.884 & 564.661 & 673.295 \\ \cline{2-8} 
& \multirow{3}{*}{\textbf{2 Follower}} & \textbf{Miner} & 163.906 & 239.518 & 304.819 & 372.045 & 435.397 \\ \cline{3-8} 
&  & \textbf{Default Validator} & 175.435 & 250.367 & 315.849 & 384.773 & 449.132 \\ \cline{3-8} 
&  & \textbf{Sharing Validator} & 175.397 & 250.078 & 315.076 & 383.825 & 447.844 \\ \cline{2-8} 
& \multirow{3}{*}{\textbf{3 Follower}} & \textbf{Miner} & 145.597 & 202.979 & 255.478 & 305.016 & 352.256 \\ \cline{3-8} 
&  & \textbf{Default Validator} & 159.253 & 218.479 & 270.447 & 320.623 & 365.106 \\ \cline{3-8} 
&  & \textbf{Sharing Validator} & 159.765 & 218.633 & 269.393 & 319.897 & 363.379 \\ \cline{2-8} 
& \multirow{3}{*}{\textbf{4 Follower}} & \textbf{Miner} & 138.346 & 188.285 & 231.101 & 272.976 & 314.880 \\ \cline{3-8} 
&  & \textbf{Default Validator} & 154.815 & 204.332 & 248.875 & 289.148 & 332.949 \\ \cline{3-8} 
&  & \textbf{Sharing Validator} & 154.416 & 203.515 & 247.842 & 287.508 & 331.248 \\ \cline{2-8} 
& \multirow{3}{*}{\textbf{5 Follower}} & \textbf{Miner} & 137.786 & 181.983 & 219.573 & 255.971 & 292.882 \\ \cline{3-8} 
&  & \textbf{Default Validator} & 153.819 & 198.089 & 236.746 & 273.503 & 316.972 \\ \cline{3-8} 
&  & \textbf{Sharing Validator} & 155.583 & 196.923 & 235.712 & 270.301 & 314.148 \\ \hline
\end{tabular}%
}
\end{minipage}\qquad
\begin{minipage}[b]{.5\textwidth}
\captionof{table}{Workload-2: average transaction execution time (ms) taken by miner (omitting time to find PoW) and validator for fixed 500 transactions per block.}\vspace{-.2cm}
\label{tab:W2-W3:TxExe}
\resizebox{1.03\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
\multicolumn{8}{c}{\textbf{Workload 2: for Fixed 500 Transactions/Block}} \\ \hline
\multicolumn{3}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Average Transaction\\ Execution Time (ms)\end{tabular}}}} &
\multicolumn{5}{c}{\textbf{Data Set (Contractual:non-Contractual Transactions)}} \\ \cline{4-8} 
\multicolumn{3}{c|}{} &
\multicolumn{1}{c|}{\textbf{$\frac{1}{1}$}} &
\multicolumn{1}{c|}{\textbf{$\frac{1}{2}$}} &
\multicolumn{1}{c|}{\textbf{$\frac{1}{4}$}} &
\multicolumn{1}{c|}{\textbf{$\frac{1}{8}$}} &
\multicolumn{1}{c}{\textbf{$\frac{1}{16}$}} \\ 
\hline\hline
\multirow{17}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\\\# Followers\end{tabular}}} &
\multirow{2}{*}{\textbf{Serial}} &
\textbf{Miner} & 899.501289 & 803.576592 & 745.571134 & 467.861432 & 348.230281 \\ \cline{3-8} 
&                                    & \textbf{Validator}         & 899.501289 & 803.576592 & 745.571134 & 467.861432 & 348.230281 \\ \cline{2-8} 
& \multirow{3}{*}{\textbf{1 Worker}} & \textbf{Miner}             & 903.435111 & 752.360205 & 643.277768 & 561.327611 & 489.805732 \\ \cline{3-8} 
&                                    & \textbf{Default Validator} & 904.014969 & 752.002998 & 648.402244 & 568.376649 & 496.685453 \\ \cline{3-8} 
&                                    & \textbf{Sharing Validator} & 903.007643 & 752.793573 & 647.327419 & 567.519549 & 495.828668 \\ \cline{2-8} 
& \multirow{3}{*}{\textbf{2 Worker}} & \textbf{Miner}             & 588.783061 & 500.214417 & 416.558371 & 288.769832 & 314.299498 \\ \cline{3-8} 
&                                    & \textbf{Default Validator} & 602.824561 & 509.827405 & 428.57958  & 375.175437 & 329.251927 \\ \cline{3-8} 
&                                    & \textbf{Sharing Validator} & 602.51179  & 508.784815 & 428.126662 & 375.175437 & 327.188706 \\ \cline{2-8} 
& \multirow{3}{*}{\textbf{3 Worker}} & \textbf{Miner}             & 476.161763 & 403.197954 & 339.777975 & 288.769832 & 253.374965 \\ \cline{3-8} 
&                                    & \textbf{Default Validator} & 488.706527 & 417.246162 & 354.410015 & 300.69738  & 264.469156 \\ \cline{3-8} 
&                                    & \textbf{Sharing Validator} & 487.988044 & 413.735028 & 353.356387 & 299.256845 & 262.558388 \\ \cline{2-8} 
& \multirow{3}{*}{\textbf{4 Worker}} & \textbf{Miner}             & 431.591137 & 361.181846 & 299.185373 & 255.518217 & 226.925341 \\ \cline{3-8} 
&                                    & \textbf{Default Validator} & 456.400858 & 377.23306  & 316.040787 & 268.870945 & 246.200944 \\ \cline{3-8} 
&                                    & \textbf{Sharing Validator} & 459.72049  & 372.980863 & 314.459004 & 265.77754  & 243.299923 \\ \cline{2-8} 
& \multirow{3}{*}{\textbf{5 Worker}} & \textbf{Miner}             & 403.518486 & 334.074014 & 278.474287 & 236.432035 & 211.909309 \\ \cline{3-8} 
&                                    & \textbf{Default Validator} & 441.50758  & 350.673057 & 295.937754 & 263.881831 & 232.858487 \\ \cline{3-8} 
&                                    & \textbf{Sharing Validator} & 437.904549 & 347.662261 & 293.810249 & 261.895526 & 229.464985 \\ \hline
\end{tabular}%
}

\end{minipage}

\end{comment}

\begin{comment}
\begin{table}[!htb]
\centering
\caption{Workload-3: average transaction execution time (ms) taken by miner (omitting time to find PoW) and validator for fixed 500 transactions per block.}\vspace{-.25cm}
\label{tab:W3:TxExe}
    \resizebox{.6\columnwidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \hline
        \multicolumn{8}{c}{\textbf{Workload-2 and Workload-3: for Fixed 500 Transactions/Block}} \\ \hline
        \multicolumn{3}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Average Transaction\\ Execution Time (ms)\end{tabular}}}} & \multicolumn{5}{c}{\textbf{Data Set (Contractual:Monetary Transactions)}} \\ \cline{4-8} 
        \multicolumn{3}{c|}{} & \textbf{$\frac{1}{1}$} & \textbf{$\frac{1}{2}$} & \textbf{$\frac{1}{4}$} & \textbf{$\frac{1}{8}$} & \textbf{$\frac{1}{16}$} \\ \hline\hline
            \multirow{17}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\\ \\\# Followers\end{tabular}}} & \multirow{2}{*}{\textbf{Serial}} & \textbf{Miner} & 899.501 & 803.577 & 745.571 & 467.861 & 348.230 \\ \cline{3-8} 
             &  & \textbf{Validator} & 899.501 & 803.577 & 745.571 & 467.861 & 348.230 \\ \cline{2-8} 
             & \multirow{3}{*}{\textbf{1 Follower}} & \textbf{Miner} & 903.435 & 752.360 & 643.278 & 561.328 & 489.806 \\ \cline{3-8} 
             &  & \textbf{Default Validator} & 904.015 & 752.003 & 648.402 & 568.377 & 496.685 \\ \cline{3-8} 
             &  & \textbf{Sharing Validator} & 903.008 & 752.794 & 647.327 & 567.520 & 495.829 \\ \cline{2-8} 
             & \multirow{3}{*}{\textbf{2 Follower}} & \textbf{Miner} & 588.783 & 500.214 & 416.558 & 357.128 & 314.299 \\ \cline{3-8} 
             &  & \textbf{Default Validator} & 602.825 & 509.827 & 428.580 & 375.175 & 329.252 \\ \cline{3-8} 
             &  & \textbf{Sharing Validator} & 602.512 & 508.785 & 428.127 & 372.610 & 327.189 \\ \cline{2-8} 
             & \multirow{3}{*}{\textbf{3 Follower}} & \textbf{Miner} & 476.162 & 403.198 & 339.778 & 288.770 & 253.375 \\ \cline{3-8} 
             &  & \textbf{Default Validator} & 488.707 & 417.246 & 354.410 & 300.697 & 264.469 \\ \cline{3-8} 
             &  & \textbf{Sharing Validator} & 487.988 & 413.735 & 353.356 & 299.257 & 262.558 \\ \cline{2-8} 
             & \multirow{3}{*}{\textbf{4 Follower}} & \textbf{Miner} & 431.591 & 361.182 & 299.185 & 255.518 & 226.925 \\ \cline{3-8} 
             &  & \textbf{Default Validator} & 456.401 & 377.233 & 316.041 & 268.871 & 246.201 \\ \cline{3-8} 
             &  & \textbf{Sharing Validator} & 459.720 & 372.981 & 314.459 & 265.778 & 243.300 \\ \cline{2-8} 
             & \multirow{3}{*}{\textbf{5 Follower}} & \textbf{Miner} & 403.518 & 334.074 & 278.474 & 236.432 & 211.909 \\ \cline{3-8} 
             &  & \textbf{Default Validator} & 441.508 & 350.673 & 295.938 & 263.882 & 232.858 \\ \cline{3-8} 
             &  & \textbf{Sharing Validator} & 437.905 & 347.662 & 293.810 & 261.896 & 229.465 \\ \hline
        \end{tabular}%
    }
\end{table}

\end{comment}


==> Arxiv on-13-3-2021/ap-summryEthTx.tex <==
\subsection{Summary of Ethereum Transaction Data}
\label{apn:SETD}
This section presents the data set designed for the experiment using transactions extracted from Ethereum blockchain and smart contract calls implemented in \emph{C++} as given in the \emph{Table \ref{tab:txn-sim} and Table \ref{tab:sc-calls}}. In the \emph{Table \ref{tab:txn-sim}} \emph{data-1-1-100} represents that 1:1 is the ratio of contractual : monetary transactions per block while 100 is the total number of transactions per block. 


%\vspace{-.4cm}
\begin{table}[ht!]
    \centering
    \caption{Summary of Simulated Transactions Data}\vspace{-.3cm}
    \label{tab:txn-sim}
    \resizebox{0.45\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        \emph{\textbf{S. No.}} & \emph{\textbf{Data (\#Txns/Block)}} & \emph{\textbf{\#Blocks}} & \emph{\textbf{\#Contract\_Txns}} & \emph{\textbf{\#Non\_Contract\_Txns}}\\
        \hline
        1 & data-1-1-100 & 3,880 & 193,959 & 194,000 \\
		2 & data-1-1-200 & 1,940 & 193,959 & 194,000 \\
        3 & data-1-1-300 & 1,294 & 193,959 & 194,100 \\
        4 & data-1-1-400 & 970 & 193,959 & 194,000 \\
        5 & data-1-1-500 & 776 & 193,959 & 194,000 \\
        \hline
        6 & data-1-2-100 & 5,705 & 193,959 & 376,530 \\
        7 & data-1-2-200 & 2,895 & 193,959 & 385,035 \\
        8 & data-1-2-300 & 1,940 & 193,959 & 388,000 \\
        9 & data-1-2-400 & 1,448 & 193,959 & 385,168 \\
        10 & data-1-2-500 & 1,162 & 193,959 & 386,946 \\
        \hline
        11 & data-1-4-100 & 9,698 & 193,959 & 775,840 \\
		12 & data-1-4-200 & 4,849 & 193,959 & 775,840 \\
        13 & data-1-4-300 & 3,233 & 193,959 & 775,840 \\
        14 & data-1-4-400 & 2,425 & 193,959 & 776,000 \\
        15 & data-1-4-500 & 1,940 & 193,959 & 776,000 \\
        \hline
        16 & data-1-8-100 & 16,164 & 193,959 & 1,422,432 \\
        17 & data-1-8-200 & 8,434 & 193,959 & 1,492,818 \\
        18 & data-1-8-300 & 5,705 & 193,959 & 1,517,530 \\
        19 & data-1-8-400 & 4,311 & 193,959 & 1,530,405 \\
        20 & data-1-8-500 & 3,464 & 193,959 & 1,538,016 \\
        \hline
        21 & data-1-16-100 & 32,327 & 193,959 & 3,038,738 \\
		22 & data-1-16-200 & 16,164 & 193,959 & 3,038,832 \\
        23 & data-1-16-300 & 10,776 & 193,959 & 3,038,832 \\
        24 & data-1-16-400 & 8,082 & 193,959 & 3,038,832 \\
        25 & data-1-16-500 & 6,466 & 193,959 & 3,039,020 \\
        \hline
    \end{tabular}
    }
\end{table}


%\vspace{-.2cm}
\begin{table}[ht!]
    \centering
    \caption{Summary of Contract Transactions Calls}
    \vspace{-.3cm}
    \label{tab:sc-calls}
    \resizebox{.49\textwidth}{!}{%
    \begin{tabular}{|c|p{2.5cm}|p{1.63cm}|p{3.3cm}|p{.9cm}|c|}
        \hline
        \emph{\textbf{S.No.}} &\emph{\textbf{Fn Name}} & \emph{\textbf{Fn Hash}} & \emph{\textbf{Parameters}} & \emph{\textbf{\#Txns}} &  \emph{\textbf{Percentile}}\\
        \hline
        1 & transfer & 0xa9059cbb & address, uint256 & 56,654 & 37.72 \\
        2 & approve & 0x095ea7b3 & address, uint256 & 11,799 & 45.58 \\
        3 & vote & 0x0121b93f & uint256 & 11,509 & 53.24 \\
        4 & submitTransaction & 0xc6427474 & address, uint256,bytes & 8,163 & 58.67 \\
        5 & issue & 0x867904b4 & address,uint256 & 5,723 & 62.49 \\
        6 & \_\_callback & 0x38bbfa50 & bytes32, string, bytes & 5,006 & 65.82 \\
        7 & playerRollDice & 0xdc6dd152 & uint256 & 4,997 & 69.15 \\
        8 & multisend & 0xad8733ca & address,address[], uint256[] & 4,822 & 72.36 \\
        9 & SmartAirdrop & 0xa8faf6f0 & - & 4,467 & 75.33 \\
        10 & PublicMine & 0x87ccccb3 & - & 4,157 & 78.10 \\
        11 & setGenesisAddress & 0x0d571742 & address, uint256, bytes & 3,119 & 80.17 \\
        \hline
    \end{tabular}

    }
\end{table}


==> Arxiv on-13-3-2021/conclusion.tex <==
\section{Conclusion and Future Work}
\label{conclusion}
%Blockchain is the technology which brings the whole new set of use cases which traditionally works in the presence of a trusted third party, not required anymore. As we know, blockchain is secure and tamper-proof decentralized distributed database and is not governed by any trusted third party, provides trust in untrusted peers. 

%In this work, we try to answer the following questions: (1) is it possible to improve the throughput by adding distributed power collectively in the current blockchain system? (2) how much speedup will we get per block if we employ such an approach? Hence 
In this paper, we proposed a distributed leader--follower framework \emph{DiPETrans} to execute transactions of block parallelly on multiple nodes (part of the same community). To the best of our knowledge, there is no such study in the literature. We tested our prototype on actual transactions extracted from Ethereum blockchain. We achieved proportional gains in performance to the number of followers. We have also seen performance gain in the execution time of the contract and monetary transactions. We evaluated \emph{DiPETrans} on various workloads, where the number of transactions ranges from 100 to 500 in a block, with a varying contract to monetary transactions. We observed that speedup often increases in a distributed setting with an increase in the number of transactions per block, thus increasing the throughput. We observed that a block execution time increases with the number of contract calls. We also have seen that speedup increases linearly with community size.

%, which can be the novelty of this work
There are several directions for future research. Assuming the number of transactions will increase over time, we can conceive a community that proposes multiple blocks in parallel. As stated earlier, an alternative way to boost performance is to use STM for follower nodes and run the transactions concurrently in each follower using multi-cores rather than serially. Another direction is that we assumed that no nested contract calls in this research, but in practice nesting is common with contracts of blockchains. So incorporating nesting is in our framework can be very useful. 

We have seen performance gain with just $5$ followers in the community. It would be interesting to see how the system scales and peak in speedup with hundreds or thousands of transactions per block and community followers? Apart from the above optimization, we are also planning to adopt a wholly distributed approach within the community instead of the leader-follower approach that is resilient to failures and other faults. We plan to integrate it with Ethereum blockchain by deploying a \emph{DiPETrans} community smart contract.

%we may expect to facilitate these transactions. {\color{blue}We can also further improve mining performance by using all the cores available with the system. The prototype implementation is tested with a trusted community that can easily be integrated into the permissible blockchain settings. However, testing for non-trusted community settings would be interesting. }

%In our future research, assuming the number of transactions will increase over time, we can conceive a community that proposes multiple blocks in parallel. As stated earlier, an alternative way to boost performance is to use STM for follower nodes and run the transactions concurrently with multi-core rather than serially. We assumed that no nested contract calls in this research, but we may expect to facilitate these transactions. {\color{red}We can also further improve mining performance by using all the cores available with the system. The prototype implementation is tested with a trusted community that can easily be integrated into the permissible blockchain settings. However, testing for non-trusted community settings would be interesting. We have seen performance gain with just six machines in the community. It would be interesting to see how the system scales with thousands of transactions per block and with hundreds (or thousands) of community followers? It will also be interesting to see a peak in speedup when there is a rise in transactions and the number of followers to hundreds or thousands in the community.} Apart from the above optimization, we are also planning to adopt a wholly distributed approach within the community instead of the leader-follower approach that is resilient to failures and other faults. We plan to integrate it with Ethereum blockchain by deploying a \emph{DiPETrans} community smart contract.

%In our future research, assuming the number of transactions will increase over time, we can conceive a community that proposes multiple blocks in parallel. As stated earlier, an alternative way to boost performance is to use STM for follower nodes and run the transactions concurrently with multi-core rather than serially. In this research, we assumed that no nested contract calls, but we may expect to facilitate these transactions. We can also further improve mining performance by making use of all the cores available with the system and dividing the search space for PoW based on that. Further, prototype blockchain implementation is tested for a trusted community, that can be extended for non-trusted community settings. Apart from the above optimization, we are also planning to adopt a wholly distributed approach within the community instead of the leader-follower approach that is resilient to failures and other faults. We plan to integrate it with Ethereum blockchain by deploying a \emph{DiPETrans} community smart contract. 



%In this work, we try to answer the following questions: (1) is it possible to improve the throughput by adding distributed power collectively in the current blockchain system? (2) how much speedup will we get per block if we employ such an approach in existing blockchains? Hence we proposed a distributed framework \emph{DiPETrans} to execute transactions of block parallelly on multiple trusted nodes (part of the same community). We tested our prototype on actual transactions extracted from Ethereum blockchain. 
%We achieved linear performance gains to the number of workers. We also saw performance gain in the runtime of contract and monetary transaction. We tested \emph{DiPETrans} on different workloads where the number of transactions varies from 100 to 500, with varying contract transactions to non-contract transactions. We found that with the increase in the number of transactions per block, speedup also increases in a distributed setting and improves the throughput. We observe that if the number of contract call increases in a block execution time also increases. We also observed that speedup linearly increases with the increase in the size of the community. In literature, there is no such study done before, which can be the novelty of this work.
%The main question we try to answer in this work is that, \emph{is it possible to improve the throughput by adding distributed power collectively through mining pools in the current blockchain system?} Another question we try to answer is that, \emph{how much speedup we will get per block if we employ such an approach in existing blockchains?} Hence we proposed a distributed framework \emph{DiPETrans} to execute transactions of block parallelly on multiple trusted nodes (part of the same community). We tested our prototype on actual transactions extracted from Ethereum blockchain and achieved linear performance gain to the number of workers. We also saw performance gain in the runtime of contract and monetary transaction. We tested \emph{DiPETrans} on different workloads where number of transactions varies from 100 to 500 with varying contract transactions : non-contract transactions = {1}:{1}, {1}:{2}, {1}:{4}, {1}:{8}, {1}:{16}. We found that with the increase in the number of transactions per block, speedup also increases in a distributed setting and improves the throughput. We observe that if the number of contract call increases in a block execution time also increases. We also observed that speedup linearly increases with the increase in the size of the community. In literature, there is no such study done before, which can be the novelty of this work.

%As part of our future work, assuming the number of transactions will increase over time, we can think of a community to work on proposing multiple blocks parallelly. As suggested earlier, another way to improve performance is to use STM at follower nodes and parallelly execute the transactions using multi-cores instead of serial execution. In this work, we have assumed that there are no nested contract calls, but we can think of an approach to provide support for those transactions. We can also further improve the performance of mining by making use of all the cores available with the system and dividing the search space for POW based on that.  Further, we tested prototype implementation for a trusted community, which can be extended for non-trusted community settings. Apart from the above optimization, we are also planning to adopt a wholly distributed approach within the community instead of the leader-follower approach and integrate it in Ethereum blockchain by deploying a \emph{DiPETrans} community smart contract. 

%As part of our future work, assuming the number of transactions will increase over time, we can think of a community to work on proposing multiple blocks parallelly. As suggested earlier, another way to improve performance is to use STM at follower nodes and parallelly execute the transactions using multi-cores instead of serial execution. In this work, we have assumed that there are no nested contract calls, but we can think of an approach to provide support for those transactions. We can also further improve the performance of mining by making use of all the cores available with the system and dividing the search space for POW based on that.  Further, we tested prototype implementation for a trusted community, which can be extended for non-trusted community settings. Apart from the above optimization, we are also planning to adopt a wholly distributed approach within the community instead of the leader-follower approach and integrate it in Ethereum blockchain by deploying a \emph{DiPETrans} community smart contract. 





%The main question we try to answer in this work is that, \emph{is it possible to improve the throughput by adding distributed power collectively through mining pools in the current blockchain system?} Hence we proposed a distributed framework \emph{DiPETrans} to execute transactions of block parallelly on multiple trusted nodes (part of the same community). We tested our prototype on actual Ethereum transactions and achieved linear performance gain to the number of workers. We saw performance gain in the runtime of contract and monetary transaction. We tested \emph{DiPETrans} on different workloads where number of transactions varies from 100 to 500 with varying contract transactions : non-contract transactions = {1}:{1}, {1}:{2}, {1}:{4}, {1}:{8}, {1}:{16}. We found that with the increase in the number of transactions per block, speedup also increases in a distributed setting and helps in improving the throughput. We observe that if the number of contract call increases in a block execution time also increases. We also observed that speedup linearly increases with the increase in the size of the community. In literature, there is no such study done before, and that can be the novelty of this work.

%As part of our future work, assuming the number of transactions will increase over time, we can think of a community to work on proposing multiple blocks parallelly. As suggested earlier, another way to improve performance is to use STM at follower nodes and parallelly execute the transactions using multi-cores instead of serial execution. In this work, we have assumed that there are no nested contract calls, but we can think of an approach to provide support for those transactions. Also, we can further improve the performance of mining by making use of all the cores available with the system and dividing the search space for POW based on that. Apart from the above optimization, we are also planning to adopt a distributed approach within the community instead of the leader-follower approach.

%We are also planning to include above-said optimization in our proposed framework.

 % There is the miner who makes use of GPU to increase their search space for PoW. But we are not sure that this is done in the mining pool based solution.
 
 
 
 

==> Arxiv on-13-3-2021/finalResults.tex <==
\begin{figure}[!htb]
    \centering
    {\includegraphics[width=1\textwidth]{figs/FinalResults/W1/W1-ExeTime.pdf}}\vspace{-.15cm}
    \caption{Workload-1: average transaction execution time by miner (omitting time to find PoW) and validator.}
    \label{fig:W1:avg-txn}
\vspace{.15cm}
	\centering
	{\includegraphics[width=1\textwidth]{figs/FinalResults/W1/W1-Speedup.pdf}}\vspace{-.15cm}
	\caption{Workload-1: average speedup by community miner and validator over serial miner and validator for transaction execution.}
	\label{fig:W1:avg-speed-up}
\end{figure}
%\vspace{.15cm}
\begin{figure}[!htb]
    {\includegraphics[width=1\textwidth]{figs/FinalResults/W2/W2-ExeTime.pdf}}\vspace{-.15cm}
    \caption{Workload-2: average transaction execution time by miner (omitting time to find PoW) and validator.}
    \label{fig:W2:avg-txn}
\vspace{.15cm}
    {\includegraphics[width=1\textwidth]{figs/FinalResults/W2/W2-Speedup.pdf}}\vspace{-.15cm}
    \caption{Workload-2: average speedup by community miner and validator over serial miner and validator for transaction execution.}
    \label{fig:W2:avg-speed-up}
%\vspace{-.55cm}
\end{figure}






==> Arxiv on-13-3-2021/intro.tex <==
\section{Introduction}
\label{introduction}
%{\color{red}\sout{According to a report published by the World Economic Forum (WEF) based on a survey on the future of the blockchain technology predicted that $\approx10\%$ of the Global Gross Domestic Product (GDP) would be stored on blockchain platforms by $2025$~\cite{WEFBlockchains2017}. Furthermore, with an annual growth rate of $26.2\%$, the capital market of $\$2.5$ billion in 2016 may touch the $\$19.9$ billion by $2025$~\cite{Zhang:2019arXiv190307602Z, CoinDesk}. Many well-known information technology vendors, governments, Internet giants, and banks are investing in blockchain to make distributed ledger technology versatile and widely used~\cite{Zhang:2019arXiv190307602Z}.}}

%A blockchain can be defined as a distributed decentralized database which is tamper-proof, publicly accessible, highly secure, append-only, the permanent collection of the records organized in the chain of the blocks \cite{nakamoto2009bitcoin, Dickerson+:ACSC:PODC:2017,Vikram:DBLP:journals/corr/abs, Ethereum, Hyperledger}. It maintains a distributed global state of the transactions in the absence of a trusted central authority. An anonymous group or individual known as Satoshi Nakamoto was the first who introduced blockchain in a paper titled Bitcoin: a peer-to-peer electronic cash system in 2008 \cite{nakamoto2009bitcoin}. Since then, it is commonly believed that there is a possibility of becoming rich by mining coins \cite{bitcoin:faq:2019}. Both industries and academia are trying to generalize this technology to support different type of applications. However, it is still not matured enough and experiencing a lot of development.

A blockchain is a distributed decentralized database that is a secure, tamper-proof, publicly accessible collection of the records organized as a chain of the \emph{blocks} \cite{nakamoto2009bitcoin,Dickerson+:ACSC:PODC:2017}. It maintains a distributed global state of the transactions in the absence of a trusted central authority. Due to its usefulness, it has gained widespread interest both in industry and academia. 

%A blockchain consists of \emph{nodes} or \emph{peers} maintained in a peer-to-peer manner. A node in the network may serve as a \emph{miner} and/or as a \emph{validator}. A miner proposes a block to add to the blockchain by verifying the requests and solving a Proof of Work (PoW) to delay-wait the network. The rest of the peers in the network validate the requests in that block, and the solution to the PoW. A \emph{block} consists of a set of transactions, timestamp, block id, nonce, coin base address (miner address), previous block's hash, current block's hash, etc. The block is added to the blockchain-based on the consensus between the peers validating that block. 
%Typically, the entire copy of the blockchain is stored on all the nodes of the system. \emph{Clients} (also known as users) external to the system use the services of the blockchain by sending transactions to the nodes of the blockchain system. A node forms a block from several requests and follows the mining and validation process to append it to the blockchain.

A blockchain consists of \emph{nodes} or \emph{peers} maintained in a peer-to-peer (P2P) manner. A node in the network may serve as a miner and/or as a validator. A \textit{miner} $m$ proposes a block to add to the blockchain, and hence is also referred to as a block producer in literature. A \textit{block} generated by the miner consists of \textit{transactions} typically encoding some business logic. Node $m$ then solves a Proof-of-Work (PoW) to delay-wait the network and then broadcasts the block through the P2P network. The rest of the peers in the network, on receiving the block, validate the transactions in that block and the solution to the PoW. Hence, they are called as \textit{validators}. \emph{Clients}, also known as users, external to the system use the blockchain services by sending transactions to the network peers. On receiving a sufficient number of transactions from clients, a node takes the role of a miner to form a block. It then follows the mining and validation process to append the block to the blockchain. A block in a typical blockchain such as Ethereum~\cite{Ethereum} consists of a set of transactions, its timestamp, block id, nonce, coin base address (miner address), the hash of the previous block in the chain, the current block's hash, etc. The block is added to the blockchain through consensus between the peers validating the block. Usually, the entire copy of the blockchain is stored on all the nodes.



%\emph{Clients} (also known as users) external to the system use the services of the blockchain by sending transactions to the nodes of the blockchain system. On receiving a sufficient number of transactions from clients, a node takes the role of a miner. It forms a block, then follows the mining and validation process to append the block to the blockchain. A block consists of a set of transactions, timestamp, block id, nonce, coin base address (miner address), previous block's hash, current block's hash, etc. The block is added to the blockchain based on the consensus between the peers validating that block. Usually, the entire copy of the blockchain is stored on all the nodes.% of the system. 

%\emph{Clients} (also known as users) external to the system use the services of the blockchain by sending transactions to the nodes of the blockchain system. A node on receiving sufficient number transactions from clients, takes the role of a miner. It forms a block, then follows the mining and validation process to append the block to the blockchain.
%The block is added to the blockchain based on a majority of peers validating that block 
%\ysnote{confirm "majority"}.\psnote{replaced ``majority'' with ``consensus''.}

\textit{Bitcoin}~\cite{nakamoto2009bitcoin}, the first blockchain system proposed by Satoshi Nakamoto, is the most popular blockchain to date. It is a cryptocurrency system that is highly secure where users need not trust others. Further, there is no central controlling agency, like the current day banking system. Ethereum~\cite{Ethereum} is another popular blockchain that provides complex services in addition to cryptocurrencies such as user-defined scripts, called \emph{smart contracts}. Such smart contracts are written in Turing complete language Solidity~\cite{Solidity}. A smart contract is like an object in the object-oriented programming language, which consists of methods and data (state). They can be used to automatically define and enforce terms and conditions in the contract without the intervention of a trusted third party. A client's request to execute a contract's \mth{s}, also called a transaction, consists of the miner and validator nodes, invoking a series of these methods and their input parameters. Such contracts can be simple cryptocurrency exchanges between wallets or more complex logic such as Ballot and Simple Auction~\cite{Solidity}.%as given in Solidity documentation \cite{Solidity}.
%\ysnote{give a brief example}. \psnote{Done.}
%A transaction can be initiated by a client or a peer, and executed by all the peers. 

%Bitcoin is an application specific distributed ledger technology.
%Bitcoin \cite{nakamoto2009bitcoin}, a highly secure cryptocurrency system, is the first public blockchain which is still highly popular. It processes the transactions in a distributed decentralized manner where a user need not trust anyone. Further there is no central controlling agency like current day banking system. Ethereum \cite{Ethereum} is another popular blockchain. As compared to Bitcoin \cite{nakamoto2009bitcoin}, Ethereum  provides support for user-defined programs (scripts), called \emph{smart contracts} \cite{Solidity} to offer complex services. 

%Smart contracts in the Ethereum are written in the Turing complete language \emph{Solidity}~\cite{Solidity}. These contracts automatically provide several operations using pre-recorded terms and conditions in the contract without the intervention of a trusted third party. In general, a smart contract is like an object in object-oriented programming languages, which consists of methods and data (state) \cite{Dickerson+:ACSC:PODC:2017, Solidity}. A client request (\emph{transaction}), consists of calls to these methods and corresponding input parameters. A transaction can be initiated by a client (user) or a peer, and executed by all the peers. Whenever a user sends a request, the corresponding method of the contract is called by the miner, and the contract state may change to the new state. In Ethereum, every account has its separate space to maintain state updates. Contracts are also yet another address on Ethereum and maintain separate space for modifications done via contract transactions \cite{Ethereum}.



%A client wishing to use the services of the blockchain contacts a node of the system and send the request, which is a transaction. A node $N_i$ on receiving several such transactions from different clients or other peers forms a \emph{block} to be added to the blockchain. The node $N_i$ is said to be a \emph{\bp} and cryptocurrencies based blockchains such as Bitcoin, Ethereum, \bp{s} are called as \emph{miners} as they can `mine' new coins.% In this document, we use these terms interchangeably. 



%It executes the respective methods of the contract and changes the current state of the contract to the new state.
%It uses the cryptographic algorithm to encrypt everything and record them in the form of a chain of the blocks hence known as a blockchain.

%In the current implementation of most popular blockchain designs such as Bitcoin \cite{nakamoto2009bitcoin} and Ethereum \cite{Ethereum}, these transactions are executed in an ordered manner first by the miner later by the validators \cite{Dickerson+:ACSC:PODC:2017}. Basically, when a miner creates a block, miner is given a choice to pick the transactions based on its preference, for e.g., giving high priority to higher transactions fees, sequentially execute associated transactions, find the proof-of-work (PoW), and finally broadcast the block to other peers for validation to earn reward and append it to its local blockchain. The validation by other peers is also done sequentially in the same order as proposed by the miner to attain the consensus. Finally, after successful validation of a block by the majority (accepted by more than 50\%) of the peers/validators, the consensus is reached, and the miner gets the incentive for that block.


%\todo[inline]{YS: a lot of the following text should move to "Background and Related Work". Just the essential needed to establish the computationally expensive parts, of PoW and transaction execution, needs to be highlighted in 1 para in the intro as motivation for the problem.}

\vspace{.2cm}
\noindent
\textbf{Drawback with Existing Systems:} Miners and validators in current blockchain systems execute the transactions serially. Further, finding the PoW, a computationally intensive brute-force process to create a new block. 
% PoW is required to delay-wait the network to reach consensus and allow miners to create a new block in their favor.
Miners compete to verify transactions and solve the PoW to create a block.
% However, the problem is that the high computation requirements make it very difficult for a resource constraint miner to compete for the block creation to get intensive
Dickerson et al.~\cite{Dickerson+:ACSC:PODC:2017} observe that the transactions are executed serially in two different contexts. First, executed serially by the miner while creating a block. Later, validators re-executes the transactions serially to validate the block. Typically, miners execute hundreds of transactions, and validators cumulatively execute millions of transactions serially for each new block. The serial execution of the transaction leads to poor throughput and is inefficient in the current era of distributed and multi-core systems. %Such block transactions are executed several times by the miners and many more times by the validators. 
%\ysnote{Intead of previous line, it will be good to say something like miners execute 100's of transactions and validators cumulatively execute millions of transactions, for each new block.}\psnote{Done.}
The high transaction fee, poor throughput (transactions/second), high block acceptance latency, and limited computation capacities prevent widespread adoption of blockchain~\cite{eos:url}. %\cite{eos:url, BC-Scalability}. 
Hence adding parallelism to the blockchain can improve efficiency and achieve higher throughput.%Hence adding parallelism to the blockchain can improve efficiency and achieve higher throughput.

%In existing blockchain systems, miners and validators execute the transactions and find the \emph{Proof of Work (PoW)} serially. {\color{blue}PoW is an answer to a mathematical puzzle that needs to be solved by the miners to add a new block to the blockchain. It includes finding the hash of the block smaller than the difficulty decided by the network.} Finding the PoW \cite{PoW} is a computationally intensive random process. This makes it difficult for a resource-constrained miner to compete for the block creation to get  incentive~\cite{Eyal:BitcoinMiningVulnerable}.

%Also, in the current era of distributed and multi-core system, sequential transaction execution results in poor throughput. Dickerson et al.~\cite{Dickerson+:ACSC:PODC:2017} observe that the transactions are executed serially in two different contexts. First, they are executed serially by the miner while creating a block. Later, each validator re-execute the transactions serially to validate the block, compounding the cost many-fold.

%In addition, high transaction fees, poor throughput (transactions/second), significant transaction acceptance latency, and limited computation capacities prevent widespread adoption~\cite{eos:url, BC-Scalability}. Hence adding parallelism to the blockchain framework can achieve better efficiency and higher throughput.

\vspace{.2cm}
\noindent
\textbf{Solution Approach:} There are several solutions proposed and used in Bitcoin and Ethereum to mitigate these issues. One such solution is that several resource constraint miners form a \emph{mining pool} or \textit{community} to solve the PoW. After block acceptance, they share the incentive among them~\cite{lewenberg2015bitcoin, MiningPools:NBERw25592, Luu:SmartPool:usenix2017}.%In the rest of the paper, we use the pool and community interchangeably.

%There are few solutions proposed and used in Bitcoin and Ethereum blockchains to mitigate these issues. One is for several resource constraint miners to form a\emph{mining pool} (community) to determine the PoW, and after block acceptance, share the incentive among them \cite{Eyal:BitcoinMiningVulnerable, Eyal:MiningPool, qin18mining, lewenberg2015bitcoin, MiningPools:NBERw25592, Wiki:MiningPool, MiningPoolCentralized}. %For sharing the incentive, several solutions (proportional, pay-per-share, pay-per-last-N-shares) have been proposed in the literature and implemented by the mining pools. In the rest of the paper, we use pool and community interchangeably.\todo{YS: we may want to stick with one}

%\todo{YS: we may want to stick with one}

Other solutions~\cite{Dickerson+:ACSC:PODC:2017, Anjana:OptSC:PDP:2019, Anjana:DBLP:journals/corr/abs} suggest concurrent execution of the transactions at runtime in two stages: first while proposing the block, and second while validating the block. This helps in achieving better performance while creating the block and when validating, hence increasing the chance of a miner to receive their fees. However, it is not straightforward; it requires a proper strategy to avoid a valid block being rejected due to false block rejection (FBR) error~\cite{Anjana:OptSC:PDP:2019} and to overcome malicious miners. Some of these use runtime techniques based on Software Transactional Memory to execute transactions concurrently. A miner concurrently executes the block transactions and constructs the block graph alongside. The graph records dependencies between the transactions where vertices are the transactions and edges between them indicate a dependency. In the end, the miner adds the block graph to the block to help the validator execute these transactions concurrently and avoid FBR error~\cite{Anjana:OptSC:PDP:2019}.

%\spnote{Please replace \cite{Anjana:DBLP:journals/corr/abs} with Netys 2020 paper.}
%\psnote{Paper is not uploaded online yet. So we updated BibTeX accordingly and left the page number field empty.}
% During the concurrent execution at validator, the FBR error may easily occur if transactions dependencies are not recorded appropriately in the block graph.

%Other solutions~\cite{Dickerson+:ACSC:PODC:2017, Anjana:OptSC:PDP:2019, Anjana:DBLP:journals/corr/abs} suggest concurrent execution of the transactions at runtime in two stages: first while proposing the block, and second while validating the block. This helps in achieving better speedups while creating the block and when validating, hence increase the chance of a miner to receive their fees. However, it is not straightforward and requires a proper strategy so that a valid block should not be rejected due to false block rejection or \emph{FBR error} \cite{Anjana:DBLP:journals/corr/abs}. These techniques follow Software Transactional Memory based runtime techniques to execute transactions concurrently. Miner concurrently executes the block transactions and construct the block graph alongside. The block graph is used to record the dependencies between the transactions where vertices depict the transactions and edges between them stores the dependencies. In the end, miner adds a block graph in block to help the validator to execute transaction concurrently and to avoid FBR error. During the concurrent execution at validator, the FBR error may easily occur if transactions dependencies are not recorded appropriately in the block graph.

%\todo[inline]{YS: The prior statements seem like a weak argument against the existing approaches. Need something more compelling on the novelty}

In contrast to those approaches, we propose to use a cluster of machines that form a community to execute or validate the transactions in a distributed manner based on a static analysis of the transactions. This improves the performance of both block mining and validation. The community has a \textit{leader} machine and a set of \textit{follower} machines. The leader is part of the blockchain while the follower nodes are at the disposal of the leader and are not part of the blockchain. The followers being at the diposal of the leader, form a trusted community with the leader, e.g., they belong to the same organization. 

%In this manner, the trusted community is formed. 

The leader performs static analysis of the transactions in a block to identify dependencies and shards them into independent transactions, which are each executed in a distributed manner by the followers concurrently (see \figref{ds}). The miners and validators can each perform this static analysis for parallel execution. This avoids encoding the block dependency graph within the block, while also preventing FBR errors. When mining, the solution space for the PoW is also partitioned and solved in parallel by the followers. %We implement and validate this approach within the Ethereum blockchain~\cite{Ethereum}.
{We implement and empirically validate the benefits of our approach within the Ethereum blockchain~\cite{Ethereum}. However, the proposed approach is generic and can be integrated into any other permissionless and permissioned (by excluding PoW computation of current approach) blockchain platform that follows an order-execute transaction execution model \cite{androulaki2018hyperledger}. } %as Ethereum %Hence, FBR error and malicious miner issue will not occur if the validator does not use the miner's dependencies information since dependencies remain the same in the static analysis. A validator can perform the static analysis before parallel execution, which makes it very straightforward to adopt. The basic idea is that unrelated transactions of the block are grouped into different shards , and shards are assigned to different nodes of the community (see {Figure \ref{fig:arch}}), which the nodes execute independently in parallel. 
%{\color{blue}It means the proposed approach applies to other PBFT consensus-based blockchains, in which its benefits will be more evident. We have chosen the PoW as we report experiments with over 5~Million transactions from the Ethereum blockchain. }
This implies \emph{DiPETrans} can be integrated with any other consensus-based (such as PBFT) order-execute blockchain platform. %\sout{We have chosen the PoW as we report experiments with over 5~Million transactions from the Ethereum blockchain.}} \spnote{Please review this.}
\textit{To our knowledge, this is the first work that uses static analysis to identify block transactions that can be executed in parallel and combines them with the benefits of sharding and mining pools.}

%In this work, our objective is to execute the transactions in parallel based on a static analysis of the transactions, using a community of trusted nodes (workers) modeled as a leader and followers, along with finding the PoW in parallel, to improve the performance of block creation and validation. We proposed a framework for distributed parallel execution in a formal setting inspired by Ethereum~\cite{Ethereum}. We follow a static analysis based sharding technique to determine the transaction dependencies. Hence, \emph{FBR error} will not occur if the validator does not use the miner's dependencies information since dependencies remain the same in the statical analysis. A validator can perform the static analysis before parallel execution, which makes it very straightforward to adopt. %\todo[inline]{YS: we need to be careful in our claims about Ethereum since we don't use it directly for our experiments} % The core idea is to form a community of multiple trusted nodes and make use of the distributed compute power using a leader-follower approach. \todo{YS:repetitive}

%Unrelated transactions of the block are grouped into different shards (see Fig.~\ref{fig:ds}), and shards are assigned to different nodes of the community (see {Fig. \ref{fig:arch}}), which the nodes execute independently in parallel. To our knowledge, this is the first work which uses static analysis for identifying block transactions that can be executed in parallel, and combines these with benefits associated with sharding and mining pools.



%\todo[inline]{YS:move this figure/description to "Proposed Method"?}

\vspace{.2cm}
\noindent
{The \textbf{key contributions} of this paper are as follows:}
\begin{itemize}
    % \item We propose a framework \emph{DiPETrans} for parallel execution of the transactions by a miner and the validators based on transaction sharding using a static analysis and mining communities. This is the first contribution which combines the advantages associated with both sharding and mining pools.
    %%\item We propose a framework \emph{DiPETrans}: \underline{Di}stributed \underline{P}arallel \underline{E}xecution of \underline{Trans}actions of Blocks in Blockchain for parallel execution of the transactions at miners and validators, based on transaction shards identified using static analysis. %\todo[inline]{YS: It appears like each of these already exist but we're just slapping them together?}
    
    %\item We propose a \emph{DiPETrans}: \underline{Di}stributed \underline{P}arallel \underline{E}xecution of \underline{Trans}actions of Blocks in Blockchain framework in \textsection \ref{methodology} for parallel execution of the transactions at miners and validators, based on transaction shards identified using static analysis.
    \item We propose a \emph{DiPETrans: \underline{Di}stributed \underline{P}arallel \underline{E}xecution of \underline{Trans}actions of Blocks in Blockchain} framework in \textsection \ref{methodology} for parallel execution of the transactions at miners and validators, based on transaction shards identified using static analysis.
    
    %\item \sout{Once the miner proposes a block; the validator executes the transactions parallelly using the same approach followed by the miner.}% However, the only difference is that validators do not determine PoW.% The validator executes the transactions parallelly and checks the final state computed by them matches with the final state of the block as computed by the miner, subsequently also confirms that the PoW is valid or not.

	\item We implement this technique using a distributed leader--follower approach within a mining community of servers, where the leader shards the transactions in the block and the followers concurrently execute (mining) or verify (validation) them. When mining, the PoW is also partitioned and solved in parallel by the members of the community.

    %\item We implemented two different approaches for the validator. In the first approach known as {\sVal}, the miner incorporates some information about the dependent transactions (shards) in the block to help the validators to execute the block transactions deterministically and in parallel. While in the second {\dVal}, the miner does not include dependency information in the block, and validators infer the dependencies themselves.
	% 5,170,597
	\item We report experiments in \textsection \ref{experiment} using over $5$~Million real transactions from the Ethereum blockchain and execute them using \emph{DiPETrans} to empirically validate the benefits of our techniques over traditional sequential execution. We achieve a maximum speedup of $2.18\times$ for the parallel miner and $2.02\times$ for the parallel validator, for $100$ to $500$ transactions per block. Further, we achieve a maximum of $5\times$ end-to-end block creation speedup using the parallel miner over a serial one, when using 6 machines in the community, including the leader.

    %\item We report experiments using 5,170,597 transactions from the Ethereum blockchain and execute them using our \emph{DiPETrans} framework to empirically validate the benefits of our techniques over traditional sequential execution. We achieved a maximum speedup of $2.18\times$ for the miner, $2.02\times$ for the validator, without information sharing (i.e., \dVal), and $2.04\times$ for with information sharing (i.e., \sVal) for 100 to 500 transactions per block, when using 6 workers (including leader) in the community. %this should not come as a contribution but is more of a result.
\end{itemize}


We present related work in \textsection \ref{relatedWork} and conclude with some future research directions in \textsection \ref{conclusion}.
%The rest of the paper is organized as follows: We present related work in \textsection \ref{relatedWork}. In \textsection \ref{methodology}, we describe the DiPETrans architecture and methodology. \textsection \ref{experiment} consists of the experimental evaluation and results. Finally, we conclude with some future research directions in \textsection \ref{conclusion}.
%\spnote{Please remove this above paragraph. Add section names directly in the contributions}
%\psnote{In the end, if we do not have sufficient space, we will remove this.}















%{\color{blue}Three paragraphs from here are moved to Background and Related Work.}
\begin{comment}
In most of the popular blockchain system such as Bitcoin and Ethereum, transactions are executed in an ordered manner first by the \emph{miners} and later by the \emph{validators}~\cite{Dickerson+:ACSC:PODC:2017}, which are peers in the network. When a miner creates a block, they may choose to select the transactions based on their preference, e.g., giving higher priority to transactions with higher fees (incentive). So after selecting the set of transactions, the miner serially executes these transactions, adds the final state to the block after execution, finds the proof-of-work (PoW)~\cite{PoW}, and broadcasts the block to other peers in the network for validation to earn the reward. PoW solves a mathematical puzzle, necessarily by brute-force, where the miner finds the hash of the block that is smaller than the given difficulty. This is computationally challenging. It is required as a delay-wait on the network to help reach consensus and allow miners to create a new block in their favor. 

Later, after receiving a block, each validator re-executes the transactions in the block serially, verifies the final state computed by them with the final state provided by the miner in the block, and also validates that miner solved the PoW correctly -- verifying the PoW solution is cheap. The transaction re-execution by the validators is done serially, in the same order as listed in the block by the miner, to attain the consensus~\cite{Dickerson+:ACSC:PODC:2017}. After validation, if the block is accepted by a majority ($>50\%$) of the validators, the block is added to the blockchain by all, and the miner gets its fee.% However, it is also possible that multiple blocks are proposed and added to the chain at the same time, which creates the fork in the chain; but, the longest chain is considered as the consistent one.

%Further, blockchain is designed such a way that every block which is added to the chain depends on the previous block's hash to force a chronological order. This ordering based on cryptographic hash makes it exponentially challenging to make any change to earlier transactions because this will requires recalculation of PoW of all the subsequent blocks and accepted by the majority of them. Also if two blocks are proposed at the same time and added to the blockchain, they form the fork, miners work on the first block they receive and switch to the longest chain of blocks as soon as the next block is formed. This allows mining to secure and maintain a global consensus based on processing power. If a miner can possess the majority of compute power, then theoretically can manipulate the transactions for its own gain \cite{BC-Mining}.

Blockchain is designed to force a chronological order between the blocks as every block added to the chain depends on the hash of the previous block. This ordering based on the cryptographic hash makes it exponentially challenging to make any change to the earlier blocks -- to make even a small change to an accepted transaction or a block in the blockchain requires recalculation of the PoW of all the subsequent blocks and their acceptance by a majority of the peers in the network. Also, if two blocks are proposed at the same time and added to the chain, they form the fork, miners work on the first block they receive and eventually switch to the longest chain. These allow mining to be secure and maintain a global consensus based on processing power.% If a miner can possess the majority of computing power, then theoretically can manipulate the transactions for its gain \cite{BC-Mining}.

\end{comment}


==> Arxiv on-13-3-2021/macros.tex <==
% comment a region

\newcommand{\punt}[1]{}
\newcommand{\cmnt}[1]{}


% a word should not be broken across lines
\newcommand{\nosplit}{\linebreak}

% no hyphenation
\def\nohyphens{\hyphenpenalty=10000\exhyphenpenalty=10000}

% ~ character
\newcommand{\tilda}{\symbol{126}}

% useful mathematical symbols

\newcommand{\ang}[1]{\langle #1 \rangle}
\newcommand{\Ang}[1]{\Big\langle #1 \Big\rangle}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}


% quantifiers
\newcommand{\myforall}[3]{\ang{\forall \: #1 : #2 : #3 }}
\newcommand{\myexists}[3]{\ang{\exists \: #1 : #2 : #3 }}
\newcommand{\mynexists}[3]{\ang{\nexists \: #1 : #2 : #3 }}
\newcommand{\Myforall}[3]{\Ang{\forall \: #1 : #2 : #3 }}
\newcommand{\Myexists}[3]{\Ang{\exists \: #1 : #2 : #3 }}
\newcommand{\Mynexists}[3]{\Ang{\nexists \: #1 : #2 : #3 }}


% for formally defining a notion
% \newcommand{\defined}{\;\;\stackrel{\triangle}{=}\;\;}
\newcommand{\defined}{\;\;\triangleq\;\;}


% mathematical implications

%\renewcommand{\implies}{\Rightarrow}
\newcommand{\follows}{\Leftarrow}

% miscellaenous
\newcommand{\myspace}{\hspace*{0.0in}}
\newcommand{\halflinespacing}{\vspace*{0.5em}}
\newcommand{\greaterlinespacing}{\vspace*{0.75em}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% keywords for pseudocode

\newcommand{\myif}{\textbf{if}}
\newcommand{\mythen}{\textbf{then}}
\newcommand{\myelse}{\textbf{else}}
\newcommand{\myendif}{\textbf{endif}}
\newcommand{\myor}{\textbf{or}}
\newcommand{\myand}{\textbf{and}}
\newcommand{\mynot}{\textbf{not}}

%% various theorem environments
%% Commented out because they are already defined in llncs file %%
%% Decommented out because they are not defined in sigplan class %%

%\newtheorem{theorem}{Theorem}
%\renewcommand{\thetheorem}{\arabic{theorem}}

%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{property}[theorem]{Property}
%\newtheorem{definition}[theorem]{Definition}

%\renewtheorem{property}[theorem]{Property}

%\newtheorem{definition}{Definition}
%\renewcommand{\thedefinition}{\arabic{definition}}

%\newtheorem{property}{Property}
%\renewcommand{\theproperty}{\arabic{property}}

%\newtheorem{observation}[theorem]{Observation}
%\renewcommand{\theobservation}{\arabic{observation}}

%\newtheorem{example}{Example}
%\renewcommand{\theexample}{\arabic{example}}

%\newtheorem{assume}{Assumption}
%\renewcommand{\theassume}{\arabic{assume}}

%\newtheorem{remark}{Remark}
%\renewcommand{\theremark}{\arabic{remark}}

%\newtheorem{axiom}[theorem]{Proposition}
%\renewcommand{\theaxiom}{\arabic{axiom}}

%\newtheorem{invariant}[theorem]{Invariant}

%\renewcommand{\theequation}{\arabic{equation}}

%-----------------Theorem Notations Defined by Petr ---------------------------------------------------------------------------------------------------------
%% Defined by Petr

%\newtheorem{acknowledgement}[theorem]{Acknowledgement}
%\newtheorem{algorithm}[theorem]{Algorithm}
%\newtheorem{case}[theorem]{Case}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{explanation}[theorem]{Explanation}
%\newtheorem{fact}[theorem]{Fact}
% \newtheorem{conclusion}[theorem]{Conclusion}
% \newtheorem{condition}[theorem]{Condition}
%\newtheorem{conjecture}[theorem]{Conjecture}
% \newtheorem{criterion}[theorem]{Criterion}
%\newtheorem{definition}[theorem]{Definition}
% \newtheorem{example}[theorem]{Example}
% \newtheorem{exercise}[theorem]{Exercise}
%\newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{notation}[theorem]{Notation}
% \newtheorem{problem}[theorem]{Problem}
%\newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{remark}[theorem]{Remark}
% \newtheorem{solution}[theorem]{Solution}
% \newtheorem{summary}[theorem]{Summary}
%\newtheorem{observation}[theorem]{Observation}
%\newenvironment{proofsketch}[1][Proof sketch]{\noindent\textbf{#1.} }{\hfill $\Box$\\[2mm]} %\rule{0.5em}{0.5em}\\}
%\newenvironment{reptheorem}[1][Theorem]{\noindent\textbf{#1}}{}

%------------------------------------------------------------------------------------------------------------------------------

% various references
\newcommand{\chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\stref}[1]{step~\ref{step:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}}
%\newcommand{\corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\axmref}[1]{Proposition~\ref{axm:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\eqnref}[1]{Eqn.(\ref{eq:#1})}
\newcommand{\eqvref}[1]{Equivalence~(\ref{eqv:#1})}
\newcommand{\ineqref}[1]{Inequality~(\ref{ineq:#1})}
%\newcommand{\invref}[1]{(\ref{inv:#1})}
\newcommand{\exref}[1]{Example~\ref{ex:#1}}
\newcommand{\propref}[1]{Property~\ref{prop:#1}}
\newcommand{\obsref}[1]{Observation~\ref{obs:#1}}
\newcommand{\asmref}[1]{Assumption~\ref{asm:#1}}
\newcommand{\thref}[1]{Thread~\ref{th:#1}}
\newcommand{\trnref}[1]{Transaction~\ref{trn:#1}}

%\newcommand{\lineref}[1]{Line~\ref{lin:#1}}
\newcommand{\algoref}[1]{{Algorithm~\ref{alg:#1}}}
\newcommand{\subsecref}[1]{SubSection~\ref{subsec:#1}}
\newcommand{\subsubsecref}[1]{SubSubSection~\ref{subsubsec:#1}}

\newcommand{\apnref}[1]{Appendix~\ref{apn:#1}}
\newcommand{\invref}[1]{Invariant~\ref{inv:#1}}

\newcommand{\Chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\Figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\Tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\Stref}[1]{Step~\ref{step:#1}}
\newcommand{\Thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\Lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\Corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\Axmref}[1]{Proposition~\ref{axm:#1}}
\newcommand{\Defref}[1]{Definition~\ref{def:#1}}
\newcommand{\Eqref}[1]{(\ref{eq:#1})}
\newcommand{\Eqvref}[1]{Equivalence~(\ref{eqv:#1})}
\newcommand{\Ineqref}[1]{Inequality~(\ref{ineq:#1})}
\newcommand{\Exref}[1]{Example~\ref{ex:#1}}
\newcommand{\Propref}[1]{Property~\ref{prop:#1}}
\newcommand{\Obsref}[1]{Observation~\ref{obs:#1}}
\newcommand{\Asmref}[1]{Assumption~\ref{asm:#1}}

\newcommand{\Lineref}[1]{Line~\ref{lin:#1}}
\newcommand{\Algoref}[1]{{\sf Algo$_{\ref{algo:#1}}$}}

\newcommand{\Apnref}[1]{Section~\ref{apn:#1}}
\newcommand{\Invref}[1]{Invariant~\ref{inv:#1}}


% environment for writing a proof

%\newcommand{\proof}[1][]{\noindent{\bf\boldmath
%                          P\hspace{-0.25ex}roof{#1}\/:\unboldmath}\hspace*{0.5em}}


%\newcommand{\theqed}{$\Box$}

%\newcommand{\qed}{\hspace*{\fill}\theqed\\\vspace*{-0.5em}}

% In case the proof is immediately followed by the start of a new section

\newcommand{\nsqed}{\hspace*{\fill} \theqed}


% End of example

\newcommand{\eoe}{\qed}

% Renews the footnote command
%\renewcommand{\thefootnote}{\alph{footnote}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Definitions by Petr 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\lf{\tiny}
\def\rrnnll{\setcounter{linenumber}{0}}
\def\nnll{\refstepcounter{linenumber}\lf\thelinenumber}
%\newcounter{linenumber}
%\newenvironment{algorithmfig}{\hrule\vskip 3mm}{ \vskip 3mm \hrule }

\def\P{\ensuremath{\mathcal{P}}}
\def\DP{\ensuremath{\Diamond\mathcal{P}}}
\def\DS{\ensuremath{\Diamond\mathcal{S}}}
\def\T{\ensuremath{\mathcal{T}}}
\def\Time{\mathbb{T}}
\def\S{\ensuremath{\mathcal{S}}}
\def\D{\ensuremath{\mathcal{D}}}
\def\W{\ensuremath{\mathcal{W}}}
\def\A{\ensuremath{\mathcal{A}}}
\def\B{\ensuremath{\mathcal{B}}}
\def\F{\ensuremath{\mathcal{F}}}
\def\R{\ensuremath{\mathcal{R}}}
\def\H{\ensuremath{\mathcal{H}}}
%\def\N{\ensuremath{\mathcal{N}}}
\def\N{\ensuremath{\mathbb{N}}}
\def\I{\ensuremath{\mathcal{I}}}
\def\O{\ensuremath{\mathcal{O}}}
\def\Q{\ensuremath{\mathcal{Q}}}
\def\K{\ensuremath{\mathcal{K}}}
\def\L{\ensuremath{\mathcal{L}}}
\def\M{\ensuremath{\mathcal{M}}}
\def\V{\ensuremath{\mathcal{V}}}
\def\E{\ensuremath{\mathcal{E}}}
\def\C{\ensuremath{\mathcal{C}}}
%\def\T{\ensuremath{\mathcal{T}}}
\def\X{\ensuremath{\mathcal{X}}}
\def\Y{\ensuremath{\mathcal{Y}}}
\def\Nat{\ensuremath{\mathbb{N}}}
\def\Om{\ensuremath{\Omega}}
\def\ve{\varepsilon}
\def\fd{failure detector}
\def\cfd{\ensuremath{?\P+\DS}}
\def\afd{timeless}
\def\env{\ensuremath{\mathcal{E}}}
%\def\faulty{unreliable}
\def\bounded{one-shot}
\def\cons{\textit{cons}}
\def\val{\textit{val}}
\def\code{\textit{code}}

\def\HSS{\mathit{h}}
\def\argmin{\mathit{argmin}}
\def\proper{\mathit{proper}}
\def\content{\mathit{content}}
\def\Level{\mathit{L}}
\def\Blocked{\mathit{Blocked}}
\def\Set{\mathit{Set}}


\newcommand{\remove}[1]{}

\newcommand{\Wset}{\textit{Wset}}
\newcommand{\Rset}{\textit{Rset}}
\newcommand{\Dset}{\textit{Dset}}
%\newcommand{\T}{$\mathcal{T}$}

%\newcommand{\parts}{\textit{parts}}

\newcommand{\trylock}{\textit{trylock}}
\newcommand{\multitrylock}{\textit{multi-trylock}}
\newcommand{\CAS}{\textit{CAS}}
\newcommand{\mCAS}{\textit{mCAS}}

\def\Nomega{\ensuremath{\neg\Omega}}
\def\Vomega{\ensuremath{\overrightarrow{\Omega}}}

\newcommand{\id}[1]{\mbox{\textit{#1}}}% for identifiers in code
\newcommand{\res}[1]{\mbox{\textbf{#1}}}% reserved words

\newcommand{\ignore}[1]{}

\newcommand{\myparagraph}[1]{\vspace{1mm}\noindent\textbf{#1}}

%------------------------------------------------------------------------------------------------------------------
% Definitions for Weak Consistency paper
%------------------------------------------------------------------------------------------------------------------

\newcommand{\op} {operation}
\newcommand{\termop} {terminal operation}
\newcommand{\nonin} {non-interference}
\newcommand{\perm} {permissive}
\newcommand{\pness} {permissiveness}
\newcommand{\ai} {abort-invisible}
\newcommand{\ait} {abort-invisiblity}
\newcommand{\vwc} {\textit{VWC}}
\newcommand{\lo} {\textit{LO}}
\newcommand{\clo} {\textit{CLO}}
\newcommand{\svlo} {\textit{CLO}}
\newcommand{\svsls} {\textit{CLO}}

\newcommand{\sts} {SS}
\newcommand{\comm}[1] {\textit{committed(#1)}}
\newcommand{\aborted}[1] {\textit{aborted}(#1)}
\newcommand{\txns}[1] {\textit{txns}(#1)}
\newcommand{\forceCom}[2] {$#1^{#2,C}$}
\newcommand{\remSub}[2] {$#2_{-#1}$}
\newcommand{\permfn}[1] {Perm(#1)}
\newcommand{\nifn}[1] {\textit{NI}(#1)}
\newcommand{\prevA}[2] {\textit{IncAbort}(#1, #2)}
\newcommand{\prevC}[2] {\textit{priorCommit}(#1, #2)}
\newcommand{\evts}[1] {evts(#1)}
\newcommand{\ssch} {sub-history\xspace}
\newcommand{\sschs} {sub-historie\xspaces}
\newcommand{\serial} {serial\xspace}
\newcommand{\serialc} {serial criterion\xspace}
\newcommand{\svserial} {sv-serial\xspace}
\newcommand{\svsc} {sv-serial criterion\xspace}

\newcommand{\wrt}[2] {#2.wTrans(#1)}
\newcommand{\wtrans} {wTrans}
\newcommand{\cwrt}[2] {#2.cwTrans(#1)}
\newcommand{\cwtrans} {cwTrans}

\newcommand{\valid} {valid}
\newcommand{\validity} {validity}
\newcommand{\legal} {legal}
\newcommand{\legality} {legality}
\newcommand{\leg}[1] {#1\text{-}legal}

\newcommand{\tobj} {\emph{t-object}}
\newcommand{\gchist} {\textit{gComHist}}
\newcommand{\lchist} {\textit{lComHist}}
\newcommand{\thist} {\textit{tHist}}
\newcommand{\gchlock} {\textit{gLock}}
\newcommand{\gseqn}{\textit{gSeqNum}}
\newcommand{\cseq} {\textit{commitSeqNum}}
\newcommand{\rseq} {\textit{readSeqNum}}
\newcommand{\lseq} {\textit{lseq}}
%\newcommand{\tryc} {\textit{tryC}}
%\newcommand{\trya}{\textit{tryA}}
\newcommand{\rvar} {\textit{readVar}}
\newcommand{\rop} {\textit{rop}}
\newcommand{\wvar} {\textit{writeVar}}
\newcommand{\wop} {\textit{wop}}
\newcommand{\cvar} {\textit{comVar}}
\newcommand{\cop} {\textit{cop}}

\newcommand{\co} {CO\xspace}
\newcommand{\opq} {opaque\xspace}
\newcommand{\opaq}[1] {#1\text{-}opaque\xspace}
%\newcommand{\opaq}[1] {#1-opaque}
\newcommand{\opaty}[1] {#1\text{-}opacity\xspace}
%\newcommand{\opaty}[1] {#1-opacity}
\newcommand{\opty} {opacity\xspace}
\newcommand{\coop} {co-opaque\xspace}
\newcommand{\coopty} {co-opacity\xspace}

\newcommand{\sble} {serializable\xspace}
\newcommand{\sbty} {serializability\xspace}
\newcommand{\lble} {linearizable\xspace}
\newcommand{\lbty} {linearizability\xspace}


% Definitions for proof in this paper
\newcommand{\pref}[2] {#2.prefix(#1)}
\newcommand{\cpref}[2] {#2.comPrefix(#1)}
\newcommand{\compref} {comPrefix\xspace}

% Definitions needed for Garbage Collection
\newcommand{\liveset} {liveSet\xspace}
\newcommand{\primary} {primary\xspace}
\newcommand{\glset} {gIncSet\xspace}
\newcommand{\waits} {waitSet\xspace}
\newcommand{\dset} {dependSet\xspace}
\newcommand{\sstate} {system-state\xspace}
\newcommand{\obsolete} {obsolete\xspace}

%------------------------------------------------------------------------------------------------------------------
% Definitions for Multiversion timestamp ordering protocol paper
%------------------------------------------------------------------------------------------------------------------
\newcommand{\mvs} {multi-version STM}

\newcommand{\tseq} {t-sequential\xspace}
\newcommand{\opg}[2] {OPG(#1, #2)}
\newcommand{\ord}[1] {ord(#1)}
\newcommand{\ordfn} {ord}
\newcommand{\mv} {mv}
\newcommand{\rf} {rf}
\newcommand{\rt} {rt}
\newcommand{\mvto} {MVTO\xspace}
\newcommand{\bto} {BTO\xspace}
\newcommand{\memop} {memory operation\xspace}

\newcommand{\cc} {correctness-criterion\xspace}


\newcommand{\readi} {\emph{$read_i$}\xspace}
\newcommand{\cl} {\emph{confList}\xspace}
\newcommand{\writei} {stm\_write\xspace}
\newcommand{\tryci} {stm\_tryC\xspace}
%\newcommand{\tryc} {\emph{tryC}\xspace}
\newcommand{\tryc} {STM.tryC\xspace}
\newcommand{\tryai} {stm\_tryA\xspace}
%\newcommand{\trya} {tryA}
\newcommand{\trya} {STM.tryA}
\newcommand{\ok} {stm\_ok}

%\newcommand{\read} {stm\_read}
%\newcommand{\write} {stm\_write}
%\newcommand{\trya} {stm\_tryA}
%\newcommand{\ok} {stm\_ok}

\newcommand{\tcntr} {\emph{tCounter}\xspace}
\newcommand{\shl} {\emph{shl}\xspace}
\newcommand{\mr} {\emph{max\_r}\xspace}
\newcommand{\mw} {\emph{max\_w}\xspace}
\newcommand{\cminer} {Concurrent Miner\xspace}
\newcommand{\cvalidator} {Concurrent Validator\xspace}
\newcommand{\conminer} {\emph{concurrent miner}\xspace}
\newcommand{\convalidator} {\emph{concurrent validator}\xspace}
\newcommand{\Conminer} {\emph{Concurrent Miner}\xspace}
\newcommand{\Convalidator} {\emph{Concurrent Validator}\xspace}
\newcommand{\ConValidator} {\emph{Concurrent validator}\xspace}
\newcommand{\CG} {\emph{Conflict Graph}\xspace}
\newcommand{\cgraph} {\emph{conflict graph}\xspace}
\newcommand{\Cgraph} {\emph{Conflict graph}\xspace}
\newcommand{\bg} {block graph\xspace}
\newcommand{\aul} {\emph{auList[]}\xspace}
\newcommand{\confg} {\emph{confGraph}\xspace}
\newcommand{\gconfl} {\emph{getConfList}\xspace}
\newcommand{\vp} {\emph{vPred}\xspace}
\newcommand{\vc} {\emph{vCurr}\xspace}
\newcommand{\vn} {\emph{vNext}\xspace}
\newcommand{\ep} {\emph{ePred}\xspace}
\newcommand{\ec} {\emph{eCurr}\xspace}
\newcommand{\en} {\emph{eNext}\xspace}
\newcommand{\vl} {\emph{vList}\xspace}
\newcommand{\el} {\emph{eList}\xspace}
\newcommand{\inc} {\emph{inCnt}\xspace}
\newcommand{\txlog} {\emph{txlog}\xspace}
\newcommand{\adde} {\emph{addEdge}\xspace}
\newcommand{\addv} {\emph{addVert}\xspace}
\newcommand{\egn} {\emph{eNode}\xspace}
\newcommand{\vgn} {\emph{vNode}\xspace}
\newcommand{\enode} {\emph{eNode}\xspace}
\newcommand{\vnode} {\emph{vNode}\xspace}
\newcommand{\searchl} {\emph{searchLocal}\xspace}
\newcommand{\searchg} {\emph{searchGlobal}\xspace}
\newcommand{\bc} {blockchain\xspace}
\newcommand{\BC} {Blockchain\xspace}
\newcommand{\scontract} {smart contract\xspace}
\newcommand{\SContract} {smart contract\xspace}
\newcommand{\Scontract} {Smart contract\xspace}
\newcommand{\au} {atomic-unit\xspace}
\newcommand{\miner} {miner\xspace}
\newcommand{\validator} {validator\xspace}
\newcommand{\Miner} {miner\xspace}
\newcommand{\Validator} {validator\xspace}
\newcommand{\exec} {\emph{executeCode}\xspace}
%\newcommand{\hb} {happens-before\xspace}
\newcommand{\bp} {block\text{-}producer\xspace}


\newcommand{\nc} {\emph{nCount}\xspace}
\newcommand{\gn} {\emph{gNode}\xspace}
\newcommand{\vt} {\emph{vTail}\xspace}
\newcommand{\vh} {\emph{vHead}\xspace}
\newcommand{\eh} {\emph{eHead}\xspace}
\newcommand{\et} {\emph{eTail}\xspace}
\newcommand{\tl} {\emph{thLog}\xspace}
\newcommand{\cachel} {\emph{cacheList}\xspace}
\newcommand{\vmain} {\emph{validatorMain}\xspace}
\newcommand{\opt} {\emph{Opt}\xspace}
\newcommand{\vtuple} {\emph{v\_tuple}\xspace}
\newcommand{\dtuple} {\emph{d\_tuple}\xspace}
\newcommand{\ctuple} {\emph{c\_tuple}\xspace}
\newcommand{\livel} {liveList\xspace}
\newcommand{\begtrans} {\emph{begin}\xspace}
\newcommand{\checkv} {check\_versions\xspace}
\newcommand{\init} {\emph{initialize}\xspace}
\newcommand{\find} {find\_lts\xspace}
\newcommand{\instup} {ins\_tuple\xspace}
\newcommand{\remid} {removeId\xspace}
\newcommand{\gc} {gc\xspace}

\newcommand{\cg}[1] {CG(#1)}

\newcommand{\mvve} {MVVE\xspace}
\newcommand{\vie} {VE\xspace}
\newcommand{\ce} {CE\xspace}

\newcommand{\gen}[1] {gen(#1)}
\newcommand{\mlive} {maxLiveSet}
\newcommand{\maxl}[1] {maxLiveSet(#1)}
\newcommand{\prefs}[1] {prefixSet(#1)}


% Definitions for the pseudocode
%\algrenewcommand{\algorithmiccomment}[1]{\hskip3em$//$ #1}
%\algrenewcommand{\algorithmiccomment}[1]{$//$ #1}
\newcommand{\rs}{rset\xspace}
\newcommand{\ws}{wset\xspace}


%\newcommand{\init} {init\xspace}
%\newcommand{\begt} {tbegin\xspace}
%\newcommand{\tread} {stm\text{-}read\xspace}
%\newcommand{\twrite} {stm\text{-}write\xspace}

\newcommand{\begt} {STM.begin\xspace}
\newcommand{\tread} {STM.read\xspace}
\newcommand{\twrite} {STM.write\xspace}

%\newcommand{\tryc} {tryC\xspace}
%\newcommand{\trya} {tryA\xspace}
\newcommand{\tmth} {stm\text{-}method\xspace}
\newcommand{\commit}{\mathcal{C}}
\newcommand{\abort}{\mathcal{A}}
%\newcommand{\op} {operation\xspace}
\newcommand{\mth} {method\xspace}


\newcommand {\incomp}[1] {#1.incomp}
\newcommand {\live}[1] {#1.live}

\newcommand{\shist}[2] {#2.subhist(#1)\xspace}
\newcommand{\subhist} {subhist\xspace}
\newcommand{\subhs} {subhistSet\xspace}
\newcommand{\shset}[1] {#1.subhistSet\xspace}

\newcommand{\mMiner}{\emph{LeaderMiner}\xspace}
\newcommand{\wMiner}{\emph{FollowerMiner}\xspace}
\newcommand{\mVal}{\emph{LeaderValidator}\xspace}
\newcommand{\wVal}{\emph{FollowerValidator}\xspace}


\newcommand{\dval}{\emph{DefaultValidator}\xspace}
\newcommand{\sval}{\emph{SharingValidator}\xspace}

\newcommand{\dVal}{\emph{Default Validator}\xspace}
\newcommand{\sVal}{\emph{Sharing Validator}\xspace}


\definecolor{celadonGreen}{rgb}{0.67, 0.88, 0.69}
%%%%%Below new commands are used for circle and rectangle around the character/text 
\newcommand\circledm[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=.1pt, fill=gray!25] (char) {#1};}}
\newcommand\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=.1pt, fill=orange!60] (char) {#1};}}
\newcommand\circleVal[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=.1pt, fill=yellow!35] (char) {#1};}}
\newcommand\circledsd[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=.4pt, fill=celadonGreen] (char) {#1};}}
\newcommand\circledphase[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=.2pt, fill=cyan!15] (char) {#1};}}
\newcommand\Otherbox[1]{\tikz[baseline=(char.base)]{\node[shape=rectangle,draw,inner sep=.7pt, fill=lime!15] (char) {#1};}}
%%% Coloring the comment as blue
\newcommand\mycommfont[1]{\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
% *** SUBFIGURE PACKAGES ***
%\usepackage[caption=false]{subfig}
%\pagestyle{plain}
%\usepackage[font=small,labelfont=bf]{caption}


==> Arxiv on-13-3-2021/proposedwork.tex <==
\section{Proposed Framework}
\label{methodology}

This section presents the proposed \emph{DiPETrans} framework. We first provide an overview of the architecture that describes the functionalities of the miner and the validator. Following that, the leader-follower approach of a mining community is illustrated. Finally, the algorithms for static analysis of transactions and distributed mining are explained.

%\todo[inline]{YS: The following para is repetitive with the solution approach in the introduction. Drop.}
%\sout{At a higher level, \emph{DiPETrans} determines the dependencies between the transaction using static analysis (pre-processing) to keep them in different shard first at the miner while creating a block and later at the validator while validating a block. The dependent transactions are grouped into different shards (as shown in \emph{Figure \ref{fig:ds}}), and after that, different shards are executed parallelly by the members of the community. However, transactions within a shard may have dependencies and executed serially. Essentially, the transactions within a shard are strictly ordered; however, across the shards, there is no order. It means shards can be executed in any order while within a shard transaction must be executed serially at least in the current implementation of the \emph{DiPETrans}. In \emph{DiPETrans}, a distributed mining pool based leader-follower approach is developed to execute the shards parallelly. The static analysis may introduce small overhead but improves overall performance.} %Based on the statical analysis, non-conflicting transactions are grouped to different shards and can be executed parallelly at the miner and validator to achieve higher throughput.



%At a higher level, \emph{DiPETrans} determines the dependencies between the transaction using statical analysis to keep them in different shard at the miner (while creating a block) and at the validator (while validating a block). The dependent transactions are grouped into the same shard, and different shards are executed parallelly. However, transactions within a shard may have dependencies and executed serially.
%The transaction dependencies are determined by pre-processing (static analysis) beforehand. Static analysis may introduced small overhead, but it will improve overall performance. So we can parallelly execute non-conflicting transactions belonging to different shards at the miner and validator to achieve higher throughput. Essentially, the transactions within a shard are strictly ordered; however, across the shards, there is no order. It means shards can be executed in any order while within a shard transaction must be executed serially at least in the current implementation of the \emph{DiPETrans}. A distributed mining pool based approach is developed to execute the different shards parallelly.

%As explained transaction dependencies are determined by pre-processing (static analysis) the block transactions beforehand. The static analysis may introduce small overhead but improves overall performance. Based on the statical analysis, non-conflicting transactions are grouped to different shards and can be executed parallelly at the miner and validator to achieve higher throughput. Essentially, the transactions within a shard are strictly ordered; however, across the shards, there is no order. It means shards can be executed in any order while within a shard transaction must be executed serially at least in the current implementation of the \emph{DiPETrans}. In \emph{DiPETrans}, a distributed mining pool based approach is proposed to execute the different shards parallelly.

%Shard transactions are executed serially, so there will be no consistency issues.% Also, we can execute different shard in any order because the final state will always be the same.
%As parallel execution of non-conflicting transactions also leads to the same final state. Achieving parallelism at the data objects level is a complex problem and will require frequent message passing between the nodes which may degrade the performance of miner in terms of block creation time and block size. The miner may store additional information into the block to help the validator to avoid the overhead associated with statical analysis, but it may increase the block size.





\subsection{DiPETrans Architecture}

%The architecture of the \emph{DiPETrans} framework is shown in \figref{arch}. There are different peers acting as distributed system or mining community. Each community is a set of devices (workers) which use their distributed compute power collaboratively to execute transactions and solve the PoW in parallel for a block. Workers in a community trust each other. As with existing mining pools, all workers in a community that participates in the parallel mining of a block get a part of the incentive fee, based on pre-agreed conditions. 

\figref{arch} shows the architecture of the \emph{DiPETrans} framework. It shows two mining communities, one acting as a miner node and the other as a validator node in the blockchain. Each community internally has multiple computing servers that use their distributed compute power collaboratively to execute transactions and solve the PoW in parallel for a block. The resources can all be owned by the same user, or they may participate in parallel mining and get a part of the incentive fee based on pre-agreed conditions.

%\figref{arch} shows the architecture of the \emph{DiPETrans} framework. It shows two mining communities, one acting as a miner node and the other as a validator node in the blockchain. Each community internally has multiple computing servers, that use their distributed compute power collaboratively to execute transactions and solve the PoW in parallel for a block. The resources can all be owned by the same user, or they may participate in parallel mining and get a part of the incentive fee based on pre-agreed conditions. 



One of the community workers is identified as the \emph{Leader}, while the others are \emph{Followers}. The \emph{Leader} represents the community and appears as a single peer in the blockchain network for all operations. Thus each peer of the blockchain in our architecture is the \emph{Leader} of its respective community. %We developed a similar approach to propose a technique for parallel execution of the block transactions. % to improve the throughput and to reduce the transaction latency along with parallel PoW. %The mining pool based approach also allows the resource constraint miner to participate in mining to get the incentive.
 %The community interacts with the public network with a single interactive address representing the miner/validator (leader address). 
When the user submits transaction request to one of the peers in the blockchain, the transaction is broadcast to every peer, including the \emph{Leader} of each community. The broadcasted transaction is then placed in the pending transaction queue of the respective peers (\figref{arch}(a), \circled{1}). Then all the miner peers in the blockchain compete to form the next block from these transactions. % and increase their chance of earning the rewards.


%\subsubsection{Functions of the Miner}
\subsubsection{Community Acting as Miner}
The leader node is responsible for coordinating the overall functionality of the community ({\figref{arch}(a)} \circled{2}). It can be selected based on a leader election algorithm or some other approach. We assume that there are no server failures within the community. When the community acts as a miner to create new blocks, there are two phases: one is transaction execution (\figref{arch}(a) \circledphase{\large{i}}), and the other is solving the PoW (\figref{arch}(a) \circledphase{ii}). Both of these are parallelized; however, phase 2 may not be needed for permissioned blockchains.

In the first phase, the leader selects the transactions from the pending transaction queue of the community (\circled{1}) to construct a block (\circled{3}). Then, it identifies the independent transactions by performing a static analysis of the transactions (discussed later in \algoref{analyze}). It groups dependent transactions into a single shard and independent ones across different shards (\circled{4}). The leader then sends the shards to the followers, along with the current state of the accounts (stateful variables) accessed by those transactions (\circled{5}, \circled{6}). 

\begin{figure}[t!]
	\centering
	{\includegraphics[width=1\textwidth]{figs/DiPETransV5.pdf}}
	%\vspace{-.05cm}
	\caption{Overview of the DiPETrans architecture}
	%\todo[inline]{YS: rename "pending transaction pool" as "Pending transaction queue" to avoid confusion with "mining pool"\newline
	%Rename "worker" as "follower" to be consistent. In our text, we treat both leader and Follower as workers.}
	%\ysnote{Remove "While Proposing Block" and "While Validating Block". Instead, at the top where you say "Community", add a second line \emph{(Acting as Miner)} and \emph{(Acting as Validator)} respectively.}
	%\ysnote{Have the legend in the bottom span the entire width and increase the font sizes}
	\label{fig:arch}
	%\vspace{-.5cm}
\end{figure}
%%\vspace{-.8cm}


On receiving a shard from the leader, the follower (worker) executes the transactions present in its shard serially (\circled{5}), computes the new state for the accounts locally, and sends the results back to the leader. While transactions across shards are independent, those within a shard may have dependencies (\figref{ds}), and hence are executed sequentially. To improve the throughput further, one can perform concurrent execution of transactions within a shard based on Software Transactional Memory (STM) to leverage multi-processing on a single device (follower)~\cite{Dickerson+:ACSC:PODC:2017,Anjana:OptSC:PDP:2019,Anjana:DBLP:journals/corr/abs}. This is left as a future extension. Once all followers complete the execution of the shards assigned to them, the leader computes the block's final state from the local states returned by the followers.

In the PoW phase of the miner (\circled{7}, \circledphase{ii}), the leader sends the block header and transactions, and different nonce ranges to the followers. Each partition forms a solution space that a follower examines to find the block hash that is smaller than the target hash. %\spnote{What is the meaning of this - that is smaller than the required difficulty? Difficulty of PoW cannot be smaller by distributed execution.}\psnote{It means that the block hash should be smaller than the target hash. The followers try to find block hash smaller than target hash.} 
This is an iterative brute-force approach that is computationally intensive. When a follower finds the correct hash, it informs the leader. The leader then notifies the remaining workers to terminate their computation. The leader proposes the block with the executed transactions and the PoW, updates its local chain (\circled{8}), and broadcasts it to all peers in the blockchain network for validation. A successful validation by a majority of peers and the addition of the block to the consensus blockchain will result in the mining community receiving the incentive fee for that block.

%\subsubsection{Functions of the Validator}
\subsubsection{Community Acting as Validator}
When the community acts as a validator, its first phase is similar to the miner, while in its second phase, it just validates the PoW done by the miner.

After receiving a block from a miner ({\figref{arch}}(b) \circleVal{9}), the remaining peers of the blockchain network serve as its validators. They validate the block by re-executing the transactions present in the block and check if the PoW hash matches. Verifying the PoW hash is computationally cheap. The transaction re-execution is identical to the first phase of mining ({\figref{arch}}(b) \circleVal{9} -- \circleVal{\footnotesize{15}}, \circledphase{\large{i}}), and use the same \algoref{analyze} for static analysis of the dependencies themselves. We will call such validator as \emph{Default Validator} (We will explain other validators later). They then verify if the block contains the correct PoW solution (\figref{arch}(b) \circledphase{ii}), and validate the final state computed by them based on their local chain with the final state supplied by the miner in the block ({\figref{arch}(b)} \circleVal{\footnotesize{13}}). If the final state computed does not match with the final state in the block stored by the miner, then the block is rejected. The miner does not get any incentive in this case. 

%\ysnote{Why is the "Pending transaction queue (G)" relevant above? Is there the equivalent of a "Pending Block Queue" for a list of blocks to be validated? Need to possibly include that in figure and text above}
%\psnote{A client transaction is broadcasted in the network so it will go to every peer "Pending transaction queue". When a peer acts as a validator, he validates a block, and after successful validator and majority consensus, the validator needs to remove the recently accepted block transaction from his "Pending transaction queue (G)" (i.e., in step G). In another case, when a validator acts as a miner, he selects the transaction from his "Pending transaction queue (3)" and tries to propose a new block.}


%{\color{red}\sout{We take two different approaches for the validation. In the first, miner offer hints on the dependency information as part of the transactions in the block with the validators. Specifically, the miner includes the shard ID for each transaction in the $other$ field of the block ({Figure \ref{fig:arch}} \Otherbox{O}), and this can directly be used by the validator to shard the transactions for parallel validation. This avoids a call to Alg.~\ref{alg:analyze} by each validator in the blockchain network. We refer to these as \emph{Sharing Validators}. The second approach is the \emph{Default Validator}, and here no additional details about shards are included in the block. The validator, if part of a community, may use the same Alg.~\ref{alg:analyze} for static analysis of the dependencies themselves, or if a stand-alone validator may validate the transactions sequentially.}}

Alternatively, a validator can also execute the transactions serially if they are not part of any community, i.e., \emph{stand-alone validators}. Yet another approach for the validator is that miners encode hints on the transaction dependency as part of the block~\cite{Dickerson+:ACSC:PODC:2017,Anjana:OptSC:PDP:2019,Anjana:DBLP:journals/corr/abs}, which allows the validators to avoid performing the static analysis again. Specifically, the miner includes the shard ID for each transaction in the $other$ field of the block ({\figref{arch}} \Otherbox{O}), and this can directly be used by the validator to shard the transactions for parallel validation. We refer to these as \sVal{s}. But, the problem here is that the miners can encode an invalid transaction dependency information that can cause the validation to be incorrect~\cite{Anjana:DBLP:journals/corr/abs}. This problem does not arise in our default validator since the static analysis is done independently by them. In our experiments, we compare the performance benefit of these approaches.

%This avoids a call to Alg.~\ref{alg:analyze} by each validator in the blockchain network. 

%We take two different approaches for the validation. In the first, miner offer hints on the dependency information as part of the transactions in the block with the validators. Specifically, the miner includes the shard ID for each transaction in the $other$ field of the block ({Figure \ref{fig:arch}} \Otherbox{O}), and this can directly be used by the validator to shard the transactions for parallel validation. This avoids a call to Alg.~\ref{alg:analyze} by each validator in the blockchain network. We refer to these as \emph{Sharing Validators}. The second approach is the \emph{Default Validator}, and here no additional details about shards are included in the block. The validator, if part of a community, may use the same Alg.~\ref{alg:analyze} for static analysis of the dependencies themselves, or if a stand-alone validator may validate the transactions sequentially. %\ysnote{note that i've renamed the validators to "Sharing Validators" and "Default Validators". Check if other places need to be replaced as well.}

%So in the first approach known as \emph{Sharing Validator,} miner includes the sharding information in $other$ ({Figure \ref{fig:arch}} \Otherbox{O}) field of the block before sending it to validators. This approach may need some extra bytes to store dependency information in the block but might improve validator performance. However, in another approach known as \emph{no Info Sharing Validator,} the miner does not share any dependency information and validator needs to determine dependencies using static analysis.


%In the current implementation, we fixed our topology as one miner and two validator communities. The miner and validator community can have 1-5 workers other than the leader. We have chosen one of the nodes of the community as a leader, and the rest nodes as workers.
%{\color{blue}
%}


\subsubsection{Sharding of the Block Transactions}
\label{shardingBlock}
Sharding is the process of identifying and grouping the dependent transactions in a block, with one shard created per group. This is illustrated in \figref{ds}, which lists a sequential list of transactions that are received at a node. 
%}, all the dependent transactions are grouped into one shard and executed serially; however, the unrelated transactions belong to different shards and are executed parallelly by different workers. 
Transaction $T_1$ accesses the account (stateful variable) \emph{A$_1$} and \emph{A$_3$}, \emph{T$_5$} accesses \emph{A$_1$} and \emph{A$_8$}, while \emph{T$_7$} accesses \emph{A$_2$} and \emph{A$_3$}. Since \emph{T$_1$, T$_5$}, and \emph{T$_7$} are accessing common accounts, they are dependent on each other and grouped into the same shard, \emph{Shard$_{1}$}. Similarly, transactions \emph{T$_2$, T$_3$}, and \emph{T$_9$} are grouped into \emph{Shard$_{2}$}, while \emph{T$_4$, T$_6$,} and \emph{T$_8$} are grouped into \emph{Shard$_{3}$}. Transactions in each shard are independent from those in other shards, and each shard can be executed in parallel by different followers of the community. However, transactions within a shard must be executed in the original order in which they arrived.%The proposed technique assumes that there is no nested call between the transactions, i.e., one contract does not internally call another contract, which prevents a static analysis based on just the inputs to the transactions.% In the presence of nested transaction calls, the technique will not work.


%%\vspace{.08cm}
%\noindent
%\textbf{\emph{Algorithm Analyze().~}}
%By using \emph{Analyze()} leader performs static analysis of the block transactions to determine disjoint (non-conflicting). The shards are assumed to have no cross-dependencies. 
% \ysnote{Pls illustrate this graph as part of Fig 2. We can rearrange to show the shards horizontally in the top right and the graph in the bottom right.}
% \psnote{done sir.}

\begin{figure}[!t]
	%\vspace{-.25cm}
	\centering
	{\includegraphics[width=.7\columnwidth]{figs/Distributed_execution_V9.pdf}}
	%%\vspace{-.6cm}
	\caption{Sharding of transactions in a block using static graph analysis}
	%\caption{Block transaction sharding.}
	%\ysnote{Rename "I/P metadata" as "Accounts Accessed". The arrow direction for dependencies are reversed. T5 and T7 are dependent on T1. Switch them.}
	\label{fig:ds}
	%\vspace{-.25cm}
\end{figure}
\begin{algorithm}%[!t]
	%\scriptsize
	{
		\SetAlgoLined
		\KwData{txnsList}
		\KwResult{sendTxnsMap}
		\SetKwFunction{FWCC}{WCC}
		\SetKwFunction{FSJF}{SJF}
		\SetKwProg{Pn}{Procedure}{:}{\KwRet $sendTxnsMap$}
		\SetKwFunction{FAnalyze}{Analyze}
		\SetKwFunction{FLoadBalance}{LoadBalance}
		
		\Pn{\FAnalyze {$txnsList$}}{
			\tcp{Prepare AdjacencyMap, ConflictMap, AddressList to find WCC}
			
			Map$<$address,List$<$txID$>>$ conflictMap;
			
			Set$<$address$>$ addressSet;
			
			Map$<$address,address$>$ adjacencyMap;
			
			\For{$tx \in txnsList$}{
				
				conflictMap[tx.from].put(tx.txID);
				
				conflictMap[tx.to].put(tx.txID);
				
				addressSet.put(tx.from);
				
				addressSet.put(tx.to);
				
				adjacencyMap[tx.from].put(tx.to);
				
				adjacencyMap[tx.to].put(tx.from);
				
			}
			
			%\For{$adr \in AddressList$}{$visited[adr]$ = $false$;}
			Map$<$shardID, Set$<$txID$>>$ shardsMap;
			
			\tcp{Call to WCC till all addresses are visited}
			
			$shardsMap$ = \FWCC($addressSet$, $conflictMap$);
			
			Map$<$followerID, List$<$Transaction$>>$ sendTxnsMap;
			
			\tcp{Equally load balance the shards for followers}
			
			$sendTxnsMap$ = \FLoadBalance($shardsMap$, $followerList$, $txnsList$);
		}
		\caption{Analyze()}
		%    \ysnote{Give more details. This is the only algo worth having pseudocode for.}
		\label{alg:analyze}
	}
	%%\vspace{-.1cm}
\end{algorithm}
\begin{algorithm}%[!t]
	%\footnotesize
	{
	
		\SetAlgoLined
		\KwData{shardsMap, followerList, txnsList}
		\KwResult{sendTxnsMap}

		\SetKwFunction{FLoadBalance}{LoadBalance}
		\SetKwProg{Pn}{Procedure}{:}{\KwRet $sendTxnsMap$}
		
		\Pn{\FLoadBalance({$shardsMap$, $followerList$, $txnsList$})}{
			
			Map<int,List<Transaction>> $sendTxnsMap$ ;
			
			\tcp{Sort the shards in decreasing order of transaction count}
			
			$shardMap$ = sorted($shardMap$, reverse=True)
			
			\For{$ccID \in shardMap$}{
				\tcp{Find the followerID which has least number of transactions and assign them the shard transactions}
				
				Map<int,List<Transaction>>::iterator $it_1$, $it_2$;
				
				%\For{$it_1 \in sendTxnsMap.begin(); it_1 \neq sendTxnsMap.end(); it_1++$}
				\For{$it_1 \in sendTxnsMap$}{
					
					%\For{($it_2=sendTxnsMap.begin(); it_2 \neq sendTxnsMap.end(); it_2++$)}{
					\For{($it_2 \in sendTxnsMap$)}{
						
						\If{$it_1\rightarrow second.size() > it_2\rightarrow second.size()$}{
							
							\tcp{Follower id with least number of transactions}
							
							$id$ = $it_2\rightarrow first$ - $1$;
							
							\tcp{Assignment of shard transactions}
							
							\For{$txid \in shardMap[ccID]$}{
								
								sendTxnsMap[followerList[id].followerID].add(txnsList[txid];
							}
						}
					}
				}
			}
		}
		\caption{{LoadBalance( )}}%:\emph{ this algorithm is used to creates the new block and populate required information. It is called by the \mMiner.}}}
		\label{alg:lb}
	}
\end{algorithm}


We model the problem of finding the shards using static analysis (\algoref{analyze}) as a graph problem. Specifically, each \emph{account} serves as a \emph{vertex} in the \emph{transaction dependency graph}, identified by its \emph{address}. We introduce an \emph{undirected edge} when a transaction access two accounts, identified by its \emph{transaction ID}. A single transaction accessing $n$ addresses will introduce $\frac{n(n-1)}{2}$ edges, forming a clique among them. Next, we find the \emph{Weakly Connected Component (WCC)} in this dependency graph. Each component forms a single shard and contains the edges (transactions) that are part of that component. The transactions within a single shard are present in their sequential order of arrival. Transactions that are not dependent on any other transaction are not present in this graph and are placed in singleton shards. This is illustrated in \figref{ds}.%, right side.
%\ysnote{We dont appear to refer to Algorithm 1 in this part where it appears. It is referred to earlier in the text.}
%\spnote{Where is Algorithm 1 being referred to in this section?}
%\psnote{Now we referred Algorithm 1 at the beginning of the above pera.}
%transactions of different shards where \emph{vertices} are \emph{addresses} in transactions and \emph{edges} are transaction \emph{ids}. Within a block, transactions have unique \emph{ids}. 


\begin{comment}
The number of shards created may exceed the number of followers. In this case, we attempt to load-balance the number of transactions per follower. To achieve this, the leader sorts the shards in decreasing order of transaction count and assigns each shard to the follower with the least current load of transactions.
%assigns one shard to each follower in chronological order (shards are ordered in decreasing order of the number of transactions). \mVal then assigns the remaining shards to the followers based on the least number of transactions in the shards. 
As long as the number of shards is many and we do not have skewed shards with many transactions that can overlead a single worker by itself, this bin-packing algorithm
({Appendix~V-C: Algorithm 9 in~\cite{DiPETransArXiv2019}}) achieves load balancing.
%(Appendix~\ref{ap:bes} \algoref{lb})
\end{comment}

The number of shards created may exceed the number of followers. In this case, we attempt to load-balance the number of transactions per follower. {To achieve this, the leader sorts the shards in decreasing order of transaction count and assigns each shard to the follower with the least current load of transactions using \algoref{lb}.}
%assigns one shard to each follower in chronological order (shards are ordered in decreasing order of the number of transactions). \mVal then assigns the remaining shards to the followers based on the least number of transactions in the shards. 
As long as the number of shards is many and we do not have skewed shards with many transactions that can overlead a single worker by itself, this bin-packing algorithm achieves load balancing.
%(Appendix~\ref{ap:bes} \algoref{lb})

% \ysnote{are we using some bin packing algo for load balancing? Explaining in 1-2 lines.} \sbnote{done sir}

%{If the number of shards created exceeds the number of followers then we assign 1 shards to each of the followers in the sequential order (shards are ordered in decreasing order). Then we assign the remaining shards to the followers based upon the criteria of having the least number of transactions. In this way we achieve load balancing among the followers assuming there is no single shard which overloads any worker by itself.}



{For example, in experiments for a block with 100 transactions, there are $\approx 39$ shards and $\approx 6$ transactions in the largest shard on an average. Moreover, load balancing of the shards among the 5 followers results in each follower being assigned $\approx 25$ transactions (refer \figref{ShardsPerBlock} and \figref{transPerShard}).} Here, we assume that all transactions take the same execution time, which may not be true in practice since smart contract function calls may vary in latency, and be costlier than non-smart contract (monetary) transactions as we can observe that in the experiments section. However, if we have an estimate of the transaction duration, existing scheduling algorithms can be easily adapted to these as well. Similarly, heterogeneity in the computational capability of followers can be handled as well.
%%\vspace{-.4cm}
%\psnote{We will add plots on shards in the results section and reference those plots here in the above paragraph about shards information. Plots will be added for the number of shards in a block, afterload balancing shard allocation to followers, etc.}





\begin{figure}[!t]
	%%\vspace{-.2cm}
	\centering
	\includegraphics[width=1\columnwidth]{figs/SequenceDiagram_V9.pdf}
	%%\vspace{-.15cm}
	\caption{Sequence diagram of operations during mining and validation}
	%	\ysnote{Assuming we are dropping Sec III.C, rename the labels for the edges to be more descriptive. Its OK to split into two separate figures for mining and validation, taking 1 column each since we're saved space....
	%	b: Create block from transaction queue;
	%	c: Identify shards from block and load balance;
	%	d: Send shard(s) to followers;
	%	e: Execute transactions in shard sequentially;
	%	f: Return updated states to leader;
	%	g: Update global state;
	%	h: Send nonce range for PoW to followers;
	%	i: Try and solve PoW;
	%	j: Return solution if found;
	%	k: Broadcast block for verification;
	%	l: Optionally shard transactions in the block, and send to followers;
	%	Rest are good as they are.}
	\label{fig:seq}
	%\vspace{-.6cm}
\end{figure}


\subsection{Sequence of Operations}
{\figref{seq}} shows the sequence diagram for processing a block by a miner and a validator community in \emph{DiPETrans}. There are 4 roles as \mMiner, \wMiner, \mVal, and \wVal. At the top of \figref{seq}, we see the \mMiner starts the block execution by creating a block from the transaction queue. The created block consists of a set of transactions \circledsd{{b}}, including block specific information such as timestamp, miner details, nonce, hash of the previous block, final state, etc. The transactions of the block are formed into a dependency graph for static analysis. The WCC algorithm used to identify disjoint sets of transactions that form shards \circledsd{\large{c}}. Load balancing and mapping of shards to followers are done as well. The \mMiner then sends the shards to the follower devices in parallel \circledsd{{d}}, and these are executed locally on each follower \circledsd{\large{e}}. After successfully completing the transactions, each \wMiner sends the updated account states back to the \mMiner \circledsd{{f}}. The \mMiner updates its global account state based on the responses received from all the \wMiner{s} \circledsd{{g}}.
% (coin base address)



%%\vspace{-.6cm}
%\input{algo}
Once all \wMiner complete executing their assigned shards(s), the \mMiner switches to the PoW phase. It assigns followers the task of finding the PoW for different ranges of the nonce concurrently \circledsd{h}. The \wMiner searches the range to solve the PoW \circledsd{\large{i}} and returns a response either when the PoW is solved, or their nonce range has been completely searched \circledsd{{j}}. %\ysnote{We mention that the leader notifies followers to stop searching if the solution has been found by one of them. Is that the case? Not mentioned here.} \sbnote{When we receive the mining status from the worker, we do not send any notification to workers to stop the search. This has not been implemented as of yet.}
A successful detection of a solution by one follower causes the leader to terminate the PoW search on other followers.
Finally, the \mMiner broadcasts the block containing the transactions, the updated account states, the PoW, and optionally the mapping from shards to transactions (required for \sVal{s}) to the peers in the blockchain network for validation \circledsd{k}.


At the lower part of \figref{seq}, we see a \mVal receives a block to verify. It needs to re-execute the block transactions and match the resulting account states with those present in the block. For this \mVal, either use the shard information present in the block (\sVal{}) or, if not present, determine it using the same dependency graph approach as the \mMiner \circledsd{\large{c}}. \mVal uses the \sVal{} approach if it trusts the \mMiner. Then \mVal assigns the shards to the \wVal{s} \circledsd{{l}}. After successfully executing the transactions assigned by \mVal \circledsd{{m}}, each \wVal returns the account states back to the \mVal \circledsd{\large{n}}. The responses are verified by the \mVal with the states present in the block \circledsd{\large{o}}. The \mVal also confirms that miner has correctly found the PoW \circledsd{p}. After both these checks succeed, the \mVal accepts the block and propagates the message to reach the consensus.




==> Arxiv on-13-3-2021/relatedWork.tex <==
\section{Related Work}
%\section{Background and Related Work}
\label{relatedWork}
This section presents an overview of existing techniques to improve the throughput and performance of the blockchains. We first give a brief overview of the work on concurrent execution of the smart contracts then presents the work on sharding based techniques.

%This section presents the background and overview of existing parallel transaction execution techniques. We first introduce the working of blockchain technology and then summarize the work on parallel execution of the smart contract transactions. In the end, we present the work on sharding techniques.


%\vspace{.05cm}
%\noindent
%\textbf{Background: } 
% \ysnote{Drop the entire background sub-section. It has been covered in Intro and is repetitive. Rename section to "Related Work". Rephrase opening para of section to only focus on related work.} 
%\psnote{done.}
%In most of the popular blockchain systems such as Bitcoin~\cite{bitcoin:faq:2019} and Ethereum~\cite{Ethereum}, transactions in a block are executed in an ordered manner first by the miners later by the validators~\cite{Dickerson+:ACSC:PODC:2017}. When a miner creates a block, the miners typically choose transactions to form a block from a pending transaction queue based on their preference, e.g., giving higher priority to the transactions with higher fees. After selecting the transactions the miner (1) serially executes the transactions, (2) adds the final state of the system to the block after execution, (3) next find the PoW~\cite{PoW} and (4) broadcast the block in the network to other peers for validation to earn the reward. PoW is an answer to a mathematical puzzle in which miners try to find the hash of the block smaller than the given difficulty. %This technique is used in the Bitcoin and Ethereum. 




%Later after receiving a block, a node validates the contents of the block. Such a node is called the validator. Thus when a node $N_i$ is \bp, every other node in the system acts as a validator. Similarly, when another node $N_j$ is the miner, then $N_i$ acts as a validator. The validators (1) re-execute the transactions in the block received serially, (2) verify to see if the final state computed by them is same as the final state provided by the miner in the block, and (3) also validates if the miner solved the puzzle (PoW) correctly. The transaction re-execution by the validators is done serially in the same order as proposed by the miner to attain the consensus~\cite{Dickerson+:ACSC:PODC:2017}. After validation, if the block is accepted by the majority (accepted by more than 50\%) of the validators, the block is added to the blockchain, and the miner gets the incentive (in case Bitcoin and Ethereum).% However, it is also possible that multiple blocks are proposed and added to the chain at the same time, which creates the fork in the chain; but, the longest chain is considered as the consistent one.


%Further, blockchain is designed in such a way that it forces a chronological order between the blocks. Every block which is added to the chain depends on the cryptographic hash of the previous block. This ordering based on cryptographic hash makes it exponentially challenging to make any change to the previous blocks. To make any small change to already accepted transactions or a block stored in the blockchain requires recalculation of PoW of all subsequent blocks and acceptance by the majority of the peers. Also, if two blocks are proposed simultaneously and added to the chain, they form a \emph{fork}, the branch with the longest chain is considered as the final. This allows mining to be secure and maintain a global consensus based on processing power.



%\vspace{.05cm}
%\noindent
%\textbf{Related Work: } 
%\ysnote{Group related work into sub-sections}
%\psnote{done.}
%Since the launch of Bitcoin in 2008 by Satoshi Nakamoto~\cite{nakamoto2009bitcoin}, blockchain technology has received immense attention from researchers in both academia and industry. Blockchain was introduced as a distributed decentralized system of digital currency. However, decentralized digital and peer-to-peer currencies~\cite{eCash:1983,vishnumurthy2003karma, Yang:2003:PMP} have been introduced earlier as well. But none of them had a common global log stored at every peer, that makes Bitcoin's distributed blockchain ledger highly decentralized and secure. Later Ethereum~\cite{Ethereum} introduced smart contracts into the blockchain and this makes the technology versatile for generalized transactions over anything with value, such as as digital identity, energy market, supply-chain, healthcare, real estate, asset tokenization, etc. Many other blockchain platforms have subsequently developed smart contracts as well, such as EOS~\cite{eos:url}, Hyperledger~\cite{Hyperledger}, MultiChain~\cite{multichain}, OmniLedger~\cite{kokoris18omniledger}, RapidChain~\cite{zamani18rapidchain}, etc.

\subsection{Multi-threaded Techniques}
%\vspace{.03cm}
%\noindent
%\textbf{Multi-threaded Techniques: }
Several challenges prevent widespread adoption of the public blockchain, such as high transaction fees, poor throughput, high latency, and limited computation capacities~\cite{eos:url} as explained in \textsection\ref{introduction}. Also, most blockchain platforms execute the transaction serially, one after another, and fail to exploit the parallel execution provided by current-day multi-core systems~\cite{Dickerson+:ACSC:PODC:2017, Anjana:OptSC:PDP:2019}. Therefore to improve the throughput and to utilize parallelism available with multi-core systems, researchers have developed solutions to execute the transactions in parallel.

For the concurrent execution of the smart contract within the single multi-core system, Dickerson et al.~\cite{Dickerson+:ACSC:PODC:2017} and Anjana et al.~\cite{Anjana:OptSC:PDP:2019, Anjana:DBLP:journals/corr/abs} proposed software transactional memory based multi-threaded approaches. They achieve better speedup over serial execution of the transactions. However, their techniques are limited to concurrent smart contract transaction executions and based on the assumption of non-nested contract calls. Saraph et al.~\cite{Vikram:DBLP:journals/corr/abs} perform an empirical analysis and exploited simple speculative concurrency in Ethereum smart contracts using a lock-based technique. They group the transactions of a block into two bins -- one with non-conflicting transactions that can be executed concurrently, while another with conflicting transactions that are executed serially. Zang and Zang~\cite{ZangandZang:ECSC:WBD:2018} propose a multi-version concurrency control based concurrent validator in which miner can use any concurrency control protocol to generate the read-write set to help the validators to execute the transactions concurrently. In~\cite{bartoletti2019true}, Bartoletti et al. presented a statistical analysis-based theoretical perspective of concurrent execution of the smart contract transactions. 

In contrast, the solution we propose focuses on the distributed computing power across multiple servers to parallelly execute and verify the block transactions and determine the PoW. This complements concurrency techniques within a single machine.
%For the concurrent execution of the smart contract within the single multi-core system, Dickerson et al.~\cite{Dickerson+:ACSC:PODC:2017} and Anjana et al.~\cite{Anjana:OptSC:PDP:2019, Anjana:DBLP:journals/corr/abs} proposed software transactional memory based multi-threaded approaches. They achieve better speedup over serial execution of the transactions. However, their techniques are based on the assumption of non-nested transaction calls. Saraph et al.~\cite{Vikram:DBLP:journals/corr/abs} perform an empirical analysis and exploited simple speculative concurrency in Ethereum smart contracts using a lock-based technique. They group the transactions of a block into two bins -- one with non-conflicting transactions that can be executed concurrently, while another with conflicting transactions that are executed serially. Zang et al.~\cite{ZangandZang:ECSC:WBD:2018} propose a multi-version concurrency control based concurrent validator in which miner can use any concurrency control protocol to generate the read-write set to help the validators to execute the transactions concurrently. In~\cite{bartoletti2019true}, Bartoletti et al. presented a statistical analysis based theoretical perspective of concurrent execution of the smart contract transactions. In contrast, the solution we propose focuses on the distributed computing power across multiple servers to parallely execute and verify the block transactions, and determine the PoW. This complements concurrency techniques within a single machine.%, to increase the chances for a miner to propose new blocks. %In contrast, the solution we propose focuses on the distributed computing power to parallelly execute and verify the block transactions and to determine the PoW in parallel.

% \ysnote{you need a single line that says why your proposed approach is different/better than these. e.g. "In contrast, the solution we propose..."}
% \psnote{done sir.}


\subsection{Sharding-based Techniques}
%\vspace{.03cm}
%\noindent
%\textbf{Sharding-based Techniques: }
Mining pools use distributed computing power of multiple peers to find the PoW in parallel and share the incentive based on pre-agreed mechanisms, e.g., proportional, pay-per-share, and pay-per-last-N-shares~\cite{lewenberg2015bitcoin, MiningPools:NBERw25592}. Both centralized and decentralized mining pools are practically used in Bitcoin and Ethereum. E.g., in the Bitcoin, $\approx 95\%$ of the mining power resides with less than 10 mining pools, while 6 mining pools hold $\approx 80\%$ of the mining power in  Ethereum~\cite{Luu:SmartPool:usenix2017}. Our work goes beyond executing the PoW in parallel and utilizes the pool to execute and verify the transactions parallelly, without affecting the correctness.
% \ysnote{Again, contrast with our work. e.g. "Our work goes beyond executing the PoW in parallel, and utilizes the pool to also execute and verify the transactions concurrently, without affecting the correctness."}
% \psnote{done sir.}



Recent studies have focused on sharding based techniques to improve the blockchain's throughput and scalability. A majority of these divide the network into multiple clusters and work on the assumption that there is no malfunction in most of the nodes, e.g., there are no more than $t$ byzantine nodes in a cluster with $n$ nodes, where $n >> t$. Additionally, several sharding solutions use a leader-based BFT consensus protocol, including Tendermint~\cite{kwon2014tendermint}, Elastico~\cite{luu2016secure}, Hyperledger Fabric~\cite{androulaki2018hyperledger}, and RedBelly~\cite{crain2018RedBelly}. However, in the proposed work, we do not partition the network into different clusters. Instead, a node itself serves as a representative for a cluster of distributed resources. Moreover, there is no need to change underlining Blockchain consensus protocols, allowing drop-in replacement of our proposed solution into existing platforms.

% \ysnote{again, whats the difference from your work?}
% \psnote{done sir.}

% \ysnote{Elastico, RedBelly, RapidChain, OmniLedger, AHL, SharPer seem to have similar features and sound repetitive. Go in-depth on 1-2, and club the rest into a single para. Contrast them with your work.}


Elastico~\cite{luu2016secure} is a sharding-based open blockchain protocol where participants join various clusters at random. The PBFT consensus protocol is used by a leader-based committee to verify the cluster transactions and add a block to the global chain stored by all nodes. However, running PBFT on a large number of nodes reduces its performance and increases the probability of failure on a few nodes. 
Hyperledger Fabric~\cite{androulaki2018hyperledger}, the most widely used permissioned blockchain platform, introduces the concept of channels. Multiple nodes in the fabric form clusters called channels and the users submit their transactions to their channel. The channel nodes maintain the partitioned state of the whole system as they execute transactions. Different channels process the transactions in parallel to improve the performance.
 %\ysnote{again, whats the difference from your work?}
RedBelly~\cite{crain2018RedBelly} blockchain performs a partially synchronous consensus run by permissioned nodes to create new blocks, while permissionless nodes issue transactions. Usually, a transaction in a cluster is verified by all the nodes in the cluster. However, in RedBelly, this verification is done by between $t+1$ to $2t+1$ nodes in the cluster to improve throughput by committing more transactions per consensus instance, where $t$ is the maximum number of byzantine nodes in the cluster. 
RapidChain~\cite{zamani18rapidchain} is a completely trustless sharding-based blockchain that achieves high throughput through inter-shard transaction execution via block pipelining and gossiping protocol. However, it also requires reconfiguration by the block creators for robustness. 
OmniLedger~\cite{kokoris18omniledger} offers a protocol to assign nodes to different clusters and processes intra-shard transactions using a lock-based atomic consensus protocol based on a partial-synchrony assumption.
AHL~\cite{Dang:2019:TSBSS} proposes a trusted hardware-assisted solution to reduce the nodes in a cluster. Nodes are randomly assigned to clusters and can ensure high security much fewer nodes per cluster than OmniLedger.
SharPer~\cite{amiri2019sharper} uses flattened consensus protocol and maintains the chain as a directed acyclic graph where each cluster stores only a view of the chain and supports intra-shard and inter-shard transactions. %In contrast, the proposed approach follows a distributed leader--follower approach within a node of the existing blockchain such as Ethereum and Bitcoin. The leader shards the block transactions, and the followers parallelly execute (mining) or verify (validation) them. %Essentially, the transactions within a shard are ordered strictly; however, across the shards, there is no order. It means shards can be executed in any order while within a shard transaction must be executed serially.



%RedBelly~\cite{crain2018RedBelly} blockchain uses a partially synchronous consensus run by permissioned nodes to create new blocks, while permissionless nodes issue transactions. A set of proposer and verifier nodes are assigned to each group of transactions. Later multiple block creators combine different transaction groups to form a super block to improve throughput by committing more transactions per consensus instance. Usually, a transaction in a shard is verified by all the nodes assigned to the shard. However, in RedBelly, this verification is done by between $t+1$ to $2t+1$ nodes, where $t$ is the maximum number of byzantine nodes in the cluster.
% \ysnote{again, whats the difference from your work?}
% \ysnote{You seem to be incorrectly mixing up the term "shard" with "cluster" and "node". Shard is a unit of data/task while cluster/node are a computational resources. Each shard can be assigned to a cluster/node for processing. Pls recheck the new text in blue.}
% \psnote{done sir.}

%RapidChain~\cite{zamani18rapidchain} is a completely trustless sharding-based blockchain with the requirement that $\leq \frac{1}{3}$ of nodes assigned to process a shard have byzantine failures. It achieves high throughput through inter-shard transaction execution via block pipelining and gossiping protocol. However, it also requires reconfiguration by the block creators for robustness. OmniLedger~\cite{kokoris18omniledger} proposes a highly secure way to assign nodes to different clusters and processes intra-shard transactions using an atomic consensus protocol based on a partially-synchronous channel assumption. It requires active participation from the nodes for fast consensus, and its locking protocol may lead to blocking issues.
%\ysnote{again, whats the difference from your work?}

%Dang et al.~\cite{Dang:2019:TSBSS} proposed AHL, a trusted hardware-assisted solution to reduce the nodes in a cluster. Nodes are randomly assigned to clusters and can ensure high security much fewer nodes per cluster than OmniLedger~\cite{kokoris18omniledger}. Besides the BFT protocol, it requires a dedicated set of nodes to support cross-shard transactions, which results in high communication costs. SharPer~\cite{amiri2019sharper} divides permissioned blockchain nodes in multiple shards and assigns different data shards to different clusters of the node. The chain is maintained as a directed acyclic graph where each shard stores only a view of the chain and supports intra-shard and inter-shard transactions. Inter-shard transactions are processed by multiple shards simultaneously while intra-shard transactions by different shards based on flattened consensus protocol. 


%In the EOS blockchain~\cite{eos:url}, sharding is implemented for parallel execution of transactions at peers. Static analysis of the block is performed to determine the non-conflicting transactions in a block~\cite{bartoletti2019true, luu2016secure, al2017chainspace}. Two transactions that do not modify the common data item are grouped into different shards, and the shards of a block are executed concurrently using multiple threads, first by the miner and later during validation by the validators. However, this idea is not implemented yet in EOS blockchain. \ysnote{If it is not implemented, why are we describing this? It seems very similar to your work}


%\ysnote{This paragraph is good. You may just want to examine 1 system in each category that you list in this para in the above paras.}
In summary, the UTXO model is used to achieve the atomicity of cross-shard transactions without the use of a distributed commit protocol in OmniLedger~\cite{kokoris18omniledger}, RedBelly~\cite{crain2018RedBelly} and RapidChain~\cite{zamani18rapidchain}. However, RapidChain fails to achieve isolation, and OmniLedger causes blocking for cross-shard transactions. A few approaches support transactions that are cross-shard while others do not. Compared to AHL~\cite{Dang:2019:TSBSS}, SharPer~\cite{amiri2019sharper} uses the account-based model and allows cross-chain transactions using a global consensus protocol based on PBFT to achieve correctness. In contrast, Hyperledger Fabric~\cite{androulaki2018hyperledger} also supports the account-based model, but requires a trusted channel among the participants to execute cross-shard transactions. Moreover, almost all existing blockchains that focus on sharding divide the network into multiple clusters and process transactions independently, using variants of the BFT consensus protocol or atomic commit protocol to increase transaction throughput and achieve scalability for the dependent transaction.

%There are several other sharding based solutions such as Tendermint~\cite{kwon2014tendermint}, RSCoin~\cite{danezis2015centrally}, Chainspace~\cite{al2017chainspace}, Cosmos~\cite{frey2018cosmos}, PolyShard~\cite{li2018polyshard}, and Caper~\cite{amiri2019caper} proposed with several changes then the solutions explained. In summary, the UTXO model is used by OmniLedger~\cite{kokoris18omniledger}, RedBelly~\cite{crain2018RedBelly}, and RapidChain~\cite{zamani18rapidchain} to achieve the atomicity of cross-shard transactions without using a distributed commit protocol. However, RapidChain fails to achieve isolation, and OmniLedger has blocking issues for cross-shard transactions. A few solutions support cross-shard transactions, while others do not. SharPer~\cite{amiri2019sharper}, similar to AHL~\cite{Dang:2019:TSBSS}, uses the account-based model and perform cross-chain transactions using a PBFT based global consensus protocol to achieve correctness. In contrast, Fabric~\cite{androulaki2018hyperledger} also supports the account-based model but requires a trusted channel among the participants to process cross-shard transactions. Further, almost all existing sharding based blockchains divide the network into multiple clusters. Process the dedicated transaction of clusters independently and for the dependent transaction either use variants of BFT consensus protocol or atomic commit protocol to improve transaction throughput and to achieve scalability. 

In our proposed approach, we do not partition the network into different clusters. Instead, we follow a leader--follower approach among the distributed clusters of cooperating nodes, where the leader serves as a representative node in the existing blockchain network such as Bitcoin and Ethereum. The leader performs the static analysis of the transactions it receives to create shards, while the followers perform the computation over the different shards concurrently. The PoW is also solved in parallel. {This can be both permissioned or permissionless %The network leader  from the blockchain network to form multiple shards when acting as a miner community. Then executes different shards independently using followers in the network while transactions within shared are executed serially.
and can be done independently for the mining and the validation phases in a transparent manner.} The coordination overheads are minimal, as all nodes within a cluster are assumed to be trusted.
%Further, the clsuter solve the PoW parallelly similar to mining pools while creating a block. When a node act as a validator community in \emph{DiPETrans}, it verifies by re-executing the transactions of the block received from other miners parallelly by performing static analysis of the block transactions. The proposed solution can be adopted in mainstream blockchain systems without significant changes.
These allow \emph{DiPETrans} to be trivially adopted within existing blockchain systems {(permissioned or permissionless)} and benefit from parallel execution without the complexity of additional distributed consensus protocols while ensuring correctness.
%These allow DiPETrans to be trivially adopted within existing blockchain systems, and gain the benefits of parallel execution without the complexity of additional distributed consensus protocols. 



























%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%    Background and Related Work     %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}

\section{Background and Related Work}
\label{relatedWork}
This section presents the background and overview of existing parallel transaction execution techniques. We first introduce the working of blockchain technology and then summarize the work on parallel execution of the smart contract transactions. In the end, we present the work on sharding techniques.


\vspace{.05cm}
\noindent
\textbf{Background: } \ysnote{Drop the entire background sub-section. It has been covered in Intro and is repetitive. Rename section to "Related Work". Rephrase opening para of section to only focus on related work.}
In most of the popular blockchain systems such as Bitcoin~\cite{bitcoin:faq:2019} and Ethereum~\cite{Ethereum}, transactions in a block are executed in an ordered manner first by the miners later by the validators~\cite{Dickerson+:ACSC:PODC:2017}. When a miner creates a block, the miners typically choose transactions to form a block from a pending transaction queue based on their preference, e.g., giving higher priority to the transactions with higher fees. After selecting the transactions the miner (1) serially executes the transactions, (2) adds the final state of the system to the block after execution, (3) next find the PoW~\cite{PoW} and (4) broadcast the block in the network to other peers for validation to earn the reward. PoW is an answer to a mathematical puzzle in which miners try to find the hash of the block smaller than the given difficulty. %This technique is used in the Bitcoin and Ethereum. 

%In most of the popular blockchain system such as Bitcoin and Ethereum, transactions are executed in an ordered manner first by the \emph{miners} and later by the \emph{validators}~\cite{Dickerson+:ACSC:PODC:2017}, which are peers in the network. When a miner creates a block, they may choose to select the transactions based on their preference, e.g., giving higher priority to transactions with higher fees (incentive). So after selecting the set of transactions, the miner serially executes these transactions, adds the final state to the block after execution, finds the proof-of-work (PoW)~\cite{PoW}, and broadcasts the block to other peers in the network for validation to earn the reward. PoW solves a mathematical puzzle, necessarily by brute-force, where the miner finds the hash of the block that is smaller than the given difficulty. This is computationally challenging. It is required as a delay-wait on the network to help reach consensus and allow miners to create a new block in their favor.


%Later, after receiving a block, each validator re-executes the transactions in the block serially, verifies the final state computed by them with the final state provided by the miner in the block, and also validates that miner solved the PoW correctly -- verifying the PoW solution is cheap. The transaction re-execution by the validators is done serially, in the same order as listed in the block by the miner, to attain the consensus~\cite{Dickerson+:ACSC:PODC:2017}. After validation, if the block is accepted by a majority ($>50\%$) of the validators, the block is added to the blockchain by all, and the miner gets its fee.


Later after receiving a block, a node validates the contents of the block. Such a node is called the validator. Thus when a node $N_i$ is \bp, every other node in the system acts as a validator. Similarly, when another node $N_j$ is the miner, then $N_i$ acts as a validator. The validators (1) re-execute the transactions in the block received serially, (2) verify to see if the final state computed by them is same as the final state provided by the miner in the block, and (3) also validates if the miner solved the puzzle (PoW) correctly. The transaction re-execution by the validators is done serially in the same order as proposed by the miner to attain the consensus~\cite{Dickerson+:ACSC:PODC:2017}. After validation, if the block is accepted by the majority (accepted by more than 50\%) of the validators, the block is added to the blockchain, and the miner gets the incentive (in case Bitcoin and Ethereum).% However, it is also possible that multiple blocks are proposed and added to the chain at the same time, which creates the fork in the chain; but, the longest chain is considered as the consistent one.


Further, blockchain is designed in such a way that it forces a chronological order between the blocks. Every block which is added to the chain depends on the cryptographic hash of the previous block. This ordering based on cryptographic hash makes it exponentially challenging to make any change to the previous blocks. To make any small change to already accepted transactions or a block stored in the blockchain requires recalculation of PoW of all subsequent blocks and acceptance by the majority of the peers. Also, if two blocks are proposed simultaneously and added to the chain, they form a \emph{fork}, the branch with the longest chain is considered as the final. This allows mining to be secure and maintain a global consensus based on processing power.

%Blockchain is designed to force a chronological order between the blocks as every block added to the chain depends on the hash of the previous block. This ordering based on the cryptographic hash makes it exponentially challenging to make any change to the earlier blocks -- to make even a small change to an accepted transaction or a block in the blockchain requires recalculation of the PoW of all the subsequent blocks and their acceptance by a majority of the peers in the network. Also, if two blocks are proposed at the same time and added to the chain, they form the fork, miners work on the first block they receive and eventually switch to the longest chain. These allow mining to be secure and maintain a global consensus based on processing power.


\vspace{.05cm}
\noindent
\textbf{Related Work: } \ysnote{Group related work into sub-sections}
%There have been several attempts to develop digitize monetary systems for data storage and money transferred via the Internet without being double spent. 
Since the launch of Bitcoin in 2008 by Satoshi Nakamoto~\cite{nakamoto2009bitcoin}, blockchain technology has received immense attention from researchers in both academia and industry. Blockchain was introduced as a distributed decentralized system of digital currency. However, decentralized digital and peer-to-peer currencies~\cite{eCash:1983,vishnumurthy2003karma, Yang:2003:PMP} have been introduced earlier as well. But none of them had a common global log stored at every peer, that makes Bitcoin's distributed blockchain ledger highly decentralized and secure. Later Ethereum~\cite{Ethereum} introduced smart contracts into the blockchain and this makes the technology versatile for generalized transactions over anything with value, such as as digital identity, energy market, supply-chain, healthcare, real estate, asset tokenization, etc. Mny other blockchain platforms have subsequently developed smart contracts as well, such as EOS~\cite{eos:url}, Hyperledger~\cite{Hyperledger}, MultiChain~\cite{multichain}, OmniLedger~\cite{kokoris18omniledger}, RapidChain~\cite{zamani18rapidchain}, etc.


%Szabo~\cite{Nick:PublicN:journals:1997} in 1997, introduced the smart contract for securing and formalizing relationships on public networks. Ethereum~\cite{Ethereum} is one of the most popular blockchains that first adopted smart contract written in Turing complete language Solidity~\cite{Solidity}. Due to the introduction of smart contracts, blockchain becomes versatile and adopted for many other applications such as digital identity, energy market, supply-chain, healthcare, real estate, asset tokenization, etc. After that many blockchain platforms have been developed based on smart contracts such as EOS~\cite{eos:url}, Hyperledger~\cite{Hyperledger}, MultiChain~\cite{multichain}, OmniLedger~\cite{kokoris18omniledger}, and RapidChain~\cite{zamani18rapidchain}. 




There are challenges that prevent widespread adoption of the public blockchain, such as high transaction fees, poor throughput, high latency, and limited computation capacities~\cite{eos:url}. Also, most blockchain platforms execute the transaction serially, one after another, and fail to exploit the parallel execution provided by current-day multi-core systems~\cite{Dickerson+:ACSC:PODC:2017, Anjana:OptSC:PDP:2019}. Therefore to improve the throughput and to utilize parallelism available with multi-core systems, researchers have developed solutions to execute the transaction in parallel.



For the concurrent execution of the smart contract within the single multi-core system, Dickerson et al.~\cite{Dickerson+:ACSC:PODC:2017} and Anjana et al.~\cite{Anjana:OptSC:PDP:2019, Anjana:DBLP:journals/corr/abs} propose Software Transactional Memory based multi-threaded approaches. They achieve better speedup over serial execution of the transactions. However, their techniques are based on the assumption of non-nested transaction calls. Saraph et al.~\cite{Vikram:DBLP:journals/corr/abs} perform an empirical analysis and exploited simple speculative concurrency in Ethereum smart contracts using a lock-based technique. They group the transactions of a block into two bins -- one with non-conflicting transactions that can be executed concurrently, while another with conflicting transactions that are executed serially. Zang et al.~\cite{ZangandZang:ECSC:WBD:2018} propose a Multi-Version Concurrency Control based concurrent validator in which miner can use any concurrency control protocol to generate the read-write set to help the validators to execute the transactions concurrently. In~\cite{bartoletti2019true}, Bartoletti et al. presented a statistical analysis based theoretical perspective of concurrent execution of the smart contract transactions. \ysnote{you need a single line that says why your proposed approach is different/better than these. e.g. "In contrast, the solution we propose..."}




Mining pools use distributed computing power of multiple servers to find the PoW in parallel and share the incentive based on pre-agreed mechanisms, e.g., proportional, pay-per-share, or pay-per-last-N-shares~\cite{qin18mining, lewenberg2015bitcoin, MiningPools:NBERw25592}. Both  centralized and decentralized mining pools are practically used in both Bitcoin and Ethereum. E.g., tn the Bitcoin, $\approx 95 \%$ of the mining power resides with less than 10 mining pools, while $\approx 80\%$ of the mining power is held by 6 mining pools in  Ethereum~\cite{Luu:SmartPool:usenix2017}. %In mining pools, computation constraint miners participate in the mining to earn the rewards they cannot achieve independently. 
\ysnote{Again, contrast with our work. e.g. "Our work goes beyond executing the PoW in parallel, and utilizes the pool to also execute and verify the transactions concurrently, without affecting the correctness."}

%Furthermore, in sharding~\cite{luu2016secure} based techniques either overall system is partitioned into smaller equally sized committees or data (blockchain) is partitioned in such a way that a new node need not to validate entire chain instead validate only specific block from the chain. In EOS blockchain~\cite{eos:url}, concept of sharding is proposed to be implemented for parallel execution of the transaction. The static analysis of the block can be performed to determine the non-conflicting transactions in a block~\cite{bartoletti2019true, luu2016secure, Mustafa:DBLP:journals/corr/abs-1708-03778}. The two transactions that do not modify the common data item (account) grouped into different shards and different shards of the block executed parallelly. So transactions of a block belong to different shards executed concurrently using multiple threads first by the miner, later during validation by the validators. EOS~\cite{eos:url}, OmniLedger~\cite{kokoris18omniledger}, and RapidChain~\cite{zamani18rapidchain} proposed to provided optimization using sharding technique.



{\color{blue}


Recent studies have focused on sharding based techniques to improve the blockchain's throughput and scalability. A majority of these divide the network into multiple clusters, and work on the assumption that there is no malfunction in most of nodes, e.g., there are no more than $t$ byzantine nodes in a cluster with $n$ nodes, where $n >> t$. Additionally, several sharding solutions use a leader-based BFT consensus protocol, including Tendermint~\cite{kwon2014tendermint}, Elastico~\cite{luu2016secure}, Hyperledger Fabric~\cite{androulaki2018hyperledger}, and RedBelly~\cite{crain2018RedBelly}. \ysnote{again, whats the difference from your work?}

%To improve throughput and scalability of the blockchain, recent exhaustive studies focus on sharding based techniques. Most of the proposed sharding-based blockchains partition the network into multiple clusters. They are based on the assumption that a large percentage of nodes are non-faulty. It means there is a maximum of 't' byzantine node per cluster (shard) and the number of nodes (n) $>>$ t in the network. Further, several sharding-based solutions use leader-based BFT consensus protocols. The sharding based permissioned blockchains such as Tendermint~\cite{kwon2014tendermint}, Elastico~\cite{luu2016secure}, Hyperledger Fabric~\cite{androulaki2018hyperledger}, and RedBelly~\cite{crain2018RedBelly} uses a variant of BFT as consensus protocol.


%Elastico~\cite{luu2016secure} is sharding based protocol for open blockchain in which participants randomly joins different committees (clusters). Elastico uses the PBFT consensus protocol to process inter-shard transactions while it does not supports intra-shard transactions. A leader based committee verifies the shard transactions. It adds the global block in the chain, stored by all the Elastico nodes. The issue in the Elastico is that running PBFT on a large number of nodes decreases the performance and runs it on fewer nodes in a shard, increasing the probability of failure.

\ysnote{Elastico, RedBelly, RapidChain, OmniLedger, AHL, SharPer seem to have similar features and sound repetitive. Go in-depth on 1-2, and club the rest into a single para. Contrast them with your work.}

Elastico~\cite{luu2016secure} is a sharding-based open blockchain protocol where participants join various clusters at random. The PBFT consensus protocol is used by a leader-based committee to verify the shard transactions and add a block to the global chain stored by all  nodes. But running PBFT on a large number of nodes reduces its performance and increases the probability of failure on a few nodes. Hyperledger Fabric~\cite{androulaki2018hyperledger}, the most widely used permissioned blockchain platform, introduces the concept of channels. Multiple nodes in the fabric form clusters called channels, and the users submit their transactions to their channel which processess different shards. The channel nodes maintain the partitioned state of the whole system as they execute transactions. Different channels process the transactions in parallel to improve the performance.% while processing the intra-shard transactions is done through trusted participants between the channels. %  and supports pluggable components
\ysnote{again, whats the difference from your work?}


RedBelly~\cite{crain2018RedBelly} blockchain uses a partially synchronous consensus run by permissioned nodes to create new blocks, while permissionless nodes issue transactions. A set of proposer and verifier nodes are assigned to each group of transactions. Later multiple block creators combine different transaction groups to form a super block to improve throughput by committing more transactions per consensus instance. Usually, a transaction in a shard is verified by all the nodes assigned to the shard. However, in RedBelly, this verification is done by between $t+1$ to $2t+1$ nodes, where $t$ is the maximum number of byzantine nodes in the cluster.% similar to the Fabric~\cite{androulaki2018hyperledger} where each transaction needs several endorsements based on predefined endorsement policy of the channel.
\ysnote{again, whats the difference from your work?}

%Hyperledger Fabric~\cite{androulaki2018hyperledger} is the most commonly used permissioned blockchain platform that introduces the concept of channels (shards) and supports pluggable components. In Fabric channels are multiple clusters of the nodes, and transactions belonging to the dedicated cluster are processed by respective cluster nodes to maintain the full system's partitioned state. Different channels process the inter-shard transactions parallelly to improve the performance while processing the intra-shard transactions trusted participants required between the channels. 


%RedBelly~\cite{crain2018RedBelly} blockchain, proposed sharding based network partition using partially synchronous consensus run by permissioned nodes where permissionless nodes issue transactions. The permission node creates new blocks. In this blockchain for each group of transactions, a different set of block creator and verifier nodes are assigned. Later multiple block creators combine different groups of transactions to form a super block to improve throughput by committing more transactions per consensus instance. Usually, a transaction belongs to a shard is verified by all the nodes in the shared. Instead, in RedBelly blockchain, each transaction must be verified by at least $t + 1$ to $2t + 1$ nodes where $t$ is the maximum number of byzantine nodes in the cluster similar to the Fabric~\cite{androulaki2018hyperledger} where each transaction needs several endorsements based on predefined endorsement policy of the channel.% The new nodes in the network added by current deciders of the network based on BFT based consenses and a configuration block are recorded into the chain along with the transaction block. The reconfiguration is done periodically. It avoids the forking issue of the Bitcoin and Ethereum by adding new blocks in global blockchain deterministically.

\ysnote{You seem to be incorrectly mixing up the term "shard" with "cluster" and "node". Shard is a unit of data/task while cluster/node are a computational resources. Each shard can be assigned to a cluster/node for processing. Pls recheck the new text in blue.}

RapidChain~\cite{zamani18rapidchain} is a completely trustless sharding-based blockchain with the requirement that $\leq \frac{1}{3}$ of nodes assigned to process a shard have byzantine failures. It achieves high throughput through inter-shard transaction execution via block pipelining and gossiping protocol. However, it also requires reconfiguration by the block creators for robustness. % It also proposed an efficient technique to process cross-shard transactions. 
OmniLedger~\cite{kokoris18omniledger} proposes a highly secure way to assign nodes to different clusters and processes intra-shard transactions using an atomic consensus protocol based on a partially-synchronous channel assumption. It requires active participation from the nodes for fast consensus, and its locking protocol may lead to blocking issues.
\ysnote{again, whats the difference from your work?}


Dang et al.~\cite{Dang:2019:TSBSS} proposed AHL, a trusted hardware-assisted solution to reduce the nodes in a cluster. Nodes are randomly assigned to clusters and can ensure high security much fewer nodes per cluster than OmniLedger~\cite{kokoris18omniledger}.
%with 80 nodes per cluster, then the $\approx$ 600 nodes in OmniLedger~\cite{kokoris18omniledger}. 
Besides the BFT protocol, it requires a dedicated set of nodes to support cross-shard transactions, which results in high communication costs. SharPer~\cite{amiri2019sharper} divides permissioned blockchain nodes in multiple shards and assigns different data shards to different clusters of the node. The chain is maintained as a directed acyclic graph where each shard stores only a view of the chain and supports intra-shard and inter-shard transactions. Inter-shard transactions are processed by multiple shards simultaneously while intra-shard transactions by different shards based on flattened consensus protocol. 

%Another solution is SharPer~\cite{amiri2019sharper}, which divides permissioned blockchain nodes in multiple shards and assigns different data shards to different clusters of the node. The chain is maintained in the form of a directed acyclic graph, and each shard maintains only a view of the chain. Data shards are replicated on the multiple nodes and support intra-shard and inter-shard transactions. Inter-shard transactions are processed by multiple shards simultaneously while intra-shard transactions by different shards based on flattened consensus protocol to order cross-shard transactions. 




%In Fabric~\cite{androulaki2018hyperledger}, processing cross-shard transactions, in contrast to SharPer~\cite{ }, requires either the existence of a trusted channel among the participants or an atomic commit protocol (inspired by two-phase commit). Similarly, in Cosmos~\cite{ }, interacting chains in any inter-blockchain communication must be aware of each other's state, which requires establishing a bidirectional trusted channel between two blockchains. Random configuration of the communities in most sharding-based blockchains such as RedBelly~\cite{crain2018RedBelly}, Fabric~\cite{androulaki2018hyperledger}, and Elastico~\cite{luu2016secure} halts the entire network, which results in considerable overhead and latency issues.

In the EOS blockchain~\cite{eos:url}, sharding is implemented for parallel execution of transactions at peers. Static analysis of the block is performed to determine the non-conflicting transactions in a block~\cite{bartoletti2019true, luu2016secure, al2017chainspace}. Two transactions that do not modify the common data item are grouped into different shards, and the shards of a block are executed 
%parallelly. So transactions of a block belong to different shards executed 
concurrently using multiple threads, first by the miner and later during validation by the validators. However, this idea is not implemented yet in EOS blockchain. \ysnote{If it is not implemented, why are we describing this? It seems very similar to your work}



%There have been a number of additional sharding solutions proposed with some variation, such as: Tendermint~\cite{kwon2014tendermint}, RSCoin~\cite{danezis2015centrally}, Chainspace~\cite{al2017chainspace}, Cosmos~\cite{frey2018cosmos}, PolyShard~\cite{li2018polyshard}, and Caper~\cite{amiri2019caper}. 
\ysnote{This paragraph is good. You may just want to examine 1 system in each category that you list in this para in the above paras.}
In summary, the UTXO model is used to achieve atomicity of cross-shard transactions without the use of a distributed commit protocol in OmniLedger~\cite{kokoris18omniledger}, RedBelly~\cite{crain2018RedBelly} and RapidChain~\cite{zamani18rapidchain}. However, RapidChain fails to achieve isolation, and OmniLedger causes blocking for cross-shard transactions. A few approaches support transactions that are cross-shard while others do not. Compared to AHL~\cite{Dang:2019:TSBSS}, SharPer~\cite{amiri2019sharper} uses the account-based model and allows cross-chain transactions using a global consensus protocol based on PBFT to achieve correctness. In contrast, Fabric~\cite{androulaki2018hyperledger} also supports the account-based model, but requires a trusted channel among the participants to execute cross-shard transactions. Moreover, almost all existing blockchains that focus on sharding divide the network into multiple clusters and process these transactions independently, using variants of the BFT consensus protocol or atomic commit protocol to increase transaction throughput and achieve scalability for the dependent transaction.

%There are several other sharding based solutions such as Tendermint~\cite{kwon2014tendermint}, RSCoin~\cite{danezis2015centrally}, Chainspace~\cite{al2017chainspace}, Cosmos~\cite{frey2018cosmos}, PolyShard~\cite{li2018polyshard}, and Caper~\cite{amiri2019caper} proposed with several changes then the solutions explained. In summary, the UTXO model is used by OmniLedger~\cite{kokoris18omniledger}, RedBelly~\cite{crain2018RedBelly}, and RapidChain~\cite{zamani18rapidchain} to achieve the atomicity of cross-shard transactions without using a distributed commit protocol. However, RapidChain fails to achieve isolation, and OmniLedger has blocking issues for cross-shard transactions. A few solutions support cross-shard transactions, while others do not. SharPer~\cite{amiri2019sharper}, similar to AHL~\cite{Dang:2019:TSBSS}, uses the account-based model and perform cross-chain transactions using a PBFT based global consensus protocol to achieve correctness. In contrast, Fabric~\cite{androulaki2018hyperledger} also supports the account-based model but requires a trusted channel among the participants to process cross-shard transactions. Further, almost all existing sharding based blockchains divide the network into multiple clusters. Process the dedicated transaction of clusters independently and for the dependent transaction either use variants of BFT consensus protocol or atomic commit protocol to improve transaction throughput and to achieve scalability. 

In our proposed approach, we do not partition the network into different clusters. Instead, a node in the existing blockchain such as Bitcoin and Ethereum itself serves as a representative for a cluster of distributed resources. The leader acts is the representative node and performs the static analysis of the transactions it receives to create shards, while the followers perform the computation over the different shards concurrently. The PoW is also solved in parallel. This can be both permissioned or permissionless, %The network leader  from the blockchain network to form multiple shards when acting as a miner community. Then executes different shards independently using followers in the network while transactions within shared are executed serially.
and can be done independently for the mining and the validation phases in a transparent manner. The coordination overheads are minimal as all nodes within a cluster are assumed to be trusted.
%Further, the clsutersolve the PoW parallelly similar to mining pools while creating a block. When a node act as a validator community in \emph{DiPETrans}, it verifies by re-executing the transactions of the block received from other miners parallelly by performing static analysis of the block transactions. The proposed solution can be adopted in mainstream blockchain systems without significant changes.
These allow \emph{DiPETrans} to be trivially adopted within existing blockchain systems, and gain the benefits of parallel execution without the complexity of additional distributed consensus protocols. 
}


%In this work, the idea of the mining pools is taken up to parallelize the transactions execution, mining, and validation. Essentially, we proposed to use these two concepts, static analysis based \emph{transaction sharding}, and \emph{distributed mining pool} to execute the transactions parallelly along with parallel PoW computation.% First, it groups non-conflicting transactions in different shards by pre-processing (static analysis) of the block transactions. Then different shards are executed parallelly using the concept of distributed mining pools. Second, after the successful execution of all the shards, PoW is determined using the distributed mining pool approach at the miner. Later validator validates the block by re-executing the block transaction parallelly. With this approach, we can achieve higher throughput, lower transactional latency, and resource constraint miners can also participate in the mining to earn rewards. %Conceptually, Byzantine consensus is then individually run on every committee, thus simultaneously processing disjoint sets of transactions (shards). Having said that an equally sized committee could either mean possessing equal hash power, equal stake, or just an equal number of nodes with proven identity. Ideally, the overall approach allows for scaling throughput almost linearly, with an increasing total number of nodes.
%Ideally, the overall approach allows for weak scaling throughput almost linearly with an increasing number of nodes in the community and by varying the ratio of contractual transactions to non-contractual transactions.

%The concept of sharding is used to group the transaction into different shards, where conflicting transactions of different smart contracts in a block grouped into different shards. We execute transactions belong to different shards parallelly with the help of distributed committee (mining pools).  

\end{comment}

==> Arxiv on-13-3-2021/results.tex <==
\section{Experiments and Results}
\label{experiment}

%This section includes the experimental setup, results, and analysis done on the \emph{DiPETrans} framework. The section consists of subsections as experiment setup, experiment configuration, and performance analysis and observations. The first subsection provides a comprehensive overview distributed experiments; the second subsection covers the configurations, and in the end, the last analysis and results subsection presents the speedup achieved by the proposed approach over the serial execution of the transaction.


%This section is organized into subsections. The first subsection provides a general overview of \emph{experimental setup}; the second subsection includes the \emph{experimental configurations}, and the last subsection \emph{performance analysis}, presents the analysis based on execution time and speedup achieved by the proposed approach over the serial.

In this section, we first provide an overview of the \emph{DiPETrans implementation}, followed by a description of the \emph{transactions workload,  experimental setup}, and \emph{performance analysis} based on \emph{execution time} and \emph{speedup} achieved by our proposed approach over a serial version.

%\ysnote{YS to revisit after reading rest of section}


\subsection{Implementation}
%To empirically evaluate the proposed approach and to determine the parallelism we can achieve on Ethereum blockchain, 
We modeled and implemented \emph{DiPETrans} as a stand-alone {permissioned blockchain framework (such as Quorum, i.e., excluding PoW in a permissioned setting) that operates on Ethereum blockchain transactions.} The leader and followers are designed as a set of micro-services that perform mining and validation operations. These include the new operations proposed in \emph{DiPETrans}. Our implementation focuses on operations within the mining community rather than with the rest of the blockchain network. The leader serves as a node with the usual Ethereum functions. The implementation is in \emph{C++} using the Apache thrift cross-platform micro-services library.\footnote[4]{\textbf{Code is available here:} \url{https://github.com/sbshrey/DiPETrans}}%\footnote[5]{\textbf{Technical report is available here:} \url{https://arxiv.org/abs/1906.11721}}
%We modeled and implemented DiPETrans as a stand-alone blockchain framework that operates on Ethereum blockchain transactions. The leader and followers designed as a set of micro-services that perform mining and validation operations. These include the new operations proposed in DiPETrans. The focus of our implementation is on operations within the mining community rather than with the rest of the blockchain network, where the leader just serves as a node with the usual Ethereum functions. The implementation is in \emph{C++} using the Apache thrift cross-platform micro-services library\footnote{Code is available here: \url{https://github.com/sbshrey/DiPETrans}}.

%To empirically evaluate the proposed approach and to determine the parallelism we can achieve on Ethereum blockchain, we implement a stand-alone version of a blockchain framework that models the peers as a set of micro-services that perform the various mining and validation operations that are essential to a blockchain network. This also includes the operations proposed in \emph{DiPETrans}. The implementation is in \emph{C++} using the Apache thrift cross-platform micro-services library.

We made several simplifying assumptions to focus on our goal of concurrent {executions of block transactions (in the permission or permissionless blockchain)}. As mentioned in \textsection\ref{introduction}, all nodes within a community (leader and followers) \emph{trust} each other, e.g., they belong to the same institute or organization or crypto exchange. However, this can be extended in the future to a trustless community using node profiling, which decreases the reputation of malicious nodes~\cite{li2020toward}, detects and removes them. The peers are assumed to be \emph{reliable}. In the future, worker failures can be addressed by distributing the shards of a failed worker to others based on a work-stealing approach. Further, we assumed a \emph{fixed community structure} where the leader knows all the followers when processing a block. The addition and removal of followers or even the leader are not considered here. These issues can partly be addressed using existing techniques~\cite{Luu:SmartPool:usenix2017} for both trusted and trustless communities.

%in our prototype 

%We made several simplifying assumptions to help focus on our goal of concurrent {executions of block transactions (in permissioned or permissionless blockchain)}. All peers in our prototype \emph{trust} each other, e.g., an institute or an organization or a crypto exchange. However, this can be extended in the future to a trustless network using node profiling, which decreases the reputation of malicious nodes~\cite{li2020toward}, and detects and removes such nodes. The peers are assumed to be \emph{reliable}. In the future, worker failures can be addressed by distributing the shards of a failed worker to others based on a work-stealing approach. Further, we assumed a \emph{fixed community structure} where the leader knows all the followers when it starts processing a block. The addition and removal of followers or even the leader are not considered here. These issues can partly be addressed using existing techniques~\cite{Luu:SmartPool:usenix2017} for both trusted and trustless communities. 

%A node wishes to join the community initiates the join method of the \emph{DiPETrans} community contract. Once the respective Tx is accepted, the node is added to the community. Similarly, it can be done to leave the community network. In a trusted community, only the trusted nodes are allowed to join the network (for example, an institute or and organization form a mining community) by the membership provider of the network. However, in a trustless community, anyone can join the network, but a node reputation-based solution must be employed to determine and remove the community's malicious nodes.

% To this point, we implemented a trusted community with no node failure. Trust-less community and workers crash failure implementation is left as a future extension.
%

%Incorporating our proposed approach into an existing blockchain framework like Ethereum is time-consuming 
%\ysnote{any other valid reason? :-)} \spnote{same here} due to the complexity of the codebase of current platforms. Instead, To this point, we implement a stand-alone version of a blockchain framework that models the peers as a set of micro-services that perform the various mining and validation operations that are essential to a blockchain network. This also includes the operations proposed in \emph{DiPETrans}. The implementation is in \emph{C++} using the Apache thrift cross-platform micro-services library. % We conduct experiments to validate the performance of the distributed execution of transactions over serial. 

\subsection{Transactions Workload}
%This section presents the transaction extraction and sampling procedure.

Our experiments used real historical transactions from the Ethereum blockchain available from Google's Bigquery public data archive \cite{BC-Bigquery}. The transactions used start from block number $4,370,000$, which forms a hard fork when Ethereum changed the mining reward from $5$ to $3$ Ethers. We extracted $\approx 80K$ blocks containing $5,170,597$ transactions. While the original transactions had $17$ fields, we selected $6$ fields of interest as part of our workload. These include the \texttt{from\_address} of the sender, the \texttt{{to\_address}} of the receiver, \texttt{{value}} transferred in \emph{Wei}-- the unit of Ethereum currency, \texttt{{input}} data sent along with the transaction, \texttt{{receipt\_contract\_address}} the contract address when it is created for the first time, and \texttt{block\_number} where this transaction was present in.

%Our experiments used real historical transactions from the Ethereum blockchain available from the Google's Bigquery public data archive \cite{BC-Bigquery}. The transactions used start from block number $4,370,000$, which forms a hard fork when Ethereum changed the mining reward from $5$ to $3$ Ethers. We extract $\approx 80K$ blocks containing $5,170,597$ transactions. While the original transactions had $17$ fields, we selected 6 fields of interest as part of our workload. These include the \texttt{from\_address} of the sender, the \texttt{{to\_address}} of the receiver, \texttt{{value}} transferred in \emph{Wei}, the unit of Ethereum currency, \texttt{{input}} data sent along with the transaction, \texttt{{receipt\_contract\_address}} which is the contract address when it is created for the first time, and \texttt{block\_number} where this transaction was present in.

%Our experiments used real historical transactions from the Ethereum blockchain available from the Google's Bigquery public data archive \cite{BC-Bigquery}. The transactions used start from block number $4,370,000$ in the blockchain, which forms a hard fork when Ethereum changed the mining reward from $5$ to $3$ Ethers. We extract $\approx 80K$ blocks containing $5,170,597$ transactions. While the original transactions had $17$ fields, we selected 6 fields of interest as part of our workload. These include the \texttt{from\_address} of the sender, the \texttt{{to\_address}} of the receiver, \texttt{{value}} transferred in \emph{Wei}, the unit of Ethereum currency, \texttt{{input}} data sent along with the transaction, \texttt{{receipt\_contract\_address}} which is the contract address when it is created for the first time, and \texttt{block\_number} where this transaction was present in.


There are two types of transactions we considered: \emph{monetary transactions} and \emph{smart contract transactions}~\cite{Vikram:DBLP:journals/corr/abs}. In the former, also known as value transfer or non-contractual transaction, \emph{coins} are transferred from one account to another account. This is a simple and low-latency operation. In a contractual transaction, one or more smart contract functions are called. We observed that there are $127$ unique Solidity functions in $20K$ contracts, out of which we implemented the top 11 most frequently called ones (\tabref{sc-calls}) that cover $\approx 80\%$ of all contract transactions. 
%We observed that there are $127$ unique Solidity functions in $20K$ contracts, out of which we implemented the top 11 most frequently called ones that cover $\approx 80\%$ of all contract transactions (refer Appendix-Table~II in~\cite{DiPETransArXiv2019}). 
%We have extracted the transactions from a range of the blocks. 
%This section presents all the information related to the experiment setup, such as transaction extraction, sampling, and transaction simulation.
These contract functions implemented in the Solidity language of Ethereum are re-implemented as C++ function calls. These can be invoked by the peers in our framework as part of their transaction execution.


%\subsubsection{Transaction Extraction and Sampling}
%We obtain the data set of the accepted transaction from Ethereum Blockchain public-data set (archive copy) available on Google's Bigquery Engine \cite{BC-Bigquery}. We have chosen the transactions from the intermediate block number \emph{4370000}, which is a hard fork in Ethereum to change the mining reward from 5 Ether to 3 Ether. We extracted $\approx80K$ blocks of data containing $\approx5M$ transactions. 

%\vspace{-.4cm}
\begin{table}[t!]
	\centering
	\caption{Summary of transactions in experiment workload}
	%\vspace{-.2cm}
	\label{tab:txn-sim}
	\resizebox{.8\columnwidth}{!}{%
		\begin{tabular}{c|c|c|r|r|r}
			\hline % (\#Txns/Block)
			{\textbf{Block type}} & $\rho$ & \multicolumn{1}{p{2cm}|}{\textbf{\# Txns/ block}} & {\textbf{\# Blocks}} & \multicolumn{1}{p{2.7cm}|}{\textbf{$\sum$\# Contract txns}} & \multicolumn{1}{p{3.3cm}}{\textbf{$\sum$\# Non-con\-tract txns}}\\
			\hline
			\hline
			data-1-1-100 & \multirow{5}{*}{$\frac{1}{1}$} & $100$ & 3,880 & 193,959 & 194,000 \\
			data-1-1-200 &  & $200$ & 1,940 & 193,959 & 194,000 \\
			data-1-1-300 &  & $300$ & 1,294 & 193,959 & 194,100 \\
			data-1-1-400 &  & $400$ & 970 & 193,959 & 194,000 \\
			data-1-1-500 &  & $500$ & 776 & 193,959 & 194,000 \\
			\hline
			data-1-2-100 & \multirow{5}{*}{$\frac{1}{2}$} &  $100$  &5,705 & 193,959 & 376,530 \\
			data-1-2-200 &  & $200$ &2,895 & 193,959 & 385,035 \\
			data-1-2-300 &  & $300$ &1,940 & 193,959 & 388,000 \\
			data-1-2-400 &  & $400$ &1,448 & 193,959 & 385,168 \\
			data-1-2-500 &  & $500$ &1,162 & 193,959 & 386,946 \\
			\hline
			data-1-4-100 & \multirow{5}{*}{$\frac{1}{4}$} &  $100$  &9,698 & 193,959 & 775,840 \\
			data-1-4-200 &  & $200$ &4,849 & 193,959 & 775,840 \\
			data-1-4-300 &  & $300$ &3,233 & 193,959 & 775,840 \\
			data-1-4-400 &  & $400$ &2,425 & 193,959 & 776,000 \\
			data-1-4-500 &  & $500$ &1,940 & 193,959 & 776,000 \\
			\hline
			data-1-8-100 & \multirow{5}{*}{$\frac{1}{8}$} &  $100$  &16,164 & 193,959 & 1,422,432 \\
			data-1-8-200 &  & $200$ &8,434 & 193,959 & 1,492,818 \\
			data-1-8-300 &  & $300$ &5,705 & 193,959 & 1,517,530 \\
			data-1-8-400 &  & $400$ &4,311 & 193,959 & 1,530,405 \\
			data-1-8-500 &  & $500$ &3,464 & 193,959 & 1,538,016 \\
			\hline
			data-1-16-100 & \multirow{5}{*}{$\frac{1}{16}$} &  $100$  &32,327 & 193,959 & 3,038,738 \\
			data-1-16-200 &  & $200$ &16,164 & 193,959 & 3,038,832 \\
			data-1-16-300 &  & $300$ &10,776 & 193,959 & 3,038,832 \\
			data-1-16-400 &  & $400$ &8,082 & 193,959 & 3,038,832 \\
			data-1-16-500 &  & $500$ &6,466 & 193,959 & 3,039,020 \\
			\hline
		\end{tabular}
	}
	%\end{table}
	
	\vspace{1cm}
	%\begin{table}[t]
	\centering
	\caption{Most frequent functions called by contract transactions}
	%\vspace{-.2cm}
	\label{tab:sc-calls}
	\resizebox{.8\columnwidth}{!}{%
		\begin{tabular}{r|l|c|p{4cm}|r|r}
			\hline
			{\textbf{\#}} &{\textbf{Function}} & {\textbf{Function Hash}} & {\textbf{Parameter Types}} & {\textbf{\# Txns}} &  {\textbf{\%'ile}}\\
			\hline\hline
			1 & transfer & 0xa9059cbb & address, uint256 & 56,654 & 37.72 \\
			2 & approve & 0x095ea7b3 & address, uint256 & 11,799 & 45.58 \\
			3 & vote & 0x0121b93f & uint256 & 11,509 & 53.24 \\
			4 & submitTransaction & 0xc6427474 & address, uint256, bytes & 8,163 & 58.67 \\
			5 & issue & 0x867904b4 & address, uint256 & 5,723 & 62.49 \\
			6 & \_\_callback & 0x38bbfa50 & bytes32, string, bytes & 5,006 & 65.82 \\
			7 & playerRollDice & 0xdc6dd152 & uint256 & 4,997 & 69.15 \\
			8 & multisend & 0xad8733ca & address, address[], uint256[] & 4,822 & 72.36 \\
			9 & SmartAirdrop & 0xa8faf6f0 & - & 4,467 & 75.33 \\
			10 & PublicMine & 0x87ccccb3 & - & 4,157 & 78.10 \\
			11 & setGenesisAddress & 0x0d571742 & address, uint256, bytes & 3,119 & 80.17 \\
			\hline
		\end{tabular}
	}
\end{table}



%\vspace{-.35cm}
%We assume that the contract call by transaction takes more time compared to the monetary transaction. We picked top 11 contract transactions calls as shown in {Table~\ref{tab:sc-calls} (Appendix~\ref{apn:SETD})}, which cover $\approx80\%$ of total contract transactions. The contracts function calls are implemented in \emph{C++} and provide similar functionality based on its Solidity version.% (mentioned in one of the smart contract publicly available).
Of the $\approx5$~Million transactions present in the Ethereum blocks, we considered $193,959$ smart contract transactions. We believe that over time, the wider use of smart contracts will ensure that they form a larger fraction than just monetary transactions. Contract transactions are also more compute-intensive to execute than monetary transactions. They hence can benefit more from our distributed framework. Hence, we created workloads with different ratios between contract and monetary transactions: $\rho \in \big\{\frac{1}{1}; \frac{1}{2}; \frac{1}{4}; \frac{1}{8}; \frac{1}{16}\big\}.$ Each block formed by miners has between 100 to 500 transactions in this ratio, depending on the workload used in an experiment. This workload used in our experiments is described in \tabref{txn-sim}. Here, the block \emph{data-1-2-300} means $\rho = \frac{1}{2}$ is the ratio of contractual to monetary transactions per block while 300 is the total number of transactions in this block.

%Of the $\approx 5$~Million transactions present in the Ethereum blocks, we considered $193,959$ smart contract transactions. We believe that over time, the wider use of smart contracts will ensure that they form a larger fraction than just monetary transactions. Contract transactions are also more compute-intensive to execute than monetary transactions and hence can benefit more from our distributed framework. So, we created workloads with different ratios between contract and monetary transactions: $\rho \in \big\{\frac{1}{1}; \frac{1}{2}; \frac{1}{4}; \frac{1}{8}; \frac{1}{16}\big\}$. Each block formed by miners has between 100 to 500 transactions in this ratio, depending on the workload used in an experiment.\footnote{The workload are described in Table~I and Table~II in the technical report Appendix-V-C~\cite{DiPETransArXiv2019}.}

%Of the $\approx 5$~Million transactions present in the Ethereum blocks we considered, $193,959$ are smart contract transactions. We believe that over time, the wider use of smart contracts will ensure that they form a larger fraction than just monetary transactions. Contract transactions are also more compute-intensive to execute than the monetary transactions, and hence can benefit more from our  distributed framework. Hence, we created workloads with different ratios between contract and monetary transactions: $\rho \in \big\{\frac{1}{1}; \frac{1}{2}; \frac{1}{4}; \frac{1}{8}; \frac{1}{16}\big\}$. Each block formed by miners has between 100 to 500 transactions in this ratio, depending on the workload used in an experiment.\footnote{The workload are described in Table~I and Table~II in the technical report Appendix-V-C~\cite{DiPETransArXiv2019}.} %\ref{tab:txn-sim} 
 %Here, the block \emph{data-1-2-300} means $\rho = \frac{1}{2}$ is the ratio of contractual to monetary transactions per block while 300 is the total number of transactions in this block.


% (see Table~\ref{tab:txn-sim} Appendix~\ref{apn:SETD}). %{Table~\ref{tab:txn-sim} (Appendix~\ref{apn:SETD})} summarizes the blocks and transaction counts where data sets maintains following ratio for contract to non contract (monetary) transactions: 
%{\small $\frac{Contract\ Transactions}{Non\ Contract\ Transactions} = 




%\ysnote{verify this para. I have rephrased it}
%\psnote{done sir.}
We define two transaction workloads with different mixes of these block types. In \textbf{Workload-1}, the number of transactions per block varies from 100 to 500, and within each, we include all available ratios of $\rho$, $\frac{1}{1}$ to $\frac{1}{16}$, i.e., all the blocks in \tabref{sc-calls} are used. In \textbf{Workload-2}, only blocks with 500 transactions are used, and with all available ratios, i.e., \emph{data-1-1-500} to \emph{data-1-16-500}. 

%We define two transaction workloads with different mixes of these block types. In \textbf{Workload-1}, the number of transactions per block varies from 100 to 500, and within each, we include all available ratios of $\rho$, $\frac{1}{1}$ to $\frac{1}{16}$. In \textbf{Workload-2}, only blocks with 500 transactions are used, and with all available ratios.\footnote{{We selected these workloads because the number of transactions per block in Ethereum on and the average is $\approx100$, while the maximum could be more than 200, which may reach a theoretical maximum of $\approx400$~\cite{EthereumGasLimit2020} after a recent increase in the gas limit.}}% i.e., \emph{data-1-1-500} to \emph{data-1-16-500}.


\subsection{Experimental Setup}
We used a commodity cluster to run the leader and followers in the mining and validation communities for our \emph{DiPETrans} blockchain network. Each node in the cluster has an 8-core AMD Opteron 3380 CPU with 32 GB RAM, running CentOS operating system and are connected using 1~Gbps Ethernet. A mining community has a leader running on one node and between one to five followers, each running on a separate node, depending on the experiment configuration. Similarly, a validation community has one leader and between one to five followers. They all run in a single-threaded mode for simplicity, though this can be extended to multi-threading with each thread serving as a follower.
%\ysnote{are you using multi-threading within a node or just using a single thread? If the latter, you can expect it to behave like a single-core server}
%\sbnote{There is no multi threading.}
%\ysnote{Does the leader also act as a follower when executing the mining/validation?}
%\psnote{No sir, leader do not acts as follower.}

% Our goal is to improve throughput for miners and validators by allowing independent transactions to execute parallelly.
%We kept transaction execution to be consistent in both the serial and distributed framework, i.e., serial and distributed execution results in the same state. The experiments are conducted with a fixed topology of 1 miner and 2 validators. The number of follower nodes varies between 1 to 5 for both miner and validators. We tested various configurations for all simulated data sets. 

\subsection{Performance Analysis}
% \ysnote{This section is not clear. I'm not sure what you're running and what you're measuring/reporting}
% \psnote{Sir, there are different experiments:\\ 
% (1) Experiments on ``end to end block creation time'' by the miner includes time taken to execute transactions and time to find PoW.\\
% (2) Experiments on ``transaction execution time'' at miner and validator do not include time to find PoW.}

For each workload, blocks are executed for a serial configuration and for a parallel configuration with 1 to 5 followers. The serial execution serves as the baseline for comparing the performance improvement of the parallel setup. Further, we executed these in different modes. One, the miner only executes the transaction and omits the PoW. Since parallelizing the PoW is trivial and available in the existing literature, this setup highlights the novel value of our static analysis technique for both mining and validation in the permission or permissionless blockchain. Also, we performed experiments with both variants of the validator: default and sharing. Two, the miner performs both transaction execution and PoW computation with concurrency benefits from both. These are described next.

%For each workload, blocks are executed for a serial configuration and for a parallel configuration with 1 to 5 followers. The serial execution serves as the baseline for comparing the performance improvement of the parallel setup. Further, we executed these in different modes. One, the miner only executes the transaction and omits the PoW. Since parallelizing the PoW is trivial and available in the existing literature, this setup highlights the novel value of our static analysis technique for both mining and validation. Also, we performed experiments with both variants of the validator: default and sharing. Two, the miner performs both transaction execution and PoW computation with concurrency benefits from both. These are described next.%\footnote{Additional experiments, are reported in (Appendix~V)\cite{DiPETransArXiv2019}}

%For each workload, blocks are executed for a serial configuration and for a parallel configuration with 1 to 5 followers. The serial execution serves as the baseline for comparing the performance improvement of the parallel setup. Further, we executed these in different modes. One, the miner only executes the transaction and omits the PoW. Since parallelizing the PoW is trivial and available in existing literature, this setup highlights the novel value of our static analysis technique for both mining and validation. Also, we performed experiments with both variants of the validator: default and sharing. Two, the miner performs both transaction execution and PoW computation with concurrency benefits from both. These are described next. Additional experiments are reported in Appendix~\ref{ap:bes}.

%Block execution time is split to identify the time taken by transaction execution and for end-to-end execution, per block. 
%\psnote{%We omit PoW time; in another, we include it.
%Experiments that include PoW time are exclusively for miners; we call this end-to-end block creation time by the miner. Experiments that consider transaction execution time and omit PoW time are for both miners and validators.}

%Block execution using mining communities gives the end-to-end block creation time by the leader and followers, while without using mining communities reports the transaction execution time just at the leader. \ysnote{I'm confused. Are you omitting PoW time for the miner?} However, transaction execution time at validator includes the time taken by transaction re-execution and verification. For \dVal{} time taken by static analysis also included as part of the time taken by the validator. \ysnote{use std terms introduced earlier, such as executing txn, finding PoW, verifying PoW. What do you mean by executing a miner without mining?!!}
%\sbnote{end-to-end block execution includes the time taken to find PoW along with transactions execution and verification.}

% \begin{comment}
% Lastly, in \textbf{Workload-3}, transactions is fixed to 500 per block, and community size varies from 1 to 5. For all this analysis, we computed execution time and speedup (with and without mining). The analysis for \emph{Workload-3}  and tables for execution time and speedup is given in \emph{Appendix~\ref{ap:bes}}.% Please refer to the \emph{tech-report}\footnote{https://arxiv.org/xxxx.yyyy} for detailed analysis of the experiments.
% \end{comment}

\input{finalResults}

%\subsubsection{Block Execution Time without Mining}
\subsubsection{Transaction Execution Time} %  Omitting Time to Find PoW
%\sbnote{we will replace ``without mining'' with ``without finding PoW''}
This section presents the results and analysis for executing transactions at the miner and verifying them at the validator. It omits the time to find the PoW at the miner and verifying it at the validator. The serial execution serves as a baseline. 

%\ysnote{is this avg time per block? Averaged across all the blocks in the workload?}
%\psnote{It is averaged across the blocks, e.g., averaged for all the blocks with 100 transactions across the $\rho$ in Figures~\ref{fig:W1:avg-txn} first point on the x-axis.}


Figures~\ref{fig:W1:avg-txn} and~\ref{fig:W2:avg-txn} show the \emph{average execution time per block (in ms)} for Workload~1 and Workload~2, respectively, for the different modes of execution. For Workload~1, the number of transactions per block increases in the X-axis, while for Workload~2, the contract to monetary transaction ratio $\rho$ varies. Subfigure (a) is for the miner, and Subfigures (b) and (c) are for the default and sharing validators. 
%Figures~\ref{fig:W1:avg-txn} and~\ref{fig:W2:avg-txn} show the \emph{average execution time per block (in ms)} for Workload~1 and Workload~2, respectively, for the different modes of execution. For Workload~1, the number of transactions per block increases in the X-axis, while for Workload~2, the contract to monetary transaction ratio $\rho$ varies. Subfigure (a) in these figures are for the miner, and Subfigures (b) and (c) are for the default and sharing validators.%, and Subfigure (d) is... 
% \ysnote{Whats diff between b/c and d? How many followers are in d? Is it avg across 1-5 followers? Do you really need it?}
% \psnote{Fig d is for a clear comparison between \sVal{} and \dVal{}. Yes, it is avg across 1-5 followers. We can remove it if it is not required; maybe we can move fig d plots in the appendix sec.}
% \ysnote{Yes, I would suggest we move out subfig (d) to appendix. The Figs (b) and (c) are clear enough.}
% \psnote{Removed Fig (d) will add it in the appendix of the tech report.}
The corresponding Figures~\ref{fig:W1:avg-speed-up} and~\ref{fig:W2:avg-speed-up} show the speedup of our parallel execution, relative to the serial execution.\footnote[6]{The additional experiments and raw values for these plots are reported in the Appendix.}%\cite{DiPETransArXiv2019}.}


% The figure \emph{\textbf{a}} shows the line plots for mean transaction execution time taken by the miner. Figure \emph{\textbf{b}} shows the transactions execution time taken by \dVal{} while figure \emph{\textbf{c}} shows transactions execution time taken by \sVal{}. The figure \emph{\textbf{d}} shows comparison for average transactions execution time taken by \dVal{} and \sVal{}.
% \ysnote{dont call it "subfigure a". Refer to use using \figref{W1:avg-txn}a}
% \psnote{done sir.}
\vspace{.2cm}
\noindent
\textbf{Workload-1.~}
%\paragraph{Workload-1.~}
%{\figref{W1:avg-txn}} shows the average transactions execution time taken by the miner and validator ({Table~\ref{tab:W1:TxExe}} Appendix~\ref{ap:bes}) . 
As shown in the \figref{W1:avg-txn}, the average execution time per block increases as the number of transactions in a block increases from 100 to 500. Each block size in this workload includes all values of $\rho$, the ratio. 
%As shown in the \figref{W1:avg-txn} the average execution time per block increases as the number of transactions in a block increases from 100 to 500. Within each block size, blocks in this workload include all values of $\rho$.
%\ysnote{What is the ratio for Workload~1? All different ratios or a fixed value of $\rho$?}
%\psnote{Its averaged across the $\rho$.}
This growth is linear, except for the serial execution that shows an increase in the slope beyond 300 transactions per block. %\ysnote{Why?}
%\sbnote{A possible reason for the increase in the slope of serial execution may be due to the increase in contractual transactions. A similar effect is not reflected in the distributed case due to parallelism.}
%\ysnote{but the growth should be linear since the blocks have a similar mix of ratios. I am guessing we're hitting some physical limit on the servers beyond that. Need to dig into it later.}
We also see that the 1 follower configuration is performing worse than the serial execution due to the overhead of static analysis at the leader and communication between the leader and follower. However, other configurations with 2 to 5 followers offer faster execution times than serial execution.

%\ysnote{YS to revisit this para once details of fig (d) are clear}
\figref{W1:avg-txn}(b) and~\ref{fig:W1:avg-txn}(c) shows the line plots for the average transactions execution time per block, taken by \dVal{} and \sVal{}, respectively. The only difference between these two validators is that \dVal{} runs static analysis on the block transactions before execution, while \sVal{} reuses the dependency graph encoded in the block. The results for both these validators are near-identical and also closely match the results for the miner. The former indicates that the transaction validation time dominates, and the overheads for static analysis are negligible. Further, since the miner in this experiment only executes transactions and not the PoW, it is understandable that the validators that use a similar transaction execution phase exhibit similar results.% The \dVal{} is expected to take more time compared to \sVal{}. However, the experiment shows no significant difference (can be observed in {Table~\ref{tab:W1:TxExe}}) as the static analysis is taking very less time.


When we examine the parallel speedup for this workload relative to the serial execution in the \figref{W1:avg-speed-up}, we observed that the speedup increases with an increasing number of followers. As seen before, with 1 follower, the speedup is below $1 \times$ while with 5 followers, the peak speedup achieved is $2.18 \times$. The speedup also improves as the number of transactions per block increases. This causes shards with a larger number of transactions to be created, and parallelization of the higher computational load amortizes the static analysis and the communication overheads. However, the speedup efficiency is sub-optimal at about 51\% for 4 followers and 44\% for 5 followers, with 500 transactions/blocks.
%The speedup increases linearly as the number of increasing from 2 to 5 followers (see \figref{W3:avg-speed-up} of Appendix~\ref{subsec:sa}), so it is expected to increase with an increase in community size or the number of transactions per block. However, 1 follower community is not achieving any speedup over serial due to static analysis and communication costs.
%
A similar trend is observed for the validators. We also noticed that the speedup curves for \sVal{} and \dVal{} are comparable. This means that the benefits of a sharing validator are negligible due to the minimal time taken by the static analysis. Further, we observed that static analysis is not a bottleneck for the leader in this workload due to just hundreds of transactions per block. So the \dVal{} will suffice, and it also avoids encoding the transaction dependency graph into the block required by the \sVal{}{}. The validators' average speedup is $1.25\times$, and their peak is $2.03\times$ with 5 followers and 500 transactions per block.
%A similar trend is observed for the validators. We also noticed that the speedup curves for \sVal{} and \dVal{} are comparable. This means that the benefits of a sharing validator are negligible due to the minimal time taken by the static analysis. So the \dVal{} will suffice, and it also avoids encoding the transaction dependency graph into the block required by the \sVal{}. The average speedup for the validators is $1.25\times$, and their peak is $2.03\times$ with 5 followers and 500 transactions per block.

% Further, \sVal{} was assumed to outperform \dVal{}. However, performance is almost the same, which means static analysis is not taking much time. We have achieved on an average $1.33\times$, $1.255\times$, and $1.259\times$ speedup respectively for parallel miner, \dVal{} and \sVal{}. Achieved max speedup of $2.18\times$ for miner, $2.02\times$ for \dVal{} and $2.04\times$ for \sVal{} for 100 to 500 transactions per block. Experiments show that parallel execution gives better speedup and can be used to form a community to receive the incentive by mining the block in the blockchain.


\vspace{.2cm}
\noindent
\textbf{Workload-2}~In this workload, the transactions per block are fixed at 500 while we vary the ratio $\rho$. {\figref{W2:avg-txn}} shows the average transaction execution time taken by the miner and the two types of validators in the Y-axis as the value of $\rho$ increases along the X-axis. We observed that reducing the ratio of contract transactions relative to the non-contractual transactions reduces the average time taken to mine or validate a block. This can be explained by the higher computational complexity of the smart contracts that execute non-trivial external function calls as part of the transaction logic.
%\textbf{Workload-2}~In this workload, the transactions per block are fixed at 500 while we vary the ratio $\rho$. {\figref{W2:avg-txn}} shows the average transaction execution time taken by the miner and the two types of validators in the Y-axis as the value of $\rho$ increases along the X-axis. We observed that reducing the ratio of contract transactions relative to the non-contractual transactions reduces the average time taken to mine or validate a block. This can be explained by the higher computational complexity taken the smart contracts that execute non-trivial external function calls as part of the transaction logic. 

%\paragraph{Workload-2}~In this workload, the transactions per block are fixed at 500 while we vary the ratio $\rho$. {\figref{W2:avg-txn}} shows the average transaction execution time taken by the miner and the two types of validators in the Y-axis as the value of $\rho$ increases along the X-axis. We observed that reducing the ratio of contract transactions relative to the non-contractual transactions reduces the average time taken to mine or validate a block. This can be explained by the higher computational complexity taken the smart contracts that execute non-trivial external function calls as part of the transaction logic. 

Unlike Workload~1, the 1 follower scenario is comparable to the serial setup rather than slower. Having more than 1 follower offers consistently better performance than serial. However, with the increase of non-contractual transactions in a block, the serial execution starts even to match the time taken by more followers. Here, given the short absolute execution time of about $400~ms$ per block for $\rho=\frac{1}{16}$ due to the simple non-contractual transactions, it is possible that the round trip communication time between the leader and the follower may start to have a tangible impact. In {\figref{W2:avg-txn}(c)}, we can observe that the time required to execute more transactions per block decreases as the number of contract transactions decreases. These trends are common to the miners and the two validators.
%Unlike Workload~1, the 1 follower scenario is comparable to the serial setup rather than slower. Having more than 1 follower offers consistently better performance than serial. But with the increase of non-contractual transactions in a block, the serial execution starts even to match the time taken by more followers. Here, given the small absolute execution time of about $400~ms$ per block for $\rho=\frac{1}{16}$ due to the simple non-contractual transactions, it is possible that the round trip communication time between the leader and the follower may start to have a tangible impact. In {\figref{W2:avg-txn}c}, we can observe that the time required to execute more transactions per block decreases as the number of contract transactions decreases. These trends are common to the miners and the two validators.

%{\figref{W2:avg-txn}d} shows that the parallel validator is always taking less time than serial, and a significant gap can be observed when the number of non-contractual transactions per block increases. However, the \dVal{} is expected to take more time compared to \sVal{}. However, the experiment shows that the analysis function is not taking much time, so there is no significant difference between them.

%\ysnote{can we comment on the number of components per block thru static analysis for different rho? And the distribution of the component sizes? These can affect the load balancing.}
%\sbnote{We do not have the relevant numbers for this analysis and it will take time to collect them. Also the data which we had simulated while running this algorithms has been deleted from the scratch of Rigel server. }
Interestingly, in \figref{W2:avg-speed-up}, the speedup curve shows improvement as the value of $\rho$ increases until $\frac{1}{4}$ and drops after that. This indicates that the sweet-spot of parallel efficiency lies with this mix of the contract and non-contract transactions, offering a peak speedup of $2.7\times$ with 5 followers and a favorable speedup efficiency of 73\% with 3 followers.

%\vspace{.08cm}
%\noindent
% \textbf{Speedup Analysis: }The speedup for \emph{Workload-1, Workload-2,} and \emph{Workload-3} is given in the {\figref{W1:avg-speed-up}} ({Table~\ref{tab:W1:Speedup}}), {\figref{W2:avg-speed-up}}, and {\figref{W3:avg-speed-up}} ({Table~\ref{tab:W2-W3:Speedup}}) respectively. In all the experiments, serial execution is considered to be a baseline, and parallel execution speedup is shown as a line chart. We achieved $\approx2\times$ speedup, using just 5 followers in the community. The speedup is linearly increasing from 2 to 5 followers (see \figref{W3:avg-speed-up} of Appendix~\ref{subsec:sa}), so it is expected to increase with an increase in community size or the number of transactions per block. However, 1 follower community is not achieving any speedup over serial due to static analysis and communication costs.


% Further, \sVal{} was assumed to outperform \dVal{}. However, performance is almost the same, which means static analysis is not taking much time. We have achieved on an average $1.33\times$, $1.255\times$, and $1.259\times$ speedup respectively for parallel miner, \dVal{} and \sVal{}. Achieved max speedup of $2.18\times$ for miner, $2.02\times$ for \dVal{} and $2.04\times$ for \sVal{} for 100 to 500 transactions per block. Experiments show that parallel execution gives better speedup and can be used to form a community to receive the incentive by mining the block in the blockchain.
%Further, \sVal{} was assumed to outperform \dVal{}, but their performance is almost the same, which means static analysis is not taking much time. We have achieved on an average $1.33\times$, $1.255\times$, and $1.259\times$ speedup respectively for parallel miner, \dVal{} and \sVal{}. Achieved max speedup of $2.18\times$ for miner, $2.02\times$ for \dVal{} and $2.04\times$ for \sVal{} for 100 to 500 transactions per block. Experiments show that parallel execution gives better speedup and can be used by the trusted node to form a community to receive the incentive by mining the block in the blockchain.



%\ysnote{YS to resume from here}
%\subsubsection{End-to-end Block Execution Time Including Time to Find PoW at Miner}
\subsubsection{End-to-end Mining Time}%Block Creation Time at Miner
Here we present the analysis for end-to-end block creation time by the miner, which includes the transaction execution time as well as the time to find the PoW. 

%We have observed that the increase in the number of transactions per block, end-to-end time increases for fining the PoW. This is because the difficulty is fixed for all the experiments at the start of the experiments. Finding PoW is a random process, so we cannot guarantee the maximum time to find PoW.

%\ysnote{move this to appendix. Its more of a background and such level of detail is not relevant}
%\psnote{done sir. moved to Appendix \ref{ap:back}}
{

\begin{figure}[!h]
%	\begin{minipage}{.48\textwidth}
	    \centering
	    {\includegraphics[width=.67\textwidth]{figs/FinalResults/WithMining/EtETimeW1-W2.pdf}}\vspace{-.15cm}
	    \caption{Average end-to-end block creation time, including the time to find PoW by community miner.}
	    \label{fig:EtETime}
%	\end{minipage}
\vspace{.35cm}
%	\begin{minipage}{.48\textwidth}
	    \centering
	     {\includegraphics[width=.65\textwidth]{figs/FinalResults/WithMining/EtESpeedupW1-W2.pdf}}\vspace{-.15cm}
	    \caption{Average end-to-end block creation speedup by community miner over serial miner.}
	    \label{fig:EtESpeedup}
 %   \end{minipage}
%\vspace{-.55cm}
\end{figure}

Existing blockchain platforms calibrate the difficulty to keep the mean end-to-end block creation time within limits like in Bitcoin; the block is created every 10 minutes and every two weeks 2016 blocks. After every 2016 blocks, the difficulty is calibrated based on how much time is taken if it has taken more than two weeks, the difficulty is reduced otherwise increased also several other factors are also considered to change the difficulty. While in Ethereum blockchain, roughly every 10 to 19 seconds, a block is produced, so the difficulty is fixed accordingly. After every block creation, if mining time goes below 9 seconds, then \emph{Geth}, a multipurpose command line tool that runs Ethereum full node, tries to increase the difficulty. In case when the block creation difference is more than 20, Geth tries to reduce the mining difficulty of the system. Solving PoW is an inherent brute-force task. Blockchain platforms calibrate the difficulty of solving it to ensure that the average block creation time remains within limits as hardware technology improves and the mix of transactions varies. In fact, Ethereum changes the difficulty level for a block based on the time taken to create the previous block, to have it lie between {9--20~secs}. For simplicity, in our experiments, we fixed the difficulty per block to be a static value. %In the proposed \emph{DiPETrans} framework throughout the experiments, 
We fixed the difficulty, and due to that reason with an increase in transaction per block increase in mining time can be observed. %\ysnote{what is this fixed based on? The difficulty as it existed at the time the blocks in our datasets were created?}
}

\figref{EtETime} shows the average execution time for each block on the Y-axis, which includes the transaction execution time and PoW time, as the number of transactions per block increases (Workload~1) or the value of $\rho$ varies (Workload~2). In contrast to the earlier experiments, we can clearly see that the execution time has increased by orders of magnitude by introducing the PoW, ranging between {10--60~secs} per block for the serial execution. We also see an apparent linear growth in time as the transactions per block increases in Workload~1. When seen along with the speedup plots in \figref{EtESpeedup}(a), we observe a substantial improvement in the average block creation time as the number of followers increase. We have a speedup of $1.15\times$ to $4.91\times$ for 1--5 followers that remain stable as the block size increases, with a speedup efficiency of 57.5 to 81.83\%. \figref{EtETime}(b) for Workload~2, where the monetary transactions increases per block, the mining time sometimes increases and sometimes decreases. The possible reason can be that we are not changing the difficulty while varying the transaction ratio.
%\ysnote{is the PoW compute cost supposed to be proportional to the number of transactions in a block? Or is it also dependent on the type of transaction (contract/monetary)?}
%\sbnote{The difficulty is indirectly dependent upon the number of transactions as it takes the block creation time into consideration for the parent block  {\color{blue}\url{https://dltlabs.com/how-difficulty-adjustment-algorithm-works-in-ethereum/}}. The above algorithm gets activated only if its going to slow or too fast meaning above 20 sec or below 10 sec. For simplicity, in our experiments, we fix the difficulty per block to be a static value.}
%and \figref{EtESpeedup}, when the number of followers increases in the community, end-to-end block creation time decreases. On \emph{Workload-1}, when transaction increases per block time taken by the mining also increases, as shown in \figref{EtETime}a. 


%\figref{EtETime}(b) for Workload~2, where the monetary transactions increases per block, the mining time sometimes increases and sometimes decreases. The possible reason can be that we are not changing the difficulty while varying the transaction ratio. %In \figref{EtESpeedup}a and \figref{EtESpeedup}b, with the varying number of transactions and transaction ratio, the speedup is almost similar, but with an increase in community members speedup is higher over the smaller community as well over serial. We achieved a maximum of $5 \times$ end-to-end block creation with mining speedup by parallel miner over serial miner when using just 6 workers (including leader) in the community. We observed that end-to-end block creation speedup linear increases with the number of followers in the community.

%Due to page limitation, remaining results are presented in technical report~\cite{DiPETransArXiv2019} as follows: Remaining results for transaction execution time and speedup in {Appendix~V-C}, Block execution time (end-to-end time) at miner in {Appendix~V-D}. For a varying number of transaction from 500 to 2500 in {Appendix~V-E}. 


{
	

%\input{shards-results}
\begin{figure}[!h]
	\begin{subfigure}{.45\textwidth}
		\centering
		{\includegraphics[width=.9\textwidth]{figs/FinalResults/Shards/all_num_shards_W1.pdf}}%\vspace{-.01cm}
		\vspace{-.15cm}\\\hspace{1cm}(a) Workload 1 (W1)
		%\caption{Workload 1 (W1)}
		%\label{fig:sfig1}
	\end{subfigure}%
	\hfill
	\begin{subfigure}{.45\textwidth}
		\centering
		{\footnotesize \color{gray} \hspace{1cm} Fixed 500 Transactions/Block}
		{\includegraphics[width=.9\textwidth]{figs/FinalResults/Shards/all_num_shards_W2.pdf}}%\vspace{-.01cm}
		\vspace{-.15cm}\\\hspace{1cm}(b) Workload 2 (W2)
		%\caption{Workload 2 (W2)}
		%\label{fig:sfig2}
	\end{subfigure}
	\vspace{-.18cm}
	\caption{Number of shards with varying transactions per block and varying data set ($\rho$).}
	\label{fig:ShardsPerBlock}
	%\end{figure}
	\vspace{.4cm}
	%\begin{figure}[!htb]
	\begin{subfigure}{.45\textwidth}
		\centering
		{\includegraphics[width=.9\textwidth]{figs/FinalResults/Shards/all_max_trans_shard__W1.pdf}}%\vspace{-.01cm}
		\vspace{-.15cm}\\\hspace{1cm}(a) Workload 1 (W1)
		%\caption{Workload 1 (W1)}
		%\label{fig:sfig1}
	\end{subfigure}%
	\hfill
	\begin{subfigure}{.45\textwidth}
		\centering
		{\footnotesize \color{gray} \hspace{1cm} Fixed 500 Transactions/Block}
		{\includegraphics[width=.9\textwidth]{figs/FinalResults/Shards/all_max_trans_shard__W2.pdf}}%\vspace{-.01cm}
		\vspace{-.15cm}\\\hspace{1cm}(b) Workload 2 (W2)
		%\caption{Workload 2 (W2)}
		%\label{fig:sfig2}
	\end{subfigure}
	\vspace{-.18cm}
	\caption{Number of transactions in a shard with varying transactions per block and varying data set ($\rho$).}
	\label{fig:transPerShard}
	%\end{figure}
	\vspace{.4cm}
	%\begin{figure}[!htb]
	\begin{subfigure}{.45\textwidth}
		\centering
		{\includegraphics[width=.9\textwidth]{figs/FinalResults/Shards/all_avg_txns_f1__W1.pdf}}%\vspace{-.01cm}
		\vspace{-.15cm}\\\hspace{1cm}(a) Workload 1 (W1)
		%\caption{Workload 1 (W1)}
		%\label{fig:sfig1}
	\end{subfigure}%
	\hfill
	\begin{subfigure}{.45\textwidth}
		\centering
		{\footnotesize \color{gray} \hspace{1cm} Fixed 500 Transactions/Block}
		{\includegraphics[width=.9\textwidth]{figs/FinalResults/Shards/all_avg_txns_f1__W2.pdf}}%\vspace{-.01cm}
		\vspace{-.15cm}\\\hspace{1cm}(b) Workload 2 (W2)
		%\caption{Workload 2 (W2)}
		%\label{fig:sfig2}
	\end{subfigure}
	\vspace{-.18cm}
	\caption{Number of transactions allocated to a follower with varying transactions per block and varying data set ($\rho$).}
	\label{fig:transPerFollower}
\end{figure}


	
	
\subsubsection{Sharding Analysis}
\label{sec:Sanalysis}
%Here we present the analysis for the number of shards per block and the number of transactions in a shard. 
Here in this section, we present the analysis for the number of shards per block, transactions in a shard, and the transactions allocated to a follower on both the workloads. In Workload~1, the number of transactions per block varies, while in Workload~2 ratio ($\rho$) of non-smart contract (monetary) transactions to smart contract transactions vary where transaction counts per block remained 500 for all the cases. These experiments considered the community with fixed five followers.




To determine available parallelism within a block, \figref{ShardsPerBlock} shows the number of shards per block on both workloads. \figref{ShardsPerBlock}(a) shows the number of shards on Workload~1, \figref{ShardsPerBlock}(b) on Workload~2 with varying ratio $\rho$, and \figref{transPerFollower} shows the number of transactions allocated to a follower. The larger the number of shards in a block, the higher the possibility of parallelism. The number of shards per block increases with the increasing number of transactions in a block on Workload~1. Nevertheless, on Workload~2, it remains approx the same due to the fixed number of transactions. However, the average number of shards is adequate to achieve parallelism within the community.


When the number of shards is higher than the community size, we reasonably load balance between the community followers. Remarkably the minimum number of shards (skewed cases where most of the transactions in a block belong to just a few shards) is significantly less, where parallelism is very low. The maximum shards on both the workloads are $\approx 370$. While the average number of shards in Workload~1 increases from $\approx 40$ to $\approx 131$ when transactions change from $100$ to $500$ per block, respectively. Based on these observations, we can conclude that enough parallelism is available within the block to improve the throughput. 



\figref{transPerShard} shows the number of transactions in the largest shard with varying number of transactions per block (\figref{transPerShard}(a)) and varying $\rho$ (\figref{transPerShard}(b)) to demonstrate the skewness present within a shard and blocks. The larger the number of transactions in the largest shard (skewed), the lower the block parallelism. We can observe in \figref{transPerShard} that the number of transactions increases in maximum shard in both workloads. The increase in transactions with varying $\rho$ on Workload~2 is relatively significant compare to Workload~1. It indicates that the correlations between transactions often escalate when monetary transaction increases in the block. As shown in \figref{transPerFollower}, after the load balancing, the average number of transactions allocated to a follower is balanced. Hence all the followers get approximately even load (we have five followers in the community).

We observed that the maximum number of shards is $\approx 370$ in a block with 500 transactions in Workload~1. On average, a shard with a maximum number of transactions is $\approx 460$ in 500 transactions block when $\rho$ is $\frac{1}{16}$. The number of shards and number of transactions (in the maximum size shard) increases with an increase in the number of transactions per block (Workload~1) and ratio $\rho$ (Workload~2), respectively.


\subsubsection{Performance Overhead Analysis}
%\subsubsection{RAM Utilization and Static Analysis Time}
\label{sec:other}
The analysis of the average RAM size taken by the followers during the execution of the transaction and the time taken by the leader for sharding block transactions (i.e., time taken by \texttt{Analyze()}(\algoref{analyze})) is discussed here in this section. 

\begin{comment}
\begin{figure}[h]
%\vspace{-.4cm}
\begin{minipage}{.48\textwidth}
\centering
{\includegraphics[width=1\textwidth]{figs/FinalResults/RAM/w1-w2-Ram-Size.pdf}}\vspace{-.15cm}
\caption{RAM utilized by followers during execution with varying transactions per block and varying data set ($\rho$).}
\label{fig:RAMSize}
%\vspace{.35cm}
\end{minipage}
\qquad
\begin{minipage}{.48\textwidth}
\centering
{\includegraphics[width=1\textwidth]{figs/FinalResults/Analyze/w1-w2-num-Analyze.pdf}}\vspace{-.15cm}
\caption{Time taken by \texttt{Analyze()}algorithm with varying transactions per block and varying data set ($\rho$).}
\label{fig:AnalyzeTime}
%\vspace{-.55cm}
\end{minipage}
\end{figure}
[t]\end{comment}



The maximum RAM used by followers increases with an increasing number of transactions in the block, which can be seen in \figref{RAMSize}(a), as expected, because additional transactions in the block may take extra space to store data as well more space during execution. However, the average RAM size remains steady. As shown in \figref{RAMSize}(b), with increasing ratio $\rho$, the average RAM size decreases; this may be because non-smart contract (monetary) transactions are less expensive in computation and latency than smart contract function calls, hence take lesser space. In contrast, the maximum RAM size in Workload~2 reaches $\approx 10,000$~Kb that is relatively closer to maximum RAM size in Workload~1.


\begin{figure}[!h]
	\begin{subfigure}{.45\textwidth}
		\centering
		{\includegraphics[width=.9\textwidth]{figs/FinalResults/RAM/all_ram__W1.pdf}}%\vspace{-.01cm}
		\vspace{-.15cm}\\\hspace{1.3cm}(a) Workload 1 (W1)
		%\caption{Workload 1 (W1)}
		%\label{fig:sfig11}
	\end{subfigure}%
	\hfill
	\begin{subfigure}{.45\textwidth}
		\centering
		{\footnotesize \color{gray} \hspace{1cm} Fixed 500 Transactions/Block}
		{\includegraphics[width=.9\textwidth]{figs/FinalResults/RAM/all_ram__W2.pdf}}%\vspace{-.01cm}
		\vspace{-.15cm}\\\hspace{1.2cm}(b) Workload 2 (W2)
		%\caption{Workload 2 (W2)}
		%\label{fig:sfig21}
	\end{subfigure}
	\vspace{-.18cm}
	\caption{RAM utilized by followers during execution with varying transactions per block and varying data set ($\rho$).}
	\label{fig:RAMSize}
	%\end{figure}
	\vspace{.35cm}
	%\begin{figure}[!b]
	\begin{subfigure}{.45\textwidth}
		\centering
		{\includegraphics[width=.9\textwidth]{figs/FinalResults/Analyze/all_analyze__W1.pdf}}%\vspace{-.01cm}
		\vspace{-.15cm}\\\hspace{1.3cm}(a) Workload~1 (W1)
		%\caption{Workload 1 (W1)}
		%\label{fig:sfigA11}
	\end{subfigure}%
	\hfill
	\begin{subfigure}{.45\textwidth}
		\centering
		{\footnotesize \color{gray} \hspace{1cm} Fixed 500 Transactions/Block}
		{\includegraphics[width=.9\textwidth]{figs/FinalResults/Analyze/all_analyze__W2.pdf}}%\vspace{-.01cm}
		\vspace{-.15cm}\\\hspace{1.2cm}(b) Workload~2 (W2)
		%\caption{Workload 2 (W2)}
		%\label{fig:sfigA21}
	\end{subfigure}
	\vspace{-.15cm}
	\caption{Time taken by \texttt{Analyze()}algorithm with varying transactions per block and varying data set ($\rho$).}
	\label{fig:AnalyzeTime}
\end{figure}



The time taken by \texttt{Analyze()}algorithm can be seen in \figref{AnalyzeTime}. It is utilized to find shards using static analysis as a graph problem. The algorithm is explained in \textsection \ref{shardingBlock}. We use microseconds ($\mu s$) here in \figref{AnalyzeTime} for visualization purposes since the analysis algorithm takes significantly less time than the execution time of the transactions. As shown in \figref{AnalyzeTime}(a), analysis time increases with increasing transactions in the block since the time taken by graph construction and WCC composition to find different shards increases with the number of transactions. However, the number of transactions in Workload~2 with varying ratio $\rho$ is fixed to 500 per block; consequently, the average time taken by the static analysis is almost comparable as shown in \figref{AnalyzeTime}(b).

\begin{figure}[!t]
	\centering
	{\includegraphics[width=1\textwidth]{figs/FinalResults/Throughput/w1-w2-Throughput.pdf}}\vspace{-.15cm}
	\caption{Throughput with varying transactions per block and varying data set ($\rho$).}
	\label{fig:Throughput}
\end{figure}
\subsubsection{Throughput Analysis}
%The analysis in parallel transactions in community set-up and serial set-up for the proposed \emph{DiPETrans} blockchain is presented here.
The throughput analysis of the proposed \emph{DiPETrans} blockchain on community configuration for parallel transaction execution and serial execution is discussed here. 


The \figref{Throughput} shows the throughput trend on the Workload~1 and Workload~2. Throughput increases with the increasing number of transactions per block. It increases with the increase in the non-smart contract (monetary) transactions per block on Workload~2. The gain in throughput on Workload~2 is relatively more significant than that of on Workload~1. This accumulation implies that non-smart contract (monetary) transactions are less expensive in computation and latency than smart contract function calls; therefore, more transactions can be executed per second.


Further, as shown in \figref{Throughput}(a), the throughput for serial execution increases with the increasing number of transactions to 300 transactions per block and reaches a maximum of 900 tps (transactions per second); after that, there is a drop-down in throughput. However, this is not the case with community-based parallel execution in the proposed approach; it keeps increasing with the increasing number of transactions per block and followers in the community, which confirms that \emph{DiPETrans} improves the throughput. The maximum throughput on Workload~1 is 1577 tps in a community with five followers at 500 transactions per block, which is $2.05 \times$ higher than that of serial execution. Nevertheless, this difference narrows down to $1.49\times$ on Workload~2 as shown in \figref{Throughput}(b), where parallel execution achieves a maximum throughput of 2147 tps when ratio $\rho = \frac{1}{16}$. However, the sweet spot of maximum throughput by parallel approach concerning serial is at $2.52 \times$ with 1690 tps on Workload~2 when $\rho = \frac{1}{4}$. This implies that the proposed approach yields maximum benefit when a block consisting of a small number of monetary transactions. Since contractual transactions are computation-intensive and executing independent contractual transactions in parallel will increases the throughput.


In addition to these experiments, we have done few additional experiments. The additional results are presented as follows in the appendix:} Remaining results for transaction execution time and speedup in {Appendix~\ref{ap:bes}}. Block execution time (end-to-end time) at miner in {Appendix~\ref{apn:betete}}. For varying number of transaction from 500 to 2500 in {Appendix~\ref{ap:txv2500}}.

%Due to page limitation remaining results are presented in appendix as follows: Remaining results for transaction execution time and speedup in {Appendix~\ref{ap:bes}}. Block execution time (end-to-end time) at miner in {Appendix~\ref{apn:betete}}. For varying number of transaction from 500 to 2500 in {Appendix~\ref{ap:txv2500}}. 



==> Arxiv on-13-3-2021/shards-results.tex <==
\begin{figure}[h]
	\begin{subfigure}{.47\textwidth}
		\centering
		{\includegraphics[width=.9\textwidth]{figs/FinalResults/Shards/all_num_shards_W1.pdf}}\vspace{-.01cm}
		(a) Workload 1 (W1)
		%\caption{Workload 1 (W1)}
		%\label{fig:sfig1}
	\end{subfigure}%
	\qquad
	\begin{subfigure}{.47\textwidth}
		\centering
		{\includegraphics[width=.9\textwidth]{figs/FinalResults/Shards/all_num_shards_W2.pdf}}\vspace{-.01cm}
		(b) Workload 2 (W2)
		%\caption{Workload 2 (W2)}
		%\label{fig:sfig2}
	\end{subfigure}
	\vspace{-.21cm}
	\caption{Number of shards with varying transactions per block and varying data set ($\rho$).}
	\label{fig:ShardsPerBlock}
%\end{figure}
%\begin{figure}[h]
\vspace{.25cm}
	\begin{subfigure}{.47\textwidth}
		\centering
		{\includegraphics[width=.9\textwidth]{figs/FinalResults/Shards/all_max_trans_shard__W1.pdf}}\vspace{-.01cm}
		(a) Workload 1 (W1)
		%\caption{Workload 1 (W1)}
		%\label{fig:sfig1}
	\end{subfigure}%
	\qquad
	\begin{subfigure}{.47\textwidth}
		\centering
		{\includegraphics[width=.9\textwidth]{figs/FinalResults/Shards/all_max_trans_shard__W2.pdf}}\vspace{-.01cm}
		(b) Workload 2 (W2)
		%\caption{Workload 2 (W2)}
		%\label{fig:sfig2}
	\end{subfigure}
	\vspace{-.21cm}
	\caption{Number of transactions in a shard with varying transactions per block and varying data set ($\rho$).}
	\label{fig:transPerShard}
%\end{figure}
%\begin{figure}[h]
\vspace{.25cm}
	\begin{subfigure}{.47\textwidth}
		\centering
		{\includegraphics[width=.9\textwidth]{figs/FinalResults/Shards/all_avg_txns_f1__W1.pdf}}\vspace{-.01cm}
		(a) Workload 1 (W1)
		%\caption{Workload 1 (W1)}
		%\label{fig:sfig1}
	\end{subfigure}%
	\qquad
	\begin{subfigure}{.47\textwidth}
		\centering
		{\includegraphics[width=.9\textwidth]{figs/FinalResults/Shards/all_avg_txns_f1__W2.pdf}}\vspace{-.01cm}
		(b) Workload 2 (W2)
		%\caption{Workload 2 (W2)}
		%\label{fig:sfig2}
	\end{subfigure}
	\vspace{-.21cm}
	\caption{Number of transactions allocated to a follower with varying transactions per block and varying data set ($\rho$).}
	\label{fig:transPerShard}
\end{figure}
\begin{comment}
\begin{figure}[t]
%\vspace{-.4cm}
\begin{minipage}{.48\textwidth}
\centering
{\includegraphics[width=.9\textwidth]{figs/FinalResults/Shards/w1-w2-num-Shards.pdf}}\vspace{-.15cm}
\caption{Number of shards per block with varying transactions per block and varying data set ($\rho$).}
\label{fig:ShardsPerBlock}
%\vspace{.35cm}
\end{minipage}
\qquad
\begin{minipage}{.48\textwidth}
\centering
{\includegraphics[width=.7\textwidth]{figs/FinalResults/Shards/w1-w2-size-Shards.pdf}}\vspace{-.15cm}
\caption{Number of transactions in a shard with varying transactions per block and varying data set ($\rho$).}
\label{fig:transPerShard}
%\vspace{-.55cm}
%\end{minipage}
\end{figure}
\end{comment}


==> Backup-intro.tex <==
\section{Introduction}
\label{introduction}
According to a report published by World  Economic  Forum  (WEF)  based on a survey on the future of the blockchain technology predicted that $\approx10\%$ of the Global Gross Domestic Product (GDP) would be stored on the blockchain by $2025$ \cite{WEFBlockchains2017}. Furthermore, with an annual growth rate of $26.2\%$, the capital market of $\$2.5$ billion in 2016 may touch the $\$19.9$ billion by 2025 \cite{Zhang:2019arXiv190307602Z, CoinDesk}. Many well-known information technology vendors, governments across the world, Internet giants, and banks are investing in blockchain to accelerate research to make distributed ledger technology versatile \cite{Zhang:2019arXiv190307602Z}. \todo{This text looks like has been lifted from elsewhere.}
% (such as Microsoft, IBM, HSBC, Cisco, JPMorgan, Goldman Sachs, etc.)

%A blockchain can be defined as a distributed decentralized database which is tamper-proof, publicly accessible, highly secure, append-only, the permanent collection of the records organized in the chain of the blocks \cite{nakamoto2009bitcoin, Dickerson+:ACSC:PODC:2017,Vikram:DBLP:journals/corr/abs, Ethereum, Hyperledger}. It maintains a distributed global state of the transactions in the absence of a trusted central authority. An anonymous group or individual known as Satoshi Nakamoto was the first who introduced blockchain in a paper titled Bitcoin: a peer-to-peer electronic cash system in 2008 \cite{nakamoto2009bitcoin}. Since then, it is commonly believed that there is a possibility of becoming rich by mining coins \cite{bitcoin:faq:2019}. Both industries and academia are trying to generalize this technology to support different type of applications. However, it is still not matured enough and experiencing a lot of development.

A blockchain is a distributed decentralized database which is a secure, tamper-proof, publicly accessible collection of the records organized as a chain of the blocks \cite{nakamoto2009bitcoin, Dickerson+:ACSC:PODC:2017,Vikram:DBLP:journals/corr/abs, Ethereum, Hyperledger}. It maintains a distributed global state of the transactions in the absence of a trusted central authority. Due to its usefulness, it has gained wide interest both in industry and academia. 

A blockchain is a distributed system consisting of \emph{nodes} or \emph{peers} maintained in a peer-to-peer manner. Normally, the entire copy of the blockchain is stored on all the nodes of the system. \emph{Clients} external to the system use the services of the blockahins by sending requests to the nodes of the blockchain systems. 

%Bitcoin is an application specific distributed ledger technology.
Bitcoin \cite{nakamoto2009bitcoin}, the first blockchain system proposed (by Satoshi Nakamoto), is the most popular blockchain system till date. It is a cryptocurrency system which is highly secure where the users need not trust anyone. Further there is no central controlling agency like current day banking system. Ethereum \cite{Ethereum} is another popular blockchain currently in use and provides various other services apart from cryptocurrencies. As compared to Bitcoin \cite{nakamoto2009bitcoin}, Ethereum  provides support for user-defined programs (scripts), called \emph{smart contracts} \cite{Solidity} to offer complex services. 

%Bitcoin \cite{nakamoto2009bitcoin} is a highly secure, cryptocurrency system is the first public blockchain which is still highly popular. It processes the transactions in a distributed decentralized manner where a user need not to trust anyone, further there is no central controlling agency like current day banking system. Ethereum \cite{Ethereum} is another popular blockchain. As compared to Bitcoin \cite{nakamoto2009bitcoin}, Ethereum  provides support for user-defined programs (scripts), called \emph{smart contracts} \cite{Solidity} to offer complex services. 

Smart contracts in the Ethereum are written in Turing complete language Solidity \cite{Solidity}. These contracts automatically provide several complex services using pre-recorded terms and conditions in the contract without the intervention of a trusted third party. In general, a smart contract is like an object in object-oriented programming languages, which consists of methods and data (state) \cite{Dickerson+:ACSC:PODC:2017, Solidity}. A client request, aka transaction, consists of these methods and corresponding input parameters. A transaction can be initiated by a client (user) or a peer and executed by all the peers. 

A client wishing to the use the services of the blockchain, contacts a node of the system and send the request which is a transaction. A node $N_i$ on receiving several such transactions from different clients or other peers, forms a \emph{block} to be added to the blockchain. The node $N_i$ is said to be a \emph{\bp} and cryptocurrencies based blockchains such as Bitcoin, Ethereum, \bp{s} are called as \emph{miners} as they can `mine' new coins. In this document, we use these terms interchangeably. 

%Whenever a user sends a request, the corresponding method of the contract is called by the miner, and the contract state may change to the new state. In Ethereum, every account has its separate space to maintain state updates. Contracts are also yet another address on Ethereum and maintain separate space for modifications done via contract transactions \cite{Ethereum}.

%It executes the respective methods of the contract and changes the current state of the contract to the new state.
%It uses the cryptographic algorithm to encrypt everything and record them in the form of a chain of the blocks hence known as a blockchain.

%In the current implementation of most popular blockchain designs such as Bitcoin \cite{nakamoto2009bitcoin} and Ethereum \cite{Ethereum}, these transactions are executed in an ordered manner first by the miner later by the validators \cite{Dickerson+:ACSC:PODC:2017}. Basically, when a miner creates a block, miner is given a choice to pick the transactions based on its preference, for e.g., giving high priority to higher transactions fees, sequentially execute associated transactions, find the proof-of-work (PoW), and finally broadcast the block to other peers for validation to earn reward and append it to its local blockchain. The validation by other peers is also done sequentially in the same order as proposed by the miner to attain the consensus. Finally, after successful validation of a block by the majority (accepted by more than 50\%) of the peers/validators, the consensus is reached, and the miner gets the incentive for that block.

In most of the popular blockchain systems such as Bitcoin and Ethereum, transactions in a block are executed in an ordered manner first by the miners later by the validators \cite{Dickerson+:ACSC:PODC:2017}. When a miner creates a block, the miners typically chooses transactions to form a block from a pool based on their preference, e.g., giving higher priority to transaction with higher fees. After selecting the transactions the miner (1) serially executes the transactions, (2) adds the final state of the system to the block after execution, (3) next find the proof-of-work (PoW) \cite{PoW} and (4) broadcast the block in the network to other peers for validation to earn the reward. PoW is an answer to a mathematical puzzle in which a miner tries to find the hash of the block smaller than the given difficulty. This technique is used in the Bitcoin and Ethereum. 

Later after receiving a block, a node validates the contents of the block. Such a node is called the \emph{validator}. Thus when a node $N_i$ is \bp then every other node in the system acts as a validator. Similarly when another node $N_j$ is the miner then $N_i$ acts as a validator. The validators (1) re-execute the transactions in the block received serially, (2) verify to see if the final state computed by them is same as the final state provided by the miner in the block, and (3) also validates if the miner solved the puzzle (PoW) correctly. The transaction re-execution by the validators is done serially in the same order as proposed by the miner to attain the consensus \cite{Dickerson+:ACSC:PODC:2017}. After validation, if the block is accepted by the majority (accepted by more than 50\%) of the validators, then the block is added to the blockchain, and the miner gets the incentive (in case Bitcoin and Ethereum).% However, it is also possible that multiple blocks are proposed and added to the chain at the same time, which creates the fork in the chain; but, the longest chain is considered as the consistent one.

%Further, blockchain is designed such a way that every block which is added to the chain depends on the previous block's hash to force a chronological order. This ordering based on cryptographic hash makes it exponentially challenging to make any change to earlier transactions because this will requires recalculation of PoW of all the subsequent blocks and accepted by the majority of them. Also if two blocks are proposed at the same time and added to the blockchain, they form the fork, miners work on the first block they receive and switch to the longest chain of blocks as soon as the next block is formed. This allows mining to secure and maintain a global consensus based on processing power. If a miner can possess the majority of compute power, then theoretically can manipulate the transactions for its own gain \cite{BC-Mining}.

Further, blockchain is designed such a way that it forces a chronological order between the blocks. Every block which is added to the chain depends on the cryptographic hash of the previous block. This ordering based on cryptographic hash makes it exponentially challenging to make any change to the previous blocks. In order to make any small change to already accepted transactions or a block stored in the blockchain requires recalculation of PoW of all the subsequent blocks and acceptance by the majority of the peers in the network. Also, if two blocks are proposed at the same time and added to the chain, they form a \emph{fork}. To resolve the forks, the branch with the longest chain is considered as the final. This allows mining to be secure and maintain a global consensus based on processing power.

% Miners work on the first block they receive and switch to the longest chain. 

% If a miner can possess the majority of computing power, then theoretically can manipulate the transactions for its gain \cite{BC-Mining}.
% Forks are formed in the absence of a robust consensus protocol. 
%miners work on the first block they receive and switch to the longest chain. These allow mining to be secure and maintain a global consensus based on processing power.% If a


%The problem in the above approach is that both miners and validators sequentially execute the transactions and finds the PoW. Further finding the PoW is highly computation intensive. In the current era of distributed and multi-core system, the sequential execution of the transactions results in poor throughput.

%The problem in the above approach is that both miners and validators sequentially execute the transactions and finds the PoW. Further finding the PoW is highly computational intensive and require a lot of calculation to form a block. The PoW is required to delay wait for the network to reach consensus and avoid miners to waste energy on execution of transactions in their favour. The high computation requirements make it very difficult for a resource constraint miner to compete for the block creation process to get intensive. In the literature, there are several solutions proposed to mitigate this issue. One such solution is that several resource constraint miners form a pool (community) and determines the PoW and at the end after successful block creation shares the incentive among them. For sharing the incentive several solutions have been proposed in the literature and used in the Bitcoin mining pools \cite{qin18mining, lewenberg2015bitcoin, MiningPools:NBERw25592}. In the rest of the paper we will use mining pool and mining community interchangeably.

%In most of the blockchains, PoW \cite{PoW} is used to achieve the consensus by all the peers in the system to add new blocks to the blockchain. So it is a consensus protocol which is nothing but a mathematical computation introduced in Bitcoin and later adopted by various other cryptocurrency based blockchain platforms. Adding a new block to the blockchain by solving a mathematical puzzle is known as mining, and the peers of the network who do this task are known as miners. The PoW requires a considerable amount of work and computations to solve the puzzle. The puzzle is to get an answer to the problem in which miners have to run a very long random trial and error procedure. The miners continuously test different numbers (nonce) until they find a lower number smaller than the block hash (i.e., the header of the hashed block). This answer is also known as the target hash. Finding the target hash is a random process, which means that it can be solved in a single attempt or may not be after so many trials.


%In the current implementation of Bitcoin and Ethereum, throughput is very low, which leads to poor transaction acceptance rate. Further, poor transaction acceptance rate leads to poor user experience. A user does not wish to wait for a longer time for his transaction to be accepted, and they prefer the current centralized system over the blockchain based solution. In Bitcoin, less than seven transactions are accepted per second over 6K full nodes; on the other hand in Ethereum, only four transactions are processed per second instead of a theoretical maximum of 25 \cite{Mustafa:DBLP:journals/corr/abs-1708-03778}. 

\vspace{1mm}
\noindent
\textbf{Drawback with Existing System:} The drawback with the existing blockchain system is that miners and validators execute the transactions serially and so is computing the PoW. Further, finding the PoW \cite{PoW} is highly computationally intensive random process which requires a lot of computation to create a new block. PoW is required to delay-wait the network to reach consensus and allow miners to create a new block in their favor. But the problem is that the high computation requirements make it very difficult for a resource constraint miner to compete for the block creation to get intensive \cite{Eyal:BitcoinMiningVulnerable}.

Also, in the current era of distributed and multi-core system, sequential transaction execution results in poor throughput. Dickerson et al., \cite{Dickerson+:ACSC:PODC:2017} observed that the transactions are executed serially in two different contexts. First, they are executed serially by the miner while creating a block. Later, validator re-executes the transactions serially to validate the block. Serial execution of the transaction leads to poor throughput. Also, block transactions are executed several times by the miners and many many times by the validators.

In addition to these problems, due to the substantial high transaction fee, poor throughput (transactions/second), significant transaction acceptance latency, and limited computation capacities prevent widespread adoption \cite{eos:url, BC-Scalability}. Hence adding parallelism to the blockchain can achieve better efficiency and higher throughput.

\vspace{1mm}
\noindent
\textbf{Solution Approach - Mining Pools:} There are few solutions proposed and used in Bitcoin and Ethereum blockchain to mitigate these issues. One such solution is that several resource constraint miners form a pool (community) known as \emph{mining pool} and determines the PoW, and after block acceptance, they share the incentive among them \cite{Eyal:BitcoinMiningVulnerable, Eyal:MiningPool, qin18mining, lewenberg2015bitcoin, MiningPools:NBERw25592, Wiki:MiningPool, MiningPoolCentralized}. %For sharing the incentive, several solutions (proportional, pay-per-share, pay-per-last-N-shares) have been proposed in the literature and implemented by the mining pools.
In the rest of the paper, we use pool and community interchangeably.

Other solutions as proposed by \cite{Dickerson+:ACSC:PODC:2017, Vikram:DBLP:journals/corr/abs, Anjana:OptSC:PDP:2019, ZangandZang:ECSC:WBD:2018, Anjana:DBLP:journals/corr/abs} suggested concurrent execution of the transactions at runtime. In proposed techniques, the concurrent execution is done in two stages first while forming the block and second while validating the block. It helps in achieving better speed up also increase chances of a miner to receive rewards. However, it is not straight forward and requires a proper strategy so that a valid block should not be rejected due to false block rejection or FBR error \cite{Anjana:DBLP:journals/corr/abs}.

In this work, our objective is to execute the transactions parallelly based on statical analysis based technique using community (pool) of the trusted nodes along with finding the PoW parallelly to improve the performance. We proposed a framework for distributed parallel execution in a formal setting based on Ethereum \cite{Ethereum}. The core idea is to form a community of multiple trusted nodes and make use of the distributed compute power using a master-slave approach. In proposed approach different tasks (transactions) are assigned to different nodes of the community (as depicted in \emph{Fig. \ref{fig:arch}}), the nodes execute the independent transactions (different shards) in parallel. As far as our knowledge, this is the first work which focuses on statical analysis based parallel execution of the block transactions and combines the benefit associated with sharding and mining pools.

\vspace{-.48cm}
\begin{figure}[hb!]
\centering
	{\includegraphics[width=0.38\textwidth]{figs/Distributed_execution_V2.pdf}}
	\caption{Sharding of the Block Transactions}
	\label{fig:ds}
\end{figure}
\vspace{-.35cm}

As shown in \emph{Fig. \ref{fig:ds}}, all the dependent transactions are grouped into one shard and executed serially; however, the non-conflicting transactions belong to different shards executed parallelly by different workers. In \emph{Fig. \ref{fig:ds}}, transaction \emph{T$_1$} access the account (data item) \emph{A$_1$}, \emph{A$_3$}, transaction \emph{T$_5$} access account \emph{A$_1$}, \emph{A$_8$}, and transaction \emph{T$_7$} access \emph{A$_2$}, \emph{A$_3$}. Here it can be seen that \emph{T$_1$, T$_5$}, and \emph{T$_7$} are accessing common data items (accounts) hence grouped into the same shard (\emph{Shard$_{1}$}). Similarly transaction \emph{T$_2$, T$_3$}, and \emph{T$_9$} are grouped into \emph{Shard$_{2}$}, while \emph{T$_4$, T$_6$,} and \emph{T$_8$} are grouped in \emph{Shard$_{3}$}. Further, there is no dependency between the shards. Hence these shards can be executed parallelly by different nodes of the community. The proposed technique is based on the assumption that there is no nested call between the transactions (one contract internally call to another contract). In the presence of nested transaction calls, the technique will not work.

%\noindent
%\textit{Why distributed mining?}
%\par Managing the cluster (compute nodes connected via high-speed LAN) by the solo miner will require skill to manage and cost associated with deployment and maintenance. With the above approach, unskilled peers can form a community and can share resources to gain the reward proportional to their participation. This approach will give equal opportunity to every peer to participate in the mining to earn the reward.


%\vspace{-.45cm}
\noindent
%\textbf{Contributions:}
\emph{The \textbf{major contributions} of this work is as follows:}
\begin{itemize}
    \item We propose a framework \emph{DiPETrans} for parallel execution of the transactions at miner and validator based on transaction sharding using static analysis and mining pools. The novelty of this work is that it is the first contribution which combines the advantages associated with both sharding and mining pools.% based parallel execution.% The proposed technique allows computation constraint miner to participate in the mining to earn the rewards (intensive) and improve the overall throughput of the system.
    \item Once the miner proposes a block; the validator executes the transactions parallelly using the same approach followed by the miner.% However, the only difference is that validators do not determine PoW.% The validator executes the transactions parallelly and checks the final state computed by them matches with the final state of the block as computed by the miner, subsequently also confirms that the PoW is valid or not.
    \item We implemented two different approaches for the validator; in the first approach, the miner incorporates some information about the conflicting transactions (shards) in the block to help the validators to execute the block transactions deterministically parallelly. While in the second approach, the miner does not include dependency information in the block, and validator have to determine the dependencies.
    \item We experimented with actual transactions from the Ethereum blockchain and simulated the behavior of the proposed technique to prove the potential benefits over traditional sequential execution.% We also show the tradeoff between sharing information about dependencies in the block to the validators concerning not sharing the information.
    \item The proposed approach achieved maximum speedup of $2.18\times$ for miner, $2.02\times$ for \emph{no info sharing validator} and $2.04\times$ for \emph{info sharing validator} for 100 to 500 transactions per block with max 5 workers in the community. %this should not come as a contribution but is more of a result.
    %\item The proposed approach achieves linear speedup for overall block execution at miner using distributed execution of transaction and mining. We achieved \textit{xxxx}, \textit{yyyy}, and \textit{zzzz} speedup for \emph{miner, info sharing validator}, and \emph{no info sharing validator} respectively.
\end{itemize}

The rest of the paper is organized as follows: We present the related work and literature in \textit{Section \ref{relatedWork}}. While in \textit{Section \ref{methodology}}, we describe the proposed methodology, \emph{DiPETrans} architecture, and algorithms. \textit{Section \ref{experiment}} consist of the experimental evaluation and results. Finally, we conclude with some future research directions in \textit{Section \ref{conclusion}}.

%The rest of the paper is organised as follows: in \textit{Section \ref{relatedWork}} we present the related work. The proposed methodology, architecture, and algorithms are given in the \textit{Section \ref{methodology}}. While \textit{Section \ref{expriment}} consist of the experimental evaluation and results. Finally in the \textit{Section \ref{conclusion}} we will conclude with some future research directions.

%The rest of the paper is organised as follows: In \textit{Section \ref{relatedWork}}, we summarize the related literature. The proposed methodology, architecture, and algorithms are presented in the \textit{Section \ref{methodology}}. \textit{Section \ref{experiment}} consist of the experimental evaluation and results. Finally, at the end, we conclude with some future research directions in \textit{Section \ref{conclusion}}.

==> ap-summryEthTx.tex <==
\subsection{Summary of Ethereum Transaction Data}
\label{apn:SETD}
This section presents the data set designed for the experiment using transactions extracted from Ethereum blockchain and smart contract calls implemented in \emph{C++} as given in the \emph{Table \ref{tab:txn-sim} and Table \ref{tab:sc-calls}}. In the \emph{Table \ref{tab:txn-sim}} \emph{data-1-1-100} represents that 1:1 is the ratio of contractual : monetary transactions per block while 100 is the total number of transactions per block. 


%\vspace{-.4cm}
\begin{table}[ht!]
    \centering
    \caption{Summary of Simulated Transactions Data}\vspace{-.3cm}
    \label{tab:txn-sim}
    \resizebox{0.45\textwidth}{!}{%
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        \emph{\textbf{S. No.}} & \emph{\textbf{Data (\#Txns/Block)}} & \emph{\textbf{\#Blocks}} & \emph{\textbf{\#Contract\_Txns}} & \emph{\textbf{\#Non\_Contract\_Txns}}\\
        \hline
        1 & data-1-1-100 & 3,880 & 193,959 & 194,000 \\
		2 & data-1-1-200 & 1,940 & 193,959 & 194,000 \\
        3 & data-1-1-300 & 1,294 & 193,959 & 194,100 \\
        4 & data-1-1-400 & 970 & 193,959 & 194,000 \\
        5 & data-1-1-500 & 776 & 193,959 & 194,000 \\
        \hline
        6 & data-1-2-100 & 5,705 & 193,959 & 376,530 \\
        7 & data-1-2-200 & 2,895 & 193,959 & 385,035 \\
        8 & data-1-2-300 & 1,940 & 193,959 & 388,000 \\
        9 & data-1-2-400 & 1,448 & 193,959 & 385,168 \\
        10 & data-1-2-500 & 1,162 & 193,959 & 386,946 \\
        \hline
        11 & data-1-4-100 & 9,698 & 193,959 & 775,840 \\
		12 & data-1-4-200 & 4,849 & 193,959 & 775,840 \\
        13 & data-1-4-300 & 3,233 & 193,959 & 775,840 \\
        14 & data-1-4-400 & 2,425 & 193,959 & 776,000 \\
        15 & data-1-4-500 & 1,940 & 193,959 & 776,000 \\
        \hline
        16 & data-1-8-100 & 16,164 & 193,959 & 1,422,432 \\
        17 & data-1-8-200 & 8,434 & 193,959 & 1,492,818 \\
        18 & data-1-8-300 & 5,705 & 193,959 & 1,517,530 \\
        19 & data-1-8-400 & 4,311 & 193,959 & 1,530,405 \\
        20 & data-1-8-500 & 3,464 & 193,959 & 1,538,016 \\
        \hline
        21 & data-1-16-100 & 32,327 & 193,959 & 3,038,738 \\
		22 & data-1-16-200 & 16,164 & 193,959 & 3,038,832 \\
        23 & data-1-16-300 & 10,776 & 193,959 & 3,038,832 \\
        24 & data-1-16-400 & 8,082 & 193,959 & 3,038,832 \\
        25 & data-1-16-500 & 6,466 & 193,959 & 3,039,020 \\
        \hline
    \end{tabular}
    }
\end{table}


%\vspace{-.2cm}
\begin{table}[ht!]
    \centering
    \caption{Summary of Contract Transactions Calls}
    \vspace{-.3cm}
    \label{tab:sc-calls}
    \resizebox{.49\textwidth}{!}{%
    \begin{tabular}{|c|p{2.5cm}|p{1.63cm}|p{3.3cm}|p{.9cm}|c|}
        \hline
        \emph{\textbf{S.No.}} &\emph{\textbf{Fn Name}} & \emph{\textbf{Fn Hash}} & \emph{\textbf{Parameters}} & \emph{\textbf{\#Txns}} &  \emph{\textbf{Percentile}}\\
        \hline
        1 & transfer & 0xa9059cbb & address, uint256 & 56,654 & 37.72 \\
        2 & approve & 0x095ea7b3 & address, uint256 & 11,799 & 45.58 \\
        3 & vote & 0x0121b93f & uint256 & 11,509 & 53.24 \\
        4 & submitTransaction & 0xc6427474 & address, uint256,bytes & 8,163 & 58.67 \\
        5 & issue & 0x867904b4 & address,uint256 & 5,723 & 62.49 \\
        6 & \_\_callback & 0x38bbfa50 & bytes32, string, bytes & 5,006 & 65.82 \\
        7 & playerRollDice & 0xdc6dd152 & uint256 & 4,997 & 69.15 \\
        8 & multisend & 0xad8733ca & address,address[], uint256[] & 4,822 & 72.36 \\
        9 & SmartAirdrop & 0xa8faf6f0 & - & 4,467 & 75.33 \\
        10 & PublicMine & 0x87ccccb3 & - & 4,157 & 78.10 \\
        11 & setGenesisAddress & 0x0d571742 & address, uint256, bytes & 3,119 & 80.17 \\
        \hline
    \end{tabular}

    }
\end{table}


==> shards-results.tex <==
\begin{figure}[h]
	\begin{subfigure}{.47\textwidth}
		\centering
		{\includegraphics[width=.9\textwidth]{figs/FinalResults/Shards/all_num_shards_W1.pdf}}\vspace{-.01cm}
		(a) Workload 1 (W1)
		%\caption{Workload 1 (W1)}
		%\label{fig:sfig1}
	\end{subfigure}%
	\qquad
	\begin{subfigure}{.47\textwidth}
		\centering
		{\includegraphics[width=.9\textwidth]{figs/FinalResults/Shards/all_num_shards_W2.pdf}}\vspace{-.01cm}
		(b) Workload 2 (W2)
		%\caption{Workload 2 (W2)}
		%\label{fig:sfig2}
	\end{subfigure}
	\vspace{-.21cm}
	\caption{Number of shards with varying transactions per block and varying data set ($\rho$).}
	\label{fig:ShardsPerBlock}
%\end{figure}
%\begin{figure}[h]
\vspace{.25cm}
	\begin{subfigure}{.47\textwidth}
		\centering
		{\includegraphics[width=.9\textwidth]{figs/FinalResults/Shards/all_max_trans_shard__W1.pdf}}\vspace{-.01cm}
		(a) Workload 1 (W1)
		%\caption{Workload 1 (W1)}
		%\label{fig:sfig1}
	\end{subfigure}%
	\qquad
	\begin{subfigure}{.47\textwidth}
		\centering
		{\includegraphics[width=.9\textwidth]{figs/FinalResults/Shards/all_max_trans_shard__W2.pdf}}\vspace{-.01cm}
		(b) Workload 2 (W2)
		%\caption{Workload 2 (W2)}
		%\label{fig:sfig2}
	\end{subfigure}
	\vspace{-.21cm}
	\caption{Number of transactions in a shard with varying transactions per block and varying data set ($\rho$).}
	\label{fig:transPerShard}
%\end{figure}
%\begin{figure}[h]
\vspace{.25cm}
	\begin{subfigure}{.47\textwidth}
		\centering
		{\includegraphics[width=.9\textwidth]{figs/FinalResults/Shards/all_avg_txns_f1__W1.pdf}}\vspace{-.01cm}
		(a) Workload 1 (W1)
		%\caption{Workload 1 (W1)}
		%\label{fig:sfig1}
	\end{subfigure}%
	\qquad
	\begin{subfigure}{.47\textwidth}
		\centering
		{\includegraphics[width=.9\textwidth]{figs/FinalResults/Shards/all_avg_txns_f1__W2.pdf}}\vspace{-.01cm}
		(b) Workload 2 (W2)
		%\caption{Workload 2 (W2)}
		%\label{fig:sfig2}
	\end{subfigure}
	\vspace{-.21cm}
	\caption{Number of transactions allocated to a follower with varying transactions per block and varying data set ($\rho$).}
	\label{fig:transPerShard}
\end{figure}
\begin{comment}
\begin{figure}[t]
%\vspace{-.4cm}
\begin{minipage}{.48\textwidth}
\centering
{\includegraphics[width=.9\textwidth]{figs/FinalResults/Shards/w1-w2-num-Shards.pdf}}\vspace{-.15cm}
\caption{Number of shards per block with varying transactions per block and varying data set ($\rho$).}
\label{fig:ShardsPerBlock}
%\vspace{.35cm}
\end{minipage}
\qquad
\begin{minipage}{.48\textwidth}
\centering
{\includegraphics[width=.7\textwidth]{figs/FinalResults/Shards/w1-w2-size-Shards.pdf}}\vspace{-.15cm}
\caption{Number of transactions in a shard with varying transactions per block and varying data set ($\rho$).}
\label{fig:transPerShard}
%\vspace{-.55cm}
%\end{minipage}
\end{figure}
\end{comment}

